A Feasibility Study on Indoor Localization and Multi-person Tracking Using Sparsely Distributed Camera Network with Edge Computing

Camera-based activity monitoring systems are becoming an attractive solution for smart building applications with the advances in computer vision and edge computing technologies. In this paper, we present a feasibility study and systematic analysis of a camera-based indoor localization and multi-person tracking system implemented on edge computing devices within a large indoor space. To this end, we deployed an end-to-end edge computing pipeline that utilizes multiple cameras to achieve localization, body orientation estimation and tracking of multiple individuals within a large therapeutic space spanning $1700m^2$, all while maintaining a strong focus on preserving privacy. Our pipeline consists of 39 edge computing camera systems equipped with Tensor Processing Units (TPUs) placed in the indoor space's ceiling. To ensure the privacy of individuals, a real-time multi-person pose estimation algorithm runs on the TPU of the computing camera system. This algorithm extracts poses and bounding boxes, which are utilized for indoor localization, body orientation estimation, and multi-person tracking. Our pipeline demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree. These results shows that localization and tracking of individuals in a large indoor space is feasible even with the privacy constrains.

==> abstract/_main_20231029.tex <==
% Abstract
% It is crucial to understand how individuals move during space navigation and socially interact in large indoor environments, as they are related to the mental and cognitive health of individuals.
% Prior approaches for monitoring indoor activities either captured coarse movements at a room level or required significant modifications to the existing infrastructure.
% Here we present a low-cost, therefore scalable, edge computing framework for tracking multiple people's detailed movements in indoor spaces of 18000+ square meters throughout a day.
% Our computing framework consists of 39 Raspberry Pi cameras that are placed in the ceiling and connected to on-premise fog server through a secure and private network.
% To maintain user privacy, Pis run multi-person detection and pose estimation models in real-time.
% By using Kalman filter-based multi-person tracking and state-of-the-art body orientation estimation methods, we are able to determine the whereabouts and facing orientations of multiple people simultaneously.
% Our system demonstrated a localization error of 1.41 meters, a Multiple-Object Tracking Accuracy (MOTA) score of 62+\%, and a mean absolute body orientation error of 29\degree on average, which was sufficient to understand group activity behaviors in wide built-in environments. 
% Our study provides practical guidance for deploying the proposed system by analyzing camera installation with respect to tracking accuracy.
% We expect the proposed system to transform existing healthcare institutions into smart spaces with low costs for improving patient well-being.
Localization of individuals in a built environment is a growing research topic. Estimating the positions, face orientation (or gaze direction) and trajectories of people through space has many uses, such as in crowd management, security, and healthcare. 
In this work, we present an open-source\footnote{https://github.com/redacted. We will release the code upon the acceptance of our manuscript.} low-cost, scalable and privacy-preserving edge computing framework for multi-person localization, i.e. estimating the positions, orientations, and trajectories of multiple people in an indoor space.
Our computing framework consists of 39 Tensor Processing Unit (TPU)-enabled edge computing camera systems placed in the ceiling of the indoor therapeutic space. The edge compute systems are connected to an on-premise fog server through a secure and private network. 
A multi-person detection algorithm and a pose estimation model run on the edge TPU in real-time to collect features which are used, instead of raw images, for downstream computations. This ensures the privacy of individuals in the space, reduces data transmission/storage and improves scalability.
We implemented a Kalman filter-based multi-person tracking method and a state-of-the-art body orientation estimation method to determine the positions and facing orientations of multiple people simultaneously in the indoor space. 
For our study site with size of 18,000 square feet, our system demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree, which is sufficient for understanding group activity behaviors in indoor environments.
Additionally, our study provides practical guidance for deploying the proposed system by analyzing various elements of the camera installation with respect to tracking accuracy. 



==> abstract/main.tex <==
% Abstract
% It is crucial to understand how individuals move during space navigation and socially interact in large indoor environments, as they are related to the mental and cognitive health of individuals.
% Prior approaches for monitoring indoor activities either captured coarse movements at a room level or required significant modifications to the existing infrastructure.
% Here we present a low-cost, therefore scalable, edge computing framework for tracking multiple people's detailed movements in indoor spaces of 18000+ square meters throughout a day.
% Our computing framework consists of 39 Raspberry Pi cameras that are placed in the ceiling and connected to on-premise fog server through a secure and private network.
% To maintain user privacy, Pis run multi-person detection and pose estimation models in real-time.
% By using Kalman filter-based multi-person tracking and state-of-the-art body orientation estimation methods, we are able to determine the whereabouts and facing orientations of multiple people simultaneously.
% Our system demonstrated a localization error of 1.41 meters, a Multiple-Object Tracking Accuracy (MOTA) score of 62+\%, and a mean absolute body orientation error of 29\degree on average, which was sufficient to understand group activity behaviors in wide built-in environments. 
% Our study provides practical guidance for deploying the proposed system by analyzing camera installation with respect to tracking accuracy.
% We expect the proposed system to transform existing healthcare institutions into smart spaces with low costs for improving patient well-being.
% Localization of individuals in a built environment is a growing research topic. Estimating the positions, face orientation (or gaze direction) and trajectories of people through space has many uses, such as in crowd management, security, and healthcare. 
\revision{
Camera-based activity monitoring systems are becoming an attractive solution for smart building applications with the advances in computer vision and edge computing technologies.
In this study, we present a feasibility study and systematic analysis of camera-based indoor localization and multi-person tracking systems using edge computing devices when deployed in a large therapeutic indoor space spanning 1700$m^2$. 
The goal is to provide practical considerations for implementing such a system for indoor activity monitoring.
Our framework consists of 39 Tensor Processing Unit (TPU)-enabled edge computing camera systems placed in the ceiling of the indoor space. 
To ensure the privacy of individuals, a multi-person pose estimation algorithm runs on the edge TPU in real-time, in which poses and bounding boxes are used for indoor localization, body orientation estimation, and multi-person tracking\footnote{https://github.com/redacted. We will release the code upon the acceptance of our manuscript.}.
Although with sparsely distributed camera networks, our system demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree, which is sufficient for comprehensively assessing the various elements of the camera installation with respect to monitoring fine-grained group activities in indoor environments.
}
% In this work, we present an open-source\footnote{https://github.com/redacted. We will release the code upon the acceptance of our manuscript.} low-cost, scalable and privacy-preserving edge computing framework for multi-person localization, i.e. estimating the positions, orientations, and trajectories of multiple people in an indoor space.
% Our computing framework consists of 39 Tensor Processing Unit (TPU)-enabled edge computing camera systems placed in the ceiling of the indoor therapeutic space. 
% The edge compute systems are connected to an on-premise fog server through a secure and private network. 
% A multi-person detection algorithm and a pose estimation model run on the edge TPU in real-time to collect features which are used, instead of raw images, for downstream computations. This ensures the privacy of individuals in the space, reduces data transmission/storage and improves scalability.
% We implemented a Kalman filter-based multi-person tracking method and a state-of-the-art body orientation estimation method to determine the positions and facing orientations of multiple people simultaneously in the indoor space. 
% For our study site with size of 18,000 square feet, our system demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree, which is sufficient for understanding group activity behaviors in indoor environments.
% Additionally, our study provides practical guidance for deploying the proposed system by analyzing various elements of the camera installation with respect to tracking accuracy. 

% collect features which are used, instead of raw images, for downstream computations. This ensures the privacy of individuals in the space, reduces data transmission/storage and improves scalability.


==> abstract/main_alternate.tex <==
% Abstract
% It is crucial to understand how individuals move during space navigation and socially interact in large indoor environments, as they are related to the mental and cognitive health of individuals.
% Prior approaches for monitoring indoor activities either captured coarse movements at a room level or required significant modifications to the existing infrastructure.
% Here we present a low-cost, therefore scalable, edge computing framework for tracking multiple people's detailed movements in indoor spaces of 18000+ square meters throughout a day.
% Our computing framework consists of 39 Raspberry Pi cameras that are placed in the ceiling and connected to on-premise fog server through a secure and private network.
% To maintain user privacy, Pis run multi-person detection and pose estimation models in real-time.
% By using Kalman filter-based multi-person tracking and state-of-the-art body orientation estimation methods, we are able to determine the whereabouts and facing orientations of multiple people simultaneously.
% Our system demonstrated a localization error of 1.41 meters, a Multiple-Object Tracking Accuracy (MOTA) score of 62+\%, and a mean absolute body orientation error of 29\degree on average, which was sufficient to understand group activity behaviors in wide built-in environments. 
% Our study provides practical guidance for deploying the proposed system by analyzing camera installation with respect to tracking accuracy.
% We expect the proposed system to transform existing healthcare institutions into smart spaces with low costs for improving patient well-being.
% Localization of individuals in a built environment is a growing research topic. Estimating the positions, face orientation (or gaze direction) and trajectories of people through space has many uses, such as in crowd management, security, and healthcare. 
\revision{
Camera-based activity monitoring systems are becoming an attractive solution for smart building applications with the advances in computer vision and edge computing technologies.
This paper introduces a comprehensive edge computing pipeline that utilizes multiple cameras to localize and track multiple individuals within a large indoor space, all while maintaining a strong focus on preserving privacy. The paper also includes a systematic analysis to assess the feasibility of the proposed system, providing practical insights for implementing indoor activity monitoring. %The goal is to provide practical considerations for implementing such a system for indoor activity monitoring.
Our pipeline consists of 39 edge computing camera systems equipped with Tensor Processing Units (TPUs) placed in the indoor space's ceiling. 
To ensure the privacy of individuals, a real-time multi-person pose estimation algorithm runs on the TPU of the computing camera system. This algorithm extracts poses and bounding boxes, which are utilized for indoor localization, body orientation estimation, and multi-person tracking \footnote{https://github.com/redacted. We will release the code upon the acceptance of our manuscript}.
Our pipeline demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree. These results shows that localization and tracking of individuals in a large indoor space is feasible even with the constrain of privacy.  }

%Although with sparsely distributed camera networks, our system demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree, which is sufficient for comprehensively assessing the various elements of the camera installation with respect to monitoring fine-grained group activities in indoor environments.
%}
% In this work, we present an open-source\footnote{https://github.com/redacted. We will release the code upon the acceptance of our manuscript.} low-cost, scalable and privacy-preserving edge computing framework for multi-person localization, i.e. estimating the positions, orientations, and trajectories of multiple people in an indoor space.
% Our computing framework consists of 39 Tensor Processing Unit (TPU)-enabled edge computing camera systems placed in the ceiling of the indoor therapeutic space. 
% The edge compute systems are connected to an on-premise fog server through a secure and private network. 
% A multi-person detection algorithm and a pose estimation model run on the edge TPU in real-time to collect features which are used, instead of raw images, for downstream computations. This ensures the privacy of individuals in the space, reduces data transmission/storage and improves scalability.
% We implemented a Kalman filter-based multi-person tracking method and a state-of-the-art body orientation estimation method to determine the positions and facing orientations of multiple people simultaneously in the indoor space. 
% For our study site with size of 18,000 square feet, our system demonstrated an average localization error of 1.41 meters, a multiple-object tracking accuracy score of 88.6\%, and a mean absolute body orientation error of 29\degree, which is sufficient for understanding group activity behaviors in indoor environments.
% Additionally, our study provides practical guidance for deploying the proposed system by analyzing various elements of the camera installation with respect to tracking accuracy. 

% collect features which are used, instead of raw images, for downstream computations. This ensures the privacy of individuals in the space, reduces data transmission/storage and improves scalability.


==> figure/discuss_cam_install.tex <==
\begin{figure}[t]
    \centering
    \begin{adjustbox}{width=\textwidth,center}
    \begin{tabular}{c@{\hspace{1mm}} c c c c c}
        & % y label 
        & % y label
        Distance between &
        Facing angle &
        Horizontal  &
        Vertical  \\
        & % y label 
        & % y label
        camera and target (m) &
        away from camera &
        angle/Field-of-View &
        angle/Field-of-View \\
        & % y label 
        & % y label
        \includegraphics[align=c, height=0.2\linewidth]{figure/discuss_cam_install/cam_dist.png} &
        \includegraphics[align=c, height=0.2\linewidth]{figure/discuss_cam_install/facing_angle.png} &
        \includegraphics[align=c, height=0.2\linewidth]{figure/discuss_cam_install/hori_angle.png} &
        \includegraphics[align=c, height=0.2\linewidth]{figure/discuss_cam_install/vert_angle.png} \\
        \rotatebox[origin=c]{90}{Localization} &
        \rotatebox[origin=c]{90}{error (meter)} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/cam_dist-loc_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/facing-loc_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/hori_angle-loc_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/vert_angle-loc_err.png} \\
        \rotatebox[origin=c]{90}{Orientation} &
        \rotatebox[origin=c]{90}{error (degree)} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/cam_dist-ori_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/facing-ori_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/hori_angle-ori_err.png} &
        \includegraphics[align=c, height=0.24\linewidth]{figure/discuss_cam_install/vert_angle-ori_err.png} \\
        & &
        D (m) & 
        $\theta$\degree &
        $\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$ &
        $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$ 
    \end{tabular}
    \end{adjustbox}
    \vspace{-0.1in}
    \caption{Localization and orientation errors regarding camera installation.
    We studied four aspects (1st row) of camera installation using dataset captured from four people walking in the study site.
    Those include 1) the distance between the camera and the person in the space (1st col.), 2) a person's facing direction away from the camera (2nd col.), 3) the horizontal angle of the captured person from the camera center (3rd col.), and 4) vertical angle of the capture person's feet location from camera center (4th col.).
    The horizontal angle ($\theta\degree_H$; 3rd col.) and vertical angle ($\theta\degree_V$; 4th col.) are normalized by horizontal ($\theta\degree_{H_{FOV}}$) and vertical ($\theta\degree_{V_{FOV}}$) field-of-view angles, respectively, referring to the camera datasheet  (Sony IMX219 8-megapixel sensor).
    Each of the aspects is associated with localization (2nd row) and orientation estimation (3rd row) errors in each sample.
    The correlation plot shows denser samples with \textcolor{blue}{BLUE}.
    The localization error and orientation error were strongly correlated with the distance between the camera and the captured person's location ($D$; 1st col.), the facing direction away from the camera ($\theta$; 2nd col.), and the normalized horizontal angle ($\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$; 3rd col.), and they were strongly negatively correlated with the normalized vertical angle($\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$; 4th col.).    
    This shows that multiple cameras installed densely with multiple views are important, as such systems allow people to be captured from closer distances ($<15m$) and directly from their facing direction ($\theta\degree_H<30\degree$), which leads to a more accurate estimate of body orientation and localization.  
    }
    \label{fig:corr_analysis}
\end{figure}

==> figure/orientation.tex <==
\begin{figure}
    \centering
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c c c}
            Activity Area &
            Kitchen &
            Left Corridor \\
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Activity area.accuracy-X.png} &
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Kitchen area.accuracy-X.png} &
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Left corridor.accuracy-X.png} \\
             Lounge &
             Right Corridor &
             Staff Zone &
             Overall \\
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Lobby.accuracy-X.png} &
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Right corridor.accuracy-X.png} &
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/Localization.Staff area.accuracy-X.png} &
             \includegraphics[width=.25\linewidth]{figure/orientation/accuracy-x/all_sess.accuracy-X.png}
        \end{tabular}
    \end{adjustbox}    
    \caption{Accuracy-$X\degree$ for body orientation estimation from different areas. 
    We show the accuracy when $X$s are 45\degree (\textcolor{red}{RED}), 90\degree (\textcolor{blue}{BLUE}), and 120\degree (\textcolor{green}{GREEN}) which corresponds to the accuracy of  eight-way (N, NE, E, SE, S, SW, W, NW), four-way (N, E, S, W), and three-way direction estimation}
    \label{fig:ori-accuracy-x}
\end{figure}



==> figure/tracker.tex <==
\begin{figure*}[t]
    \centering
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c}
            \includegraphics[align=c, height=.4\linewidth]{figure/tracker/kalman_tracker.png} &
            \includegraphics[align=c, height=.4\linewidth]{figure/tracker/hungarian_matching.png} \\
            (a) & (b) 
        \end{tabular}
    \end{adjustbox}
    \vspace{-0.1in}
       \caption{Kalman filter-based multi-person tracker using predict, detect, match, update, and repeat framework.
       (a) Given multi-person tracking until time $t-1$, Kalman filter trackers make predictions of each person's location at time $t$. 
       Then, the Hungarian method finds matches between 2D poses from predictions and detections at time $t$, shown in \textcolor{red}{red} lines in (b).
       The predictions get updated with the matched detections.
       The corresponding matches between predictions and detections in time $t-1$ and $t$ are color coded as \textcolor{green}{green} and \textcolor{blue}{blue}.
       For the unmatched detections, a new tracker initiates, which is \textcolor{red}{red}.
       Until the tracking is complete, this process is repeated.
       % \yash{what green and blue color represent? are they used to represent two seperate objects? I suggest reshaping the figure by increasing the size of nested pictures.}\hyeok{Explained colors. And increased the size of figure.}
       (b) Hungarian matching algorithm finds the most similar 2D poses between prediction and detections based on $L_2$-norm distance between all pairs of poses.
       }
    \label{fig:kalman_tracker}
\end{figure*}

==> sections/conclusion/main.tex <==
\section{Conclusion}

% A movement monitoring system should be considerate of the privacy of the subjects and needs to operate continuously and passively at low cost so that it can be adapted to existing infrastructures. 
% Previous monitoring systems, however, were limited by either a lack of granularity of tracking or cost and fabrication factors that prevented them from being scalable.
\revision{
The camera-based movement monitoring system is becoming popular with the advancements in edge computing platforms and computer vision techniques.
In this work, we study the feasibility of using edge computing cameras for monitoring activities in a large therapeutic space through a comprehensive analysis of indoor localization, multi-person tracking, and body orientation estimation techniques.
Our sensing hub uses low-cost edge computing devices - a Raspberry Pi, its camera module, a TPU, and a computing structure that is easy to install in existing buildings. 
}
% This system is integrated with an efficient machine learning system that is capable of detecting multiple people and monitoring their trajectory and body orientation throughout the day.
% Since these devices are small and inexpensive, we were able to conceal 39 edge computing systems above the ceiling tiles, where power and network connections were available, and have a small camera attached below the tiles in a manner similar to a smoke detector.
In our study, the described system demonstrated highly reliable multi-person tracking ($62.0\sim88.6\%$ MOTA) and body orientation estimation (29.0\degree) across various functional spaces.
For the region with more cameras ($7>$), our system could track people in crowded activities with a higher level of accuracy (88.6\% MOTA).
Furthermore, we expect our detailed analysis of the camera installation to provide practical guidelines for those who plan to transform their spaces by integrating our pipeline.
In our future work, we intend to increase the density of camera installation following our analysis and test the feasibility of tracking social interactions in more complex scenarios in which people have group activities surrounded by furniture or using gym equipment.


==> sections/conclusion/main_alternate.tex <==
\section{Conclusion}
\revision{
Camera-based movement monitoring systems are gaining popularity thanks to the progress in edge computing platforms and computer vision methodologies. In this study, we proposed an edge computing pipeline for localization and tracking of individuals in a vast indoor space while preserving privacy. We also demonstrated the practicality of employing the edge computing cameras to monitor activities within the space using indoor localization, multi-person tracking, and body orientation estimation. Our sensing hub leveraged cost-effective edge computing components, including a Raspberry Pi, its camera module, a Tensor Processing Unit (TPU), and a user-friendly computing infrastructure that can be readily integrated into pre-existing building setups.
}
% This system is integrated with an efficient machine learning system that is capable of detecting multiple people and monitoring their trajectory and body orientation throughout the day.
% Since these devices are small and inexpensive, we were able to conceal 39 edge computing systems above the ceiling tiles, where power and network connections were available, and have a small camera attached below the tiles in a manner similar to a smoke detector.
In our study, the described system demonstrated highly reliable multi-person tracking ($62.0\sim88.6\%$ MOTA) and body orientation estimation (29.0\degree) across various functional spaces.
For the region with more cameras ($7>$), our system could track people in crowded activities with a higher level of accuracy (88.6\% MOTA).
Additionally, we anticipate that our comprehensive examination of camera installation will offer valuable insights for individuals interested in implementing our system to enhance their environments. In our future work, we plan to increase the camera density based on the insights from our analysis. We will also assess the viability of tracking social interactions in more intricate settings, such as those involving group activities amid furnishings or the use of gym equipment.



==> sections/discussion/_main_20230329.tex <==
\section{Discussion}

Here, we demonstrate how camera installation changes model behavior with respect to localization and body orientation estimation tasks.
Then, we discuss the limitation and potential applications of the proposed method that can largely benefit from our low-cost and privacy-preserving monitoring system using distributed camera networks.

\subsection{Impact of Camera Installation on Model Behavior}
\label{sec:cam_install}

\input{figure/discuss_cam_install}

In our study site, the camera installation is determined primarily by the power and network source reachable using extension cables, resulting in 39 cameras unequally installed in the space. %\yash{"uniformly installed throughout the space"}\hyeok{No. it is not true.}
From our localization and body orientation analysis, we observed the density of the cameras (number of cameras per captured area size) is highly correlated with the accuracy of the model.
Here, we examine this in more detail to understand the impact of camera installation on four different factors related to localization and body orientation estimation accuracy.
Those include 1) the distance between the camera and the captured person, 2) the facing direction of the captured person from camera viewpoints, 3) the horizontal location of the captured person away from the camera center, and 4) the vertical location of the captured person's foot location from camera center.
\autoref{fig:corr_analysis} shows Pearson correlation analysis for each factor we study, where denser samples are colored more \textcolor{blue}{BLUE}.

\subsubsection{Distance Between Camera and Person}

Across all cameras, we measured the distance between captured people from the camera location and the corresponding localization errors (\autoref{fig:corr_analysis}; 1st col).
Localization error (2nd row) showed that the majority of our samples were within ~ 2 meters error when the distance between the person and camera was within 15 meters.
A strong positive correlation exists between the localization error and camera distance as the distance increases from 20 meters ($R=0.823$, $p<0.005$). %\yash{whats the null hypothesis here?}\hyeok{null hypothesis is that no correlation exists.}
Orientation error (3rd row) also demonstrated a positive correlation with the increasing distance of the captured person from the camera ($R=0.335$, $p < 0.005$).
The majority of orientation errors were less than $25\degree$ when the location of captured person was below 15 meters.
This shows that the Raspberry Pi camera (Sony IMX219 8-megapixel sensor) can capture objects well within 15 meters, which is large enough for our pose estimation and body orientation estimation model to make accurate predictions.
As a result of the person being further away from the camera, the pixel region that constitutes the person decreases significantly, which increases the errors in body orientation and localization.
The model was more confused when people were occluding each other, as multiple people looked like a single person from a distance.

\subsubsection{Facing Angle Away from Camera Viewpoint}

The facing direction of the captured person had a significant impact on the accuracy of both localization and body orientation estimation (\autoref{fig:corr_analysis}; 2nd col).
The facing angles within $50\degree$ were found to be crucial to ensuring a $<2m$ localization error and a $<25\degree$ body orientation error.
Specifically, the 2D pose estimation model performed best when the person was facing the camera, and as the person turned, more distortions were introduced to the estimated keypoint locations, which affected localization accuracy.
This was similar to the body orientation estimation model, as the confidence of the model was high when the person was facing forward. 
The model had more confusion as the person started facing away from the camera.
Many times, pose estimation models confused frontal and rear views of the person, especially when the person was farther than $20m$ from the camera, resulting in unrealistically twisted keypoints.
There was a strong positive correlation between the facing angle and both localization ($R=0.375$, $p<0.005$) and body orientation estimation ($R=0.436$, $p<0.005$) errors.

\subsubsection{Horizontal Displacement from Camera Center}

Next, we studied the impact of the horizontal displacement of the captured person from the camera center (\autoref{fig:corr_analysis}; 3rd col).
We quantified the horizontal displacement as the horizontal angle, $\theta\degree_H$, of the person from the camera center that is normalized by horizontal field-of-view, $\theta\degree_{H_{FOV}}$, which is normalized horizontal angle, $\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$.
As a person gets closer to the horizontal center of the camera, the normalized horizontal angle approaches zero.
The normalized horizontal angle increases to $1$ when the person is at the edge of the frame. 
When the value is larger than $1$, then only part of the body is observable from the camera.
According to our analysis, the person must be captured within 30\% of horizontal camera displacement to have a localization error of less than $2m$ and an orientation error of less than 25\degree.
The localization and body orientation errors increased with strong positive correlations as the captured person moved away from the horizontal center, $R=0.681 (p<0.005)$ and $R=0.467 (p<0.005)$, respectively.
Again, this illustrates the advantage of densely installing camera to capture people with overlapping viewpoints of $30\degree$ horizontal angle displacements.

\subsubsection{Vertical Displacement from Camera Center}

Following horizontal displacement, we studied the effect of vertical displacement of a person from the camera center (\autoref{fig:corr_analysis}; 4th col.).
The vertical displacement was quantified as a vertical angle, $\theta\degree_V$, of the person captured from the camera center that is normalized by vertical field-of-view, $\theta\degree_{V_{FOV}}$, referring to the camera, namely normalized vertical angle, $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$.
We specifically consider the foot location, which we use to localize, as a point of reference to calculate the normalized vertical angle.
As shown in \autoref{fig:corr_analysis} (4th col., 1 row), when the person is closer to the camera, the normalized vertical angle increases and only the upper body is partially captured by the camera due to the limited vertical field-of-view.
In our analysis, the foot locations of people with $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \geq 0.8$ were not captured sufficiently, and the pose estimation model could not detect the person.
On the other hand, as the person moves further from the camera, the normalized vertical angle decreases and can capture the full body in the field of view, but with the cost of increased distance between the camera and the person.
For $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$ close to zero, localization and body orientation error increased significantly, with the increased distance between the captured person and the camera.
On the whole, as the person approached the vertical camera center for greater coverage of more body parts, localization and orientation errors decreased with a strong negative correlation, $R=-0.495 (p<0.005)$ and $R=-0.317 (p<0.005)$, respectively.
The optimal range of normalized vertical angle was between $0.05\leq \sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \leq 0.2$, which were equivalent of $6m$ to $23m$ distance between the captured person and the camera, which draws a similar conclusion from camera distance analysis earlier.

\subsection{Limitations}

Overall, our pipeline was capable of reliably localizing people ($1.4m$ error), tracking people (62.0\% MOTA), and estimating body orientation (28.97\degree). 
But, our evaluation is with limited precision in our ground truth annotation.
The precision of our ground truth location is $2m$, and orientation is $45\degree$.
As noted earlier, the location of people in the space was mapped to the closest 1-meter marker. 
Additionally, we discovered structural differences of around $1.5m$ from the building blueprint, which we used to develop our localization model.
Nevertheless, we considered a margin of 2 meters of localization error sufficient for tracking participant behavior at our study site for our future applications.
For body orientation annotation, it was difficult to have participants turn exactly in $5\degree \sim 10\degree$ intervals.
Regardless, we consider an error range within $45\degree$ is reasonable to identify the facing of the people in the space while having group interactions.
The normal horizontal field-of-view of the human eye is about 135\degree, and our system can detect dyadic interactions from overlapping field-of-view between two people with at most $90\degree$ margin of error. 
% \chaitra{Is it a good idea to leave out details like this about future applications so that people don't steal our ideas?}\hyeok{Yes. It is okay. Do not be too afraid of others' stealing ideas.}
In our model, the body orientation MAE was 28.97\degree overall, which was well within the $45\degree$ margin of error.

The spaces that were not covered in our evaluation are filled with tables, yoga mats, or gym equipment that were used for various activities.
Future studies will examine how complex movements and occlusions affect our tracking and body orientation estimation methods when people interact with those furniture and equipments.
% We are currently collecting social interaction activities across the study site throughout the day as part of our ongoing study. \chaitra{Is this line necessary?}\hyeok{Nope. Removed}
Despite these limitations in our evaluation, the proposed work shows promise as an initial step toward analyzing complex movements in open spaces.

\subsection{Future Applications}

\hyeok{Cut it down.}

Low-cost, privacy-preserving, and passive monitoring system with distributed camera network has several applications for objectively quantifying individual and group activities.
For multiple people to be monitored in a privacy-preserving manner, our system does not require special fabrication or expensive equipment.
This provides an opportunity to monitor, transform, and test the space design in an efficient way with large-scale studies.

% \chaitra{I feel like we can shorten this section and don't have to go into details. I personally think that we would be giving away good ideas (as I mentioned in a previous comment) if we go into details. I will write a shorter version of this section this week to get all yours thoughts on it.} \hyeok{Chaitra, please come up with your version and we can discuss it.} \hyeok{We will shorten this down anyway, due to Gari's request.}

\subsubsection{Clinical Application}

The movement of people living with neurodegenerative disorders, such as Alzheimer's disease, is affected by cognitive impairment and dementia~\cite{bahureksa2017impact}.
In the early stage of cognitive impairment, namely Mild Cognitive Impairment (MCI), patients start to show gait patterns that deviate from neurotypical populations. \chaitra{note for myself: insert citation}
When people living with MCI gradually lose spatial and temporal awareness, they wander, where they get confused about their location and become lost while walking~\cite{jeong2016relationship,neubauer2018we}.
In addition, patients are likely to isolate themselves and refrain from social activities~\cite{khan2023sensor}, leading to a high risk of mental health problems, such as depression~\cite{zafar2021loneliness}.
It is, therefore, vital to monitor elders' movement and social interaction characteristics to detect early cognitive impairment risks and provide appropriate interventions.
Our system allows continuous and objective assessment of gait, wandering, and group activities.
% With our system, large spaces in assisted living institutions or nursing homes can be transformed into smart spaces without expert hardware fabrication, allowing for continuous and objective assessment of gait, wandering, and group activities.
We can continuously collect 2D pose and spatial movement information throughout the day by installing low-cost Raspberry Pis in existing infrastructure.
The future work will further enable a system that can predict falling episodes in real-time, thereby preventing a severe outcome, by directly utilizing 2D poses from multi-view cameras across the facility~\cite{lach2017falls,allali2017management}.
In addition, particularly in the era of pandemics and among immunocompromised populations, monitoring detailed movements and trajectories of multiple people is important in order to intervene for appropriate social distancing monitoring to prevent disease contamination due to crowding in indoor spaces~\cite{hegde2022modeling}.

\subsubsection{Design of Patient-centered Environments}

{
Our system supports patient-centered research and design, not only for individuals living with MCI but also for any context that needs a deep understanding of human behavior in the built environment. 
Still, there are unique contributions of our system to the (re)design of the space where this study was developed.
Designing healthcare facilities for individuals living with MCI poses challenges for architects as it requires unique design considerations that differ from those for cognitively healthy older adults and dementia patients~\cite{challenge_arch_2020}. 
While people with MCI also experience cognitive decline, their condition is less debilitating than that of dementia patients~\cite{Gauthier2006_classic}.
The 18000+ square feet space in this study was a one-of-a-kind project designed based on a series of goals, such as promoting social interaction, environmental exploration, spatial flexibility, safety, independent learning of everyday tasks (e.g., cooking), contact with nature, exercise, and cognitive stimulation. 
The designed spaces were adjustable and equipped with technologies, such as tunable lighting and controllable zone-based sound systems, to experiment with achieving these goals. 
Our system allows for the identification of individuals' postures, locations, and duration of engagement in various activities at all times while maintaining their privacy. 
This capability supports architects in (re)designing environments that align with their objectives, as mentioned earlier, not only for this specific space. 
In this case, valuable design improvement feedback can be drawn from conclusions such as the areas around the kitchen and dining spaces encouraging more extended standing interaction among larger groups of people than the lounge areas.}

\subsubsection{Workspace Design}

Multi-person monitoring can revolutionize the design of a workplace by allowing the designer to take into account the fine-grained movements of multiple people in the space.
Social interactions at work, which are highly correlated with productivity and well-being, are influenced by workplace design~\cite{lee2019empirical}.
Our system can provide detailed information on socio-spatial formation patterns, such as space occupancy, behavioral mapping~\cite{cox2018understanding}, Proxemics (physical distance between the people)~\cite{ballendat2010proxemic,hall1963system}, F-formation (shape and size of group formation)~\cite{danninger2005using,kendon1990spatial}.
For large indoor spaces with a large number of people having different social dynamics, understanding those patterns longitudinally can provide localized and personalized design principles to best serve various purposes of space use through furniture layouts and interior elements in highly collaborative spaces like our study centers.
{In healthcare settings, space and furniture layout can play a critical role not only in promoting collaboration and socialization but also in preventing behavior-related issues among healthcare workers, such as contamination by infectious diseases~\cite{contamination1}.
Addressing these issues has the potential to greatly improve treatment outcomes~\cite{treatmentoutcomes}. 
Nonetheless, initial design concepts frequently lack crucial design elements that can help prevent such mistakes. 
This often occurs despite the existence of a wealth of knowledge on known risks and prevention strategies~\cite{missingindesign}.
In the particular space where our study was conducted, specific design goals and standards were established beforehand. Despite these guidelines, all designs are prone to flaws. Fortunately, our system can provide information on how individuals interact within the space to foster project improvement.}

{In summary, our system is valuable for mapping behaviors within healthcare facilities. A comprehensive approach to facility design is necessary, which includes considering not only physical aspects, but also the flow of patients and staff, as well as resource allocation. By taking these factors into account, healthcare facilities can better meet the needs of their patients and staff, while also enhancing the quality of care they provide.}

==> sections/discussion/_main_chaitra_20231029.tex <==
\section{Discussion}

Our analysis demonstrated that our pipeline was capable of reliably localizing people ($1.4m$ error), tracking people ($62.0\sim88.6\%$ MOTA), and estimating body orientation (28.97\degree). 
In this section, we discuss the limitation and potential applications of the proposed method that can largely benefit from our low-cost and privacy-preserving monitoring system using distributed camera networks.

\subsection{Limitations}

% The ground truth annotation of the datasets discussed in \ref{sec:benchmark_data_collection} have an average location accuracy of $2m$ and average orientation accuracy of $45\degree$.
As noted earlier, the location of people in the space was mapped to the closest 1-meter marker, which is sufficient resolution considering the varying foot sizes of people. 
Additionally, we discovered structural differences of around $1.5m$ from the building blueprint, which was used to develop our localization model.
Nevertheless, we considered a margin of 2 meters of localization error as sufficient for tracking participant behavior at our study site for our future applications.
For body orientation annotation, it was difficult to have participants turn exactly in $5\degree \sim 10\degree$ intervals.
Regardless, we consider an error range within $45\degree$ is reasonable to identify the facing orientation of people in the study space while having group interactions.
The normal horizontal field-of-view of the human eye is about 135\degree, and our system can detect dyadic interactions from overlapping field-of-view between two people with at most $90\degree$ margin of error. 
In our model, the body orientation MAE was $28.97\degree$ overall, which was well within the $45\degree$ margin of error.

The areas in the study space that were not covered in our evaluation are filled with tables, yoga mats, or gym equipment that were used for various activities.
Future studies will examine how complex movements and occlusions affect our tracking and body orientation estimation methods when people interact with those furniture and equipments.
Despite these limitations in our evaluation, the proposed work shows promise as an initial step towards analyzing complex movements in open spaces.

\subsection{Future Applications}

Our system allows for the identification of individuals' postures, locations, and duration of engagement in various activities at all times while maintaining their privacy. 
This provides an opportunity for several applications based on objectively quantifying individual and group activities.

\subsubsection{Clinical Application}

Our system can be used to understand behavior and potentially detect behavioral changes of individuals with various neurological or mental impairments. In the future, it could also be used to detect certain mental disorders.
For example, in the early stages of cognitive impairment, namely Mild Cognitive Impairment (MCI), patients start to show gait patterns that deviate from neurotypical populations ~\cite{LINDHRENGIFO202283} ~\cite{de2017gait}. 
It is, therefore, vital to monitor elders' movement characteristics to detect early cognitive impairment risks and provide appropriate interventions.
Our system allows continuous and objective assessment of gait, wandering, and group activities.
We can continuously collect 2D pose and spatial movement information throughout the day by installing low-cost edge computing systems in existing infrastructure.
The future work will further enable a system that can predict falling episodes in real-time, thereby preventing a severe outcome, by directly utilizing 2D poses from multi-view cameras across the facility~\cite{lach2017falls,allali2017management}.

\subsubsection{Design of Patient-centered Environments}

Our system supports patient-centered research and design, not only for individuals living with MCI but also for any context that needs a deep understanding of human behavior in the built environment. 
This capability supports architects in (re)designing environments that align with their objectives, as mentioned earlier, not only for this specific space. 
In this case, valuable design improvement feedback can be drawn from conclusions such as the areas around the kitchen and dining spaces encouraging more extended standing interaction among larger groups of people than the lounge areas.

\subsubsection{Workspace Design}

Multi-person monitoring can revolutionize the design of a workplace by allowing the designer to take into account the fine-grained movements of multiple people in the space.
Social interactions at work, which are highly correlated with productivity and well-being, are influenced by workplace design~\cite{lee2019empirical}.
Our system can provide detailed information on socio-spatial formation patterns, such as space occupancy, behavioral mapping~\cite{cox2018understanding}, Proxemics (physical distance between the people)~\cite{ballendat2010proxemic,hall1963system}, F-formation (shape and size of group formation)~\cite{danninger2005using,kendon1990spatial}.
For large indoor spaces with a large number of people having different social dynamics, understanding those patterns longitudinally can provide localized and personalized design principles to best serve various purposes of space use through furniture layouts and interior elements in highly collaborative spaces like our study centers.

In summary, our system is valuable for mapping behaviors within healthcare facilities. A comprehensive approach to facility design is necessary, which includes considering not only physical aspects, but also the flow of patients and staff, as well as resource allocation. By taking these factors into account, healthcare facilities can better meet the needs of their patients and staff, while also enhancing the quality of care they provide.

==> sections/discussion/_main_old.tex <==
\section{Discussion}

Our analysis demonstrated that our pipeline was capable of reliably localizing people ($1.4m$ error), tracking people (62.0\% MOTA), and estimating body orientation (28.97\degree). 
With this success, we discuss the limitation and potential applications of the proposed method that can largely benefit from our low-cost and privacy-preserving monitoring system using distributed camera networks.

\subsection{Limitations}

% Our ground truth annotation had a certain degree of limited precisions.
The precision of our ground truth location is $2m$, and orientation is $45\degree$.
As noted earlier, the location of people in the space was mapped to the closest 1-meter marker. 
Additionally, we discovered structural differences of around $1.5m$ from the building blueprint, which we still had to rely on to develop our localization model.
Nevertheless, we considered a margin of 2 meters of localization error sufficient for tracking participant behavior at our study site for our future applications.
For body orientation annotation, it was difficult to have participants turn exactly in $5\degree \sim 10\degree$ intervals.
Regardless, we consider an error range within $45\degree$ is reasonable to identify the facing of the people in the space while having group interactions.
The normal horizontal field-of-view of the human eye is about 135\degree, and our system can detect dyadic interactions from overlapping field-of-view between two people with at most $90\degree$ margin of error. 
% \chaitra{Is it a good idea to leave out details like this about future applications so that people don't steal our ideas?}\hyeok{Yes. It is okay. Do not be too afraid of others' stealing ideas.}
In our model, the body orientation MAE was 28.97\degree overall, which was well within the $45\degree$ margin of error.

The spaces that were not covered in our evaluation are filled with tables, yoga mats, or gym equipment that were used for various activities.
Future studies will examine how complex movements and occlusions affect our tracking and body orientation estimation methods when people interact with those furniture and equipments.
% We are currently collecting social interaction activities across the study site throughout the day as part of our ongoing study. \chaitra{Is this line necessary?}\hyeok{Nope. Removed}
Despite these limitations in our evaluation, the proposed work shows promise as an initial step toward analyzing complex movements in open spaces.

\subsection{Future Applications}

% \hyeok{Cut it down.}

Our system allows for the identification of individuals' postures, locations, and duration of engagement in various activities at all times while maintaining their privacy. 
This provides an opportunity for several applications based on objectively quantifying individual and group activities.
% For multiple people to be monitored in a privacy-preserving manner, our system does not require special fabrication or expensive equipment.

% \chaitra{I feel like we can shorten this section and don't have to go into details. I personally think that we would be giving away good ideas (as I mentioned in a previous comment) if we go into details. I will write a shorter version of this section this week to get all yours thoughts on it.} \hyeok{Chaitra, please come up with your version and we can discuss it.} \hyeok{We will shorten this down anyway, due to Gari's request.}

\subsubsection{Clinical Application}

% The movement of people living with neurodegenerative disorders, such as Alzheimer's disease, is affected by cognitive impairment and dementia~\cite{bahureksa2017impact}.
In the early stage of cognitive impairment, namely Mild Cognitive Impairment (MCI), patients start to show gait patterns that deviate from neurotypical populations. 
% \chaitra{note for myself: insert citation} \hyeok{I will remove this, as no further action was taken.}
% When people living with MCI gradually lose spatial and temporal awareness, they wander, where they get confused about their location and become lost while walking~\cite{jeong2016relationship,neubauer2018we}.
% In addition, patients are likely to isolate themselves and refrain from social activities~\cite{khan2023sensor}, leading to a high risk of mental health problems, such as depression~\cite{zafar2021loneliness}.
It is, therefore, vital to monitor elders' movement characteristics to detect early cognitive impairment risks and provide appropriate interventions.
Our system allows continuous and objective assessment of gait, wandering, and group activities.
% With our system, large spaces in assisted living institutions or nursing homes can be transformed into smart spaces without expert hardware fabrication, allowing for continuous and objective assessment of gait, wandering, and group activities.
We can continuously collect 2D pose and spatial movement information throughout the day by installing low-cost Raspberry Pis in existing infrastructure.
The future work will further enable a system that can predict falling episodes in real-time, thereby preventing a severe outcome, by directly utilizing 2D poses from multi-view cameras across the facility~\cite{lach2017falls,allali2017management}.
% In addition, particularly in the era of pandemics and among immunocompromised populations, monitoring detailed movements and trajectories of multiple people is important in order to intervene for appropriate social distancing monitoring to prevent disease contamination due to crowding in indoor spaces~\cite{hegde2022modeling}.

\subsubsection{Design of Patient-centered Environments}

Our system supports patient-centered research and design, not only for individuals living with MCI but also for any context that needs a deep understanding of human behavior in the built environment. 
% Still, there are unique contributions of our system to the (re)design of the space where this study was developed.
This capability supports architects in (re)designing environments that align with their objectives, as mentioned earlier, not only for this specific space. 
In this case, valuable design improvement feedback can be drawn from conclusions such as the areas around the kitchen and dining spaces encouraging more extended standing interaction among larger groups of people than the lounge areas.

\subsubsection{Workspace Design}

Multi-person monitoring can revolutionize the design of a workplace by allowing the designer to take into account the fine-grained movements of multiple people in the space.
Social interactions at work, which are highly correlated with productivity and well-being, are influenced by workplace design~\cite{lee2019empirical}.
Our system can provide detailed information on socio-spatial formation patterns, such as space occupancy, behavioral mapping~\cite{cox2018understanding}, Proxemics (physical distance between the people)~\cite{ballendat2010proxemic,hall1963system}, F-formation (shape and size of group formation)~\cite{danninger2005using,kendon1990spatial}.
For large indoor spaces with a large number of people having different social dynamics, understanding those patterns longitudinally can provide localized and personalized design principles to best serve various purposes of space use through furniture layouts and interior elements in highly collaborative spaces like our study centers.
% In healthcare settings, space and furniture layout can play a critical role not only in promoting collaboration and socialization but also in preventing behavior-related issues among healthcare workers, such as contamination by infectious diseases~\cite{contamination1}.
% Addressing these issues has the potential to greatly improve treatment outcomes~\cite{treatmentoutcomes}. 
% Nonetheless, initial design concepts frequently lack crucial design elements that can help prevent such mistakes. 
% This often occurs despite the existence of a wealth of knowledge on known risks and prevention strategies~\cite{missingindesign}.
% In the particular space where our study was conducted, specific design goals and standards were established beforehand. Despite these guidelines, all designs are prone to flaws. Fortunately, our system can provide information on how individuals interact within the space to foster project improvement.

In summary, our system is valuable for mapping behaviors within healthcare facilities. A comprehensive approach to facility design is necessary, which includes considering not only physical aspects, but also the flow of patients and staff, as well as resource allocation. By taking these factors into account, healthcare facilities can better meet the needs of their patients and staff, while also enhancing the quality of care they provide.

==> sections/discussion/main.tex <==
\section{Discussion}

\revision{
Our experiment results demonstrated the possibility of using edge computing devices and cameras to continuously monitor fine-grained activities across large indoor spaces.}
% In this section, we discuss the limitations and potential applications of our systems that can largely benefit from our low-cost and privacy-preserving monitoring system.

\subsection{Multi-person Tracking and Localization}

\subsubsection{4 People Walking around Entire Space}

\revision{
Overall evaluation shows that the proposed model can consistently track people over the sequence if the person is detected,
and can also handle certain degree of missing detections (FNs) coming from the limitations in the multi-person pose detection model on edge computing systems.
To run the pose detection model on edge computing system, a resource-constrained device, we are currently using the model that is specifically tailored to emphasize efficiency over performance compared to the state-of-the-art models~\cite{dos2021monocular}. 
This was also reflected in high Precision (93.48\%), high MT (1.83), and low ML (0.33).
The overall localization performance was within a reasonable error range, as our tracking rate is 1 Hz and people normally walk $1.42m/s$ in everyday activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
Also, the precision of our ground truth annotations have a margin of 1-meter error as the participants' locations were labeled as the closest 1-meter interval marker in the space.
}

\revision{
The performance of the model varied depending on the areas in the study space.
For the Activity area (A), where most physical activity happens in the study site, MOTA score was 88.63\%, and MOTP was $1.38m$ with high Precision (95.6\%) and Recall (93.62\%), which is sufficient to detect, track and understand group activity and space usage behavior in this area.
In the Activity Area (A), seven cameras were tracking movements and this shows that the multi-view camera is especially important when detections are noisy, as overlapping viewpoints help to capture people from the front, back, and side while walking, as shown in \autoref{fig:camera_config}. 
The lower MOTA was observed when only a few (two or three) cameras were available to cover the wide capture space.
Kitchen, Left Corridor, or Right Corridor had 67.16\%, 54.53\%, 60.25\% MOTA and $1.48m$, $1.92m$, and $1.75m$ MOTP, respectively.
The Kitchen, Left Corridor, and Right Corridor had long corridors, which are $24m\times 3m$, $33m\times 2m$, and $33m\times 1.5m$, respectively.
Having few cameras for those regions to capture people from far was severely hampered by the occlusion and challenges in detecting poses, due to too small pixel region for each person, resulting in high FNRs (1.01, 1.53, 1.56, respectively). 
However, our system still showed high Precision (95.6\%, 91.3\%, 100\%) in those regions, showing that detected objects are mostly correctly localized.
}

\revision{
Staff Zone has four cameras installed to capture movements from the sides (left and right) while walking.
The size of the staff zone ($14m\times 3m$) is the smallest compared to other areas, which also makes cameras capture people closer in the distance.
This resulted in a higher MOTA score (73.47\%) with a lower MOTP score ($1.11m$) and lower FNRs (0.40) compared to other areas.
The Lounge area only has one camera covering the space and had the lowest performance with a MOTA score of 33.44\%. 
This was mainly due to the shortage of power and network source near the lounge area, where only a single camera was available to cover the entire space. Additionally, there are occlusions from the front desk, chairs, and other items.
In summary, our experiment results show that multi-view cameras with closer distances to people are important to address challenges for noisy pose estimations in edge computing devices low MOTP and high MOTA scores.
}

\subsubsection{5 People Walking Past Each Other}
\revision{
Our results demonstrate that having four multi-view cameras capturing the activities from different views could compensate for occlusions while people actively move, although with noisy or missing pose estimations while subjects move.
}

\subsection{Body Orientation Estimation}

\subsubsection{4 People Walking around Entire Space}

\revision{
The body-orientation estimation performance was sufficient to tell eight (N, NE, E, SE, S, SW, W, NW) orientations reliably. 
Similar to the localization and tracking, the performance of orientation estimation varied across the study space, depending on the captured area size and the overlaps in multi-view cameras covering the space.
Activity Area (\autoref{tab:orientation}, 1st row), having seven cameras from the front, back, and sides with the most overlapping views, had errors showing 25.91$\degree$ MAE, and, Staff Zone (\autoref{tab:orientation}, 6th row) also had comparably lower MAE (32.41\degree) as this area has four cameras installed with overlapping field-of-views with close distance to people.
Left and Right Corridors (\autoref{tab:orientation}, 3rd and 5th rows), where low MOTA score was observed, surprisingly had low errors as well, 21.68$\degree$ and 32.41$\degree$ MAEs, respectively.
These areas had challenges in localization and tracking due to lower number of cameras covering the narrow and long distances.
But, for body orientation estimation, due to the narrow width of the corridor, it was easy for the model to estimate body orientations from human bounding box images since people tend to face forward or opposite to the camera viewpoints when they are moving. 
For the Lounge area (\autoref{tab:orientation}, 4th rows), where only a single camera is covering the space, it was very difficult to identify body orientations, with 47.37\degree\; MAE and Acc.-45\degree\; of 55.4\%, due to the occlusions from objects in the space. 
This analysis shows that the instrumentation of camera placement is a dependent variable of the space structure, as only a few (1 or 2) cameras were sufficient for narrow corridors to cover linear movements, whereas multi-view cameras are more recommended for open spaces to take account for complex and free wandering.
}

\subsubsection{5 People Walking Past Each other}

\revision{
Overall, the body orientation estimation model was significantly confused by the occlusions between people.
Yet, Acc.-90\degree showed 81.4\%, where our model can identify four equally spaced cardinal directions (N, E, S, W) at minimum, even when people are closely located together and dynamically changing group formations.
These findings provide a baseline for group activity analysis in a crowded area, as understanding group activity requires finding group formation and facing directions while moving.
}

\subsubsection{5 people Changing Orientations in Place}

\revision{
When evaluating this scenario, the model was able to identify equally spaced four directions (N, E, S, W) at minimum, showing Acc.-90\degree of 69.3\%.
% the model demonstrated a significant error rate (\autoref{tab:orientation}, last row), in which MAE was 63.4\degree.
% Similarly, in the five-person experiment, the model was able to identify equally spaced four directions (N, E, S, W) at minimum, showing Acc.-90\degree of 69.3\%.
Likewise in the previous experiment, the major source of error was coming from the occlusions between people close in the distance, capturing multiple people in a human bounding box.
Furthermore, our body orientation estimation model found it difficult to detect slight changes ($5\degree\sim 10\degree$) in facing direction between subsequent frames, as the model makes frame-by-frame estimation.
This also shows that our model performed better when people were walking as our multi-person tracking method updates the orientation information with moving directions.
}

\revision{
The accuracy of each session also showed differences according to the number of cameras and the size of captured areas covered by those cameras.
Session 1 (\autoref{tab:orientation}, 9th row), where three cameras were covering $55m^2$ space, showed an MAE of 73.7\degree, although the samples only had small size groups having two or three members.
The MAE (65.2\degree) was lower in Session 2 (\autoref{tab:orientation}, 10th row), where members had a group size of four, but the capture area ($28m^2$) was smaller than that of Session 1, clearly demonstrating the importance of multi-view cameras.
This was more apparent for Session 3 (\autoref{tab:orientation}, 11th row), which has a social group size of 5 people, but with the lowest MAE (50.4\degree) amongst all three sessions.
The capture space was only $15m^2$ and four cameras were available.
}

\subsection{Impact of Parameters of Camera Installation}

% \revision{In our experiment results, we observed that the placement of cameras has high correlation with the localization and orientation estimation accuracy.
% Here, we quantify this in more detail to understand the impact of four different factors of camera installation related to localization and body orientation estimation accuracy.
% }

\subsubsection{Distance Between Camera and Person}

\revision{
The majority of our samples were within $\sim2$ meters and $25\degree$ error, respectively for localization and orientation error, when the the distance between the person and camera was within 15 meters.
This shows that, for edge computing cameras, the pixel region that constitutes the person decreases significantly if the person is farther than 15 meters. 
% the edge computing camera (Sony IMX219 8-megapixel sensor) can capture objects well within 15 meters, which is large enough for our pose estimation and body orientation estimation models to make accurate predictions.
% As a result of the person being further away from the camera, the pixel region that constitutes the person decreases significantly, which increases the errors in body orientation and localization.
The models were more confused when people were occluding each other, as multiple people looked like a single person from a distance.
Also, pose estimation models confused frontal and rear views of the person many times, especially when the person was farther than $20m$ from the camera, resulting in unrealistically twisted keypoints.
}

\subsubsection{Facing Angle with Respect to Camera Viewpoint}

\revision{
The facing direction of the captured person had a significant impact on the accuracy of both localization and body orientation estimation.
Facing angles within $50\degree$ of the camera line-of-sight were found to be crucial to ensuring a $<2m$ localization error and a $<25\degree$ body orientation error.
Specifically, the 2D pose estimation model performed best when the person was facing the camera with higher confidence in estimations.
}

\subsubsection{Horizontal Displacement from Camera Center}

\revision{
A person must be captured within 30\% of the horizontal field of view 
% \chaitra{What is horizontal camera displacement?}\hyeok{I updated this to horizontal field of view}
to have a localization error of less than $2m$ and an orientation error of less than 25\degree. 
When the person is captured closer to the frame boundaries, the lens distortion in the edge computing camera violates the planar assumption of floor and degrades the projective transformation (Sec.~\ref{sec:indoor_localization}), which significantly increases the localization error.
Also, orientation estimation error increases as subjects are only partially captured in the frame boundaries.
}

\subsubsection{Vertical Displacement from Camera Center}

\revision{
Shown in \autoref{fig:corr_analysis} (4th col.), with our edge computing camera module, the foot locations of people with $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \geq 0.8$ were not captured sufficiently, and the pose estimation model could not detect the person.
For $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$ closer to zero, localization and body orientation error increased significantly, with the increased distance between the captured person and the camera.
The optimal range of normalized vertical angle was between $0.05\leq \sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \leq 0.2$, which were equivalent of $6m$ to $23m$ distance between the captured person and the camera, which draws a similar conclusion from camera horizontal distance analysis above.
}

\subsection{Limitations}

% The ground truth annotation of the datasets discussed in \ref{sec:benchmark_data_collection} have an average location accuracy of $2m$ and average orientation accuracy of $45\degree$.
% As noted earlier, the location of people in the space was mapped to the closest 1-meter marker, which is sufficient resolution considering the varying foot sizes of people. 
We discovered structural differences of around $1.5m$ from the building blueprint, which was used to develop our localization model in Sec.~\ref{sec:indoor_localization}.
Nevertheless, we considered a margin of 2 meters of localization error as sufficient for tracking participant behavior at our study site for our future applications.
For body orientation annotation, it was difficult to have participants turn exactly in $5\degree \sim 10\degree$ intervals.
Regardless, we consider an error range within $45\degree$ to be reasonable for tracking social interactions while our subjects having group activities.
The normal horizontal field-of-view of the human eye is about 135\degree, and our system can detect dyadic interactions from overlapping field-of-view between two people with at most $90\degree$ margin of error. 
In our analysis, the body orientation MAE was $28.97\degree$ overall, which was well within the $45\degree$ margin of error.

The areas that were not covered in our evaluation are filled with tables, yoga mats, or gym equipment.
Future studies will examine how complex movements and occlusions affect our tracking and body orientation estimation methods when people interact with those furniture and equipment.
\revision{
Despite these limitations in our evaluation, the proposed work shows promise as an initial step towards analyzing complex movements in open spaces using a privacy-preserving camera-based activity monitoring system using secure edge computing framework.
}

\subsection{Future Applications}

% Our system allows for the identification of individuals' postures, locations, and duration of engagement in various activities at all times while maintaining their privacy. 
% This provides an opportunity for several applications based on objectively quantifying individual and group activities.
\revision{
\noindent \textit{Clinical Application:}
Our system allows continuous and objective assessment of gait, wandering, and group activities.
Our system can be used to understand behavior and potentially detect behavioral changes in individuals with various neurological or mental impairments~\cite{LINDHRENGIFO202283}. 
The future work will further enable a system that can predict falling episodes in real-time, thereby preventing a severe outcome, by directly utilizing 2D poses from multi-view cameras across the facility~\cite{lach2017falls,allali2017management}.
}

\revision{
\noindent \textit{Workspace Design:}
Social interactions at work, which are highly correlated with productivity and well-being, are influenced by workplace design~\cite{lee2019empirical}.
Our system can provide detailed information on socio-spatial formation patterns, such as space occupancy, behavioral mapping~\cite{cox2018understanding}, Proxemics (physical distance between the people)~\cite{ballendat2010proxemic,hall1963system}, F-formation (shape and size of group formation)~\cite{danninger2005using,kendon1990spatial}, which allows the designer to take into account to design the workplace.
}

%-------

% \subsubsection{Clinical Application}

% Our system can be used to understand behavior and potentially detect behavioral changes of individuals with various neurological or mental impairments. In the future, it could also be used to detect certain mental disorders.
% For example, in the early stages of cognitive impairment, namely Mild Cognitive Impairment (MCI), patients start to show gait patterns that deviate from neurotypical populations ~\cite{LINDHRENGIFO202283} ~\cite{de2017gait}. 
% It is, therefore, vital to monitor elders' movement characteristics to detect early cognitive impairment risks and provide appropriate interventions.
% Our system allows continuous and objective assessment of gait, wandering, and group activities.
% We can continuously collect 2D pose and spatial movement information throughout the day by installing low-cost edge computing systems in existing infrastructure.
% The future work will further enable a system that can predict falling episodes in real-time, thereby preventing a severe outcome, by directly utilizing 2D poses from multi-view cameras across the facility~\cite{lach2017falls,allali2017management}.

% \subsubsection{Design of Patient-centered Environments}

% Our system supports patient-centered research and design, not only for individuals living with MCI but also for any context that needs a deep understanding of human behavior in the built environment. 
% This capability supports architects in (re)designing environments that align with their objectives, as mentioned earlier, not only for this specific space. 
% In this case, valuable design improvement feedback can be drawn from conclusions such as the areas around the kitchen and dining spaces encouraging more extended standing interaction among larger groups of people than the lounge areas.

% \subsubsection{Workspace Design}

% Multi-person monitoring can revolutionize the design of a workplace by allowing the designer to take into account the fine-grained movements of multiple people in the space.
% Social interactions at work, which are highly correlated with productivity and well-being, are influenced by workplace design~\cite{lee2019empirical}.
% Our system can provide detailed information on socio-spatial formation patterns, such as space occupancy, behavioral mapping~\cite{cox2018understanding}, Proxemics (physical distance between the people)~\cite{ballendat2010proxemic,hall1963system}, F-formation (shape and size of group formation)~\cite{danninger2005using,kendon1990spatial}.
% For large indoor spaces with a large number of people having different social dynamics, understanding those patterns longitudinally can provide localized and personalized design principles to best serve various purposes of space use through furniture layouts and interior elements in highly collaborative spaces like our study centers.

% In summary, our system is valuable for mapping behaviors within healthcare facilities. A comprehensive approach to facility design is necessary, which includes considering not only physical aspects, but also the flow of patients and staff, as well as resource allocation. By taking these factors into account, healthcare facilities can better meet the needs of their patients and staff, while also enhancing the quality of care they provide.

==> sections/experiment/main.tex <==
\section{Experiment}

% Everything is moved to ../method/main.tex for \section{Method \& Materials}


==> sections/experiment/main_20230329.tex <==
\section{Experiment}

\subsection{Benchmark Data Collection}\label{sec:benchmark_data_collection}

\input{figure/ep6_func_spaces.tex}

\input{figure/data_collection.tex}

Our study site has 18,286 square feet of space and is designed to have different functioning spaces, including a library, kitchen, dining area, gym, and so on, as shown in \autoref{fig:ep6_func}.
Our benchmark dataset has four to five people walking in the study site.
To accurately annotate the location and timing of the people, we taped the entire space with 1-meter markers. 
Participants were asked to walk according to the instructed group formation and walking paths.
While people were walking, an observer was annotating the exact timing and location of people at each second.
The body orientation of people was also manually annotated by the observer using the north (upper direction for \autoref{fig:ep6_func}) as a reference.

\autoref{fig:data_collection} describes the locations and formation of groups taken by participants while collecting benchmark datasets to consider the realistic use cases of the study site by visitors.
For the benchmark dataset, we have covered areas that are of interest for tracking behaviors in the study space (\autoref{fig:data_collection}, a). 
Those include locations mainly used by the visitors for eating (dining, kitchen), physical exercises, lounge, and staff zones (\autoref{fig:ep6_func}), where participants agreed to their behaviors being captured.
For the annotation, we selected the closest 1-meter markers as ground-truth locations of the participants while they were walking, considering the varying foot size and stride length of each participant.

While walking, we changed the group formation as well to simulate realistic movement in the space (\autoref{fig:data_collection}, b).
For the wider corridors, group formations of two or three people walking side-by-side were used.
Otherwise, multiple people were walking in straight lines. Walking in groups helped to test the effect of occlusions, where people are not seen from a camera viewpoint.
For the seating areas, we have also asked participants to sit naturally as they communicate with one another.
As shown in \autoref{fig:camera_config}, (a), some locations, such as kitchen or staff areas, are covered by multiple cameras, and other locations, such as long corridors, are covered by single or two cameras.
As discussed earlier, the camera was installed at locations with accessible power and network sources using extension cables in the existing infrastructure of the building above the ceiling.


\subsection{Multi-person Tracking Baseline}

\subsubsection{Hungarian matching-base tracking}
% \yash{did we find baseline for multi-view position estimation by simply averaging the estimated location by each camera?}\hyeok{I have it in one of my experiments. But, didn't include in the paper due to page length and due to the lesser importance compared to the baselines in the paper.}
Our proposed tracker is compared with a Hungarian matching-based tracker~\cite{kuhn1955hungarian}, which only considers frame-by-frame matching between 2D pose detections, in order to illustrate the importance of modeling temporal dynamics of 2D movements.
Based on the results of multiview multi-person localization at time $t$ and $t+1$, the Hungarian tracker generates a bipartite graph with nodes representing samples from two consecutive timesteps and edges representing Euclidean distances between samples. 
Since our tracking rate is 1 Hz, we remove any edge distance larger than 1.5 meters in the created bipartite graph, as people normally walk 1.42 m/s in everyday activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
Then, the Hungarian method finds the matchings (or edges) that have a minimum sum of Euclidean distances.
Potentially missing samples (false negatives) in a frame $t$ are filled in by linearly interpolating the matched detection from frame $t-1$ and $t+1$.
The Hungarian matching is applied until no matching is found any longer along the time.

\subsection{Body Orientation Estimation Baseline}

Our body orientation method inherently learns the geometric relationship between 2D pose, 3D pose, and the corresponding body orientation of the observed human bounding box.
We compare the proposed method with two baselines that only use 2D information and then a baseline that only models the 3D geometry of detected 2D poses.
Through this practice, we will demonstrate the importance of modeling both 3D geometry and pose-body orientation relationships.

\subsubsection{2D pose-based Heuristic Approach}

This method uses a heuristic approach to estimate body orientation from only 2D pose information.
Specifically, it uses 2D facial keypoints, including nose, eyes, and ears, and estimates the 2D vector originating from the average of left and right eyes and ears keypoints to nose keypoints on 2D image pixels.
We directly project those 2D vectors from the image frame to the 2D coordinate space of the study site using a perspective transformation matrix, $M$, derived from \autoref{eqn:perspective_mat}.

\subsubsection{2D pose-based Deep Learning Approach}

This baseline model applied a learning-based method, where the model directly estimates body orientation from 2D pose input.
We used a graphical convolutional network (GCN)~\cite{yan2018spatial} to process 2D pose data to predict body orientation angle in 5-\degree intervals.
For training the model, we used MS COCO 2D keypoints~\cite{lin2014microsoft} dataset and the corresponding body orientation annotation provided by  Wu~\etal~\cite{wu2020mebow}.
We augmented 2D keypoints input by randomly flipping horizontally or adding Gaussian noises to simulate noisy pose detections from our pipeline.

\subsubsection{2D-3D pose Geometric matching-based Approach}

To model the 3D geometry of the human body pose~\cite{takahashi2018human}, we first estimated 3D pose information from the detected 2D poses from our pipeline.
We lift the estimated 2D poses to 3D poses by using the 3D pose estimation method~\cite{pavllo20193d}.
Then, the 3D poses are calibrated according to the camera viewpoint using Perspective-n-point projection technique~\cite{lepetit2009epnp}.
Specifically, at each time step $t$, we learn the extrinsic parameters, which are rotation and translation matrices, of the estimated 3D chest keypoints (left and right shoulders and left and right pelvis) for projecting 3D pose to the corresponding 2D keypoints in the image space. 

\begin{equation}
    [R|T]^t = \arg\min_{R,T}\| p^t_2 - sK[R|T]p^t_3 \|
\end{equation}

\noindent where $R\in\mathbb{R}^{3\times 3}$ is a rotation matrix subject to $R^TR=I\in\mathbb{R}^{3\times3}$ and $det(R) = 1$ and $T\in\mathbb{R}^{3\times 1}$ is a translation matrix that minimizes the projection error of chest keypoints of 3D pose, $p^t_3$, to 2D pose, $p^t_2$, at timestep $t$ given intrinsic camera lense parameter, $K\in\mathbb{R}^{3\times 3}$.
We fix the camera intrinsic matrix, $K$, with the parameters provided by the manufacturer~\cite{rpi_camera} and the scale parameter is arbitrarily set as $s=1$ as we do not require the absolute scale of the 3d pose size, but only the facing direction.
For each person, we smoothed $[R|T]^t$ over all time steps using moving SLERP filter~\cite{shoemake1985animating} and moving average filter for rotation and translation matrices, respectively, to keep the temporal consistency.
From the 3D pose calibrated according to the chest orientation, we acquire the 3D chest norm vector perpendicular to the left-to-right shoulder vector and left shoulder-to-left pelvis vector, $\Vec{v}^t_{chest} = \Vec{v}^t_{L.Shoulder \rightarrow R.Shoulder} \times \Vec{v}^t_{L.Shoulder \rightarrow L.Pelvis}$, at each timestep $t$.
The estimated 3D chest norm vector is projected to a 2D chest vector on a transverse plane, which represents the facing of each people in the scene with respect to the camera viewpoint.

\subsection{Evaluation}

We evaluate our multi-view multi-person tracking systems with respect to localization, tracking, and body orientation estimation performances following the standard evaluation methods~\cite{bernardin2006multiple,wu2020mebow}.

\subsubsection{Multi-person Tracking and Localization}

As there is no single metric for evaluating multi-person tracking methods, we utilize the following metrics to understand the performance of the proposed system~\cite{dendorfer2020mot20}.
$\uparrow$ and $\downarrow$ are shown for the metrics that are higher or lower the better, respectively.

\begin{itemize}
    \item MOTA $\uparrow$ (Multi-Object Tracking Accuracy) combines three kinds of error sources, which are false positives, missed targets, and identity switches.    
    \item IDF1 $\uparrow$ (ID F1 score) is the ratio of correctly identified detections over the average number of ground-truth and computed detections.
    \item MT $\uparrow$ (Mostly Tracked targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at least 80\% of their respective life span.
    \item ML $\downarrow$ (Mostly Lost targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at most 20\% of their respective life span.
    \item FPR $\downarrow$ (False Positives Rate) measures the average number of false alarms per frame.
    \item FNR $\downarrow$ (False Negatives Rate) measures the average number of missed targets per frame.
    \item Rcll $\uparrow$ (Recall) measures the ratio of correct detections to the total number of ground-truth locations.
    \item Prcn $\uparrow$ (Precision) measures the number of detected objects over the sum of detected and false positives.
    \item IDSR $\downarrow$ (ID Switch Ratio) measures the number of ID switches (IDS) over recall.
    \item Frag $\downarrow$  (Fragmentation) measures the total number of times a trajectory is fragmented, which are interruptions during tracking.
\end{itemize}

Specifically, $MOTA=1-\frac{\sum_t FN_t + FP_t + IDS_t}{\sum_t GT_t}$,
% \yash{This definition suggests that MOTA could potentially produce negative values, but earlier you mentioned that this metric is typically bounded between 0 and 1 unless we are forcing/constraining the algorithm to find/detect fixed number of objects/persons}\hyeok{As I clarified in the meeting. Yes. MOTA can go to negative but this means something is very wrong in the prediction.} 
where $FN_t$, $FP_t$, $IDS_t$, and $GT_t$ are false negatives (misses), false positives, ID switches, and ground-truths at time $t$.
One important evaluation that preceded tracking is detection. 
In this work, we define a ground-truth target at the time $t$ is detected if the estimated sample location is within 1.5 meters in euclidean distance.
Otherwise, the target is considered as \textit{missed}. 
As mentioned earlier, the 1.5-meter reference is based on the fact that people rarely walk faster than 1.42 m/s on an everyday basis~\cite{browning2006effects,mohler2007visual,levine1999pace}.

To demonstrate the localization accuracy of the estimated samples, we also report multiple object tracking precision, $MOTP=\frac{\sum_{i,t} d^i_t}{\sum_t c_t}$.
$d^i_t$ is the euclidean distance between the $i$th detected ground-truth sample and estimated sample, and $c_t$ is the number of detection at time $t$. 
In other words, MOTP is the average euclidean distance error for the detected samples, which shows the performance of the proposed systems to estimate the precise location of target samples that is independent of tracking trajectories or ID switches.
% We will also evaluate the proposed kalman filter-based tracking model with Hungarian matching-based tracking approach, which only considers detections in subsequent frames ignoring temporal consistency over the time.. 
% Majority of multi-view multi-person tracking methods are based on RGB color or depth images, which is not available in our dataset~\cite{gan2021self,haque2017towards,guo2022review}.
% Also, previous multi-view multi-person tracking methods are based on 2D image planes, and the global coordinate was projected directly using the known relationship between camera intrinsic and extrinsic parameters~\cite{tang2017multiple,liem2014joint}.
% The proposed approach differs as only 2D poses are available to preserve the privacy of the visitors and staff in our study site.

\subsubsection{Body Orientation}

Our benchmark dataset and the proposed method represent the body orientation as a continuous angle.
Following the standard definition of body orientation in the previous work~\cite{wu2020mebow,yu2019continuous,andriluka2010monocular}, we defined the human orientation $\theta \in [0\degree, 360\degree)$ as the chest facing direction on the transverse plane that is projected to the 2D coordinate in the study site, where the north (top) direction is the reference with clock-wise rotation.
Following previous work, we use two metrics: Mean Absolute Error (MAE) of angular distance and Accuracy-$X\degree$~\cite{wu2020mebow}.
Accuracy-$X\degree$ is defined as the ratio of the samples that are predicted within the deviation of $X\degree$ according to the ground-truth orientation. 
By using $X\in [0\degree, 180\degree]$, Accuracy-$X\degree$ measures fine-grained model accuracy.
% compared to the discrete orientation classification methods based on either equally spaced four (N, E, S, W) or eight (N, NE, E, SE, S, SW, W, NW) orientations~\cite{yu2019continuous}.
% We will compare the proposed body orientation estimation method with a number of baseline methods that is based on 1) 2D pose only or 2) 3D human pose and projection geometry~\cite{takahashi2018human}.
% For discrete evaluation, the continuous values in ground truth and estimated orientations are mapped to the closed four or eight direction and the estimated orientation is considered correct if the value is mapped to the correct directional bin.
% Following the previous work, we will use $X=\{5, 15, 22.5, 30, 45\}$.


==> sections/intro/_main_20230329.tex <==
%--------------------------------
% Before Restructuring ACM IMWUT to IEEE format
%--------------------------------

\section{Introduction}

%-----------------------------------------
% [] Importance of vision-based localization and tracking
% [] Limitation of Previous work
% [] Contribution of our work
% [] Major motivation of the proposed work
% major contribution and results of the proposed work
% broader impact of the proposed work
%-----------------------------------------

Indoor localization and tracking have been an active research area to support various critical applications, such as smart hospitals~\cite{haque2017towards,yang2020role}, smart office~\cite{lopez2017human}, or customer analysis in shopping mall~\cite{dogan2019analyzing}.
A wide range of sensors has been used to detect the whereabouts of multiple people in indoor spaces over the past two decades, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR)~\cite{cheol2017using}, WiFi~\cite{van2016performance}, and Bluetooth~\cite{yoo2018real}.

Recent advances in multi-person pose estimation~\cite{dai2022survey,dos2021monocular} and tracking have led to the use of cameras to track people indoors~\cite{tsai2016vision,cosma2019camloc}.
Some also explored using depth or thermal cameras to tackle the privacy challenges~\cite{luo2018computer,xue2018vision,haque2017towards}.
Vision-based approaches were very effective in capturing accurate and detailed movements continuously over time.
In most cases, however, only one camera is used to monitor users in a room, making it difficult to observe trajectories and movements in large indoor environments~\cite{luo2018computer,xue2018vision}.
Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing built-in infrastructure have not been fully examined. This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.
% Previous works have not discussed the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% \yash{I would make the claim less stronger, something like : Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing built-in infrastructure have not been fully examined. This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.}\hyeok{Better! I reflected this.}
%Also, it has not been discussed in previous work the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% These feasibility challenges can limit the use of those indoor tracking techniques in existing infrastructure that will have huge impact on quantifying human behavior in various contexts.

In this work, we propose a cost-effective, easy-to-install (with minimal modification of existing infrastructure) multi-person tracking system over a wide indoor space (18000+ square feet) using distributed multi-camera networks installed using edge, fog, and cloud computing frameworks.
We used 39 Raspberry Pis with camera sensors and Google Coral TPU USB accelerators. 
Each Raspberry Pi package costs less than \$500 combined~\cite{suresha2022edge}. 
The Raspberry Pi can easily be connected to the network and power sources available in the existing infrastructure in order to integrate the proposed system.
To preserve the privacy of the users, we process raw color frames in real-time on the device to detect 2D poses~\cite{papandreou2018personlab}, which are used to localize, track, and estimate the body orientation of multiple users.
As far as we know, this is the first work to estimate the orientations, positions and trajectories of multiple people using an edge and cloud computing framework for vastly wide indoor space monitoring.
%As far as we know, this is the first work to estimate the orientation of people as well as the localization and trajectory of multiple people using an edge and cloud computing framework for vastly wide indoor space monitoring.
{The space where the study was carried out offers therapeutic activities for individuals with Mild Cognitive Impairment (MCI), a stage between normal aging and dementia characterized by a decline in cognitive functions such as memory and attention~\cite{Gauthier2006_classic}. 
The design of the space was focused on promoting user engagement in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas).}
Observing how people's facing orientation varies while they move is an important factor in understanding social interaction or human attention~\cite{hall1963system,cristani2011social}.

In our experiment, our system demonstrates 62+\% Multiple-Object Tracking Accuracy (MOTA) score~\cite{bernardin2006multiple} on average for tracking people throughout the wide indoor space (18000+ square feet).
Specifically, for regions in our study site where a higher number of cameras were installed (7+), our system showed an 88+\% MOTA score.
%Especially for the region in our study site that has more cameras installed (7+), our system showed an 88+\% MOTA score.
Our body orientation estimation method showed an average of 28.9\degree error %\yash{I would use the exact average pose estimation error that we calculated (e.g., 29.5\degree)}\hyeok{Done.}
when compared against ground truth orientations collected from people walking in varying group formations. This is enough to sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis when multiple people were detected in a frame. % \yash{I would state more than one object was in the frame}.\hyeok{Done.}
%Overall, our body orientation estimation method showed <30\degree error compared to ground truth collected from people walking in varying group formations, which could sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis.
To provide practical guidelines when deploying the proposed system, we analyze key factors to consider when installing cameras, such as camera distances and viewpoints with respect to the captured person, and their impact on localization and orientation estimation errors.
It is expected that this work will promote the transformation of ordinary indoor spaces into smart indoor spaces with low costs to opportunistically provide services to improve people's well-being on a daily basis~\cite{haque2017towards,yang2020role,lopez2017human}{, while providing feedback to improve built environments such as the healthcare setting where this study was carried out.} 


==> sections/intro/_main_20231029.tex <==
\section{Introduction}

%-----------------------------------------
% [] Importance of vision-based localization and tracking
% [] Limitation of Previous work
% [] Contribution of our work
% [] Major motivation of the proposed work
% major contribution and results of the proposed work
% broader impact of the proposed work
%-----------------------------------------

Indoor localization and tracking is an active research area to support various applications, such as smart hospitals~\cite{haque2017towards,yang2020role}, smart offices~\cite{lopez2017human}, or customer analysis in shopping mall~\cite{dogan2019analyzing}. 
A wide range of sensors has been used to simultaneously detect the whereabouts and movement of multiple people in indoor spaces over the past two decades, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR)~\cite{cheol2017using}, WiFi~\cite{van2016performance}, and Bluetooth~\cite{yoo2018real}.

Recent advances in multi-person pose estimation~\cite{dai2022survey,dos2021monocular} and tracking have led to the use of cameras to track people indoors~\cite{tsai2016vision,cosma2019camloc}.
Some works also explored using depth or thermal cameras to tackle the privacy challenges~\cite{luo2018computer,xue2018vision,haque2017towards}.
Vision-based approaches have proven to be very effective in capturing accurate and detailed movements continuously over time.

In most cases, however, only one camera is used to monitor subjects in a room, making it difficult to observe trajectories and movements in large indoor environments~\cite{luo2018computer,xue2018vision}.
Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing indoor infrastructure have not been fully examined~\cite{boovaraghavan2023mites}. 
This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.
% Previous works have not discussed the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% \yash{I would make the claim less stronger, something like : Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing built-in infrastructure have not been fully examined. This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.}\hyeok{Better! I reflected this.}
%Also, it has not been discussed in previous work the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% These feasibility challenges can limit the use of those indoor tracking techniques in existing infrastructure that will have huge impact on quantifying human behavior in various contexts.

In this work, we propose a cost-effective, easy-to-install (with minimal modification of existing infrastructure) and privacy-preserving multi-person localization and tracking system over a wide indoor space (18000+ square feet) using distributed multi-camera networks installed using edge, fog, and cloud computing frameworks.
The edge computing system consists of 39 edge compute unit, each comprising a Raspberry Pi (v4 B) with a camera and Google Coral TPU USB accelerator for a total cost of less than \$200 each~\cite{suresha2022edge}. Each edge unit is connected to an on-site `fog' server via a private network, rather than WiFi, to enable security. (The WiFi was disabled.)
Raw color frames are processed automatically in real-time on the Coral TPU and edge computing system to detect 2D poses~\cite{papandreou2018personlab} and extract bounding boxes containing images of people present in the frame.
The extracted information, which is used to simultaneously localize, track, and estimate the body orientation of multiple subjects, do not contain individually-specific information.
To the best of our knowledge, this is the first work to simultaneously estimate the orientations, positions and trajectories of multiple people using an edge and fog/cloud computing framework for wide indoor space monitoring.

For context, the physical environment where our study was carried out offers therapeutic activities for individuals with Mild Cognitive Impairment (MCI), a clinically-defined stage between normal aging and dementia characterized by a decline in cognitive functions, such as memory and attention~\cite{Gauthier2006_classic}. 
This environment was designed to promote engagement of individuals with MCI in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas).
%Observing how orientation of the head with respect to others varies over time is an important factor in understanding social interaction or human attention~\cite{hall1963system,cristani2011social}.
% In our experiment, our system demonstrates 62+\% Multiple-Object Tracking Accuracy (MOTA) score~\cite{bernardin2006multiple} on average for tracking people throughout the wide indoor space (18000+ square feet).
% Specifically, for regions in our study site where a higher number of cameras were installed (7+), our system showed an 88+\% MOTA score.
% %Especially for the region in our study site that has more cameras installed (7+), our system showed an 88+\% MOTA score.
% Our body orientation estimation method showed an average of 28.9\degree error %\yash{I would use the exact average pose estimation error that we calculated (e.g., 29.5\degree)}\hyeok{Done.}
% when compared against ground truth orientations collected from people walking in varying group formations. This is enough to sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis when multiple people were detected in a frame. % \yash{I would state more than one object was in the frame}.\hyeok{Done.}
% %Overall, our body orientation estimation method showed <30\degree error compared to ground truth collected from people walking in varying group formations, which could sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis.
% To provide practical guidelines when deploying the proposed system, we analyze key factors to consider when installing cameras, such as camera distances and viewpoints with respect to the captured person, and their impact on localization and orientation estimation errors.
However, the framework presented in this article is rather general and could be used to analyze movement and interactions of individuals in many contexts, such as the emergency room, care homes,   
It is expected that this work will promote the transformation of ordinary indoor spaces into smart indoor spaces with low costs to opportunistically provide services to improve people's well-being on a daily basis~\cite{haque2017towards,yang2020role,lopez2017human}, while providing feedback to improve built environments such as the healthcare setting where this study was carried out. Notably, because the edge computing framework is privacy-preserving with processing at the edge, our proposed system addresses concerns over using tracking and video capture of individuals. 


==> sections/intro/main.tex <==
\section{Introduction}

%-----------------------------------------
% [] Importance of vision-based localization and tracking
% [] Limitation of Previous work
% [] Contribution of our work
% [] Major motivation of the proposed work
% major contribution and results of the proposed work
% broader impact of the proposed work
%-----------------------------------------

Indoor localization and tracking is an active research area to support various applications, such as smart hospitals~\cite{haque2017towards,yang2020role}, smart offices~\cite{lopez2017human}, or customer analysis in shopping mall~\cite{dogan2019analyzing}. 
A wide range of sensors has been used to simultaneously detect the whereabouts and movement of multiple people in indoor spaces over the past two decades, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR)~\cite{cheol2017using}, WiFi~\cite{van2016performance}, and Bluetooth~\cite{yoo2018real}.
Recent advances in multi-person pose estimation~\cite{dai2022survey,dos2021monocular} and tracking have led to the use of cameras to monitor indoor activities~\cite{tsai2016vision,cosma2019camloc}, and
% Some works also explored using depth or thermal cameras to tackle the privacy challenges~\cite{luo2018computer,xue2018vision,haque2017towards}.
vision-based approaches have proven to be very effective in capturing accurate and detailed movements continuously over time.
\revision{
However, most studies have only examined a few cameras in small rooms and have not studied a system that integrates localization, tracking, and body orientation estimation techniques required to understand fine-grained activities comprehensively
~\cite{luo2018computer,xue2018vision,luo2018computer,xue2018vision,haque2017towards}.
Also, advancements in edge computing now allow for low-cost, powerful devices to monitor activity in existing buildings~\cite{jin2022survey,suresha2022edge,barthelemy2019edge}. 
But, the utility of these technologies for indoor monitoring in large buildings remains unstudied.
}

% Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing indoor infrastructure have not been fully examined~\cite{boovaraghavan2023mites}. 
% This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.
% Previous works have not discussed the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% \yash{I would make the claim less stronger, something like : Despite significant advancements in vision-based tracking, the cost and feasibility of installing cameras into existing built-in infrastructure have not been fully examined. This could pose challenges and potentially significant expenses, depending on the level of modification required to install multiple cameras.}\hyeok{Better! I reflected this.}
%Also, it has not been discussed in previous work the cost and feasibility of installing cameras into existing built-in infrastructure, which can be challenging or extremely expensive depending on the level of modification needed to install multiple cameras.
% These feasibility challenges can limit the use of those indoor tracking techniques in existing infrastructure that will have huge impact on quantifying human behavior in various contexts.

\revision{
In this work, we provide a feasibility study and systematic analysis of a camera-based indoor localization and tracking system to monitor multiple people across a wide indoor space (1700$m^2$) using an edge computing framework.
We installed 39 cameras distributed in the ceiling of an indoor space having a complex structure with various functioning spaces, including a gym, library, kitchen, classroom, etc., using edge computing units (Raspberry Pi v4 B).
To preserve the privacy of individuals, raw color frames are processed automatically in real-time on the Coral Tensor Processing Unit (TPU) to detect 2D poses~\cite{papandreou2018personlab}, which is used to simultaneously localize, track, and estimate the body orientation of multiple subjects.
Using our camera infrastructure, we aim to provide a comprehensive analysis of the camera installation and its relations with the performance of our system in various activity scenarios.
We expect this work to provide practical guidelines for practitioners when installing a multi-view camera-based activity monitoring system using edge computing frameworks in existing facilities.
}

\revision{
For context, the physical environment of our study was designed to promote the engagement of older adults in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas).
}
Notably, because the edge computing framework is privacy-preserving with processing at the edge, our proposed system addresses concerns over using tracking and video capture of individuals. 
The proposed system is easy to install in existing indoor environments and potentially useful for capturing, for example, critical behaviors in therapeutic units like our study site. 


% In this work, we propose a cost-effective, easy-to-install (with minimal modification of existing infrastructure) and privacy-preserving multi-person localization and tracking system over a wide indoor space (18000+ square feet) using distributed multi-camera networks installed using edge, fog, and cloud computing frameworks.
% The edge computing system consists of 39 edge compute unit, each comprising a Raspberry Pi (v4 B) with a camera and Google Coral TPU USB accelerator for a total cost of less than \$200 each~\cite{suresha2022edge}. Each edge unit is connected to an on-site `fog' server via a private network, rather than WiFi, to enable security. (The WiFi was disabled.)
% Raw color frames are processed automatically in real-time on the Coral TPU and edge computing system to detect 2D poses~\cite{papandreou2018personlab} and extract bounding boxes containing images of people present in the frame.
% The extracted information, which is used to simultaneously localize, track, and estimate the body orientation of multiple subjects, do not contain individually-specific information.
% To the best of our knowledge, this is the first work to simultaneously estimate the orientations, positions and trajectories of multiple people using an edge and fog/cloud computing framework for wide indoor space monitoring.

% For context, the physical environment where our study was carried out offers therapeutic activities for individuals with Mild Cognitive Impairment (MCI), a clinically-defined stage between normal aging and dementia characterized by a decline in cognitive functions, such as memory and attention~\cite{Gauthier2006_classic}. 
% This environment was designed to promote engagement of individuals with MCI in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas).
%Observing how orientation of the head with respect to others varies over time is an important factor in understanding social interaction or human attention~\cite{hall1963system,cristani2011social}.
% In our experiment, our system demonstrates 62+\% Multiple-Object Tracking Accuracy (MOTA) score~\cite{bernardin2006multiple} on average for tracking people throughout the wide indoor space (18000+ square feet).
% Specifically, for regions in our study site where a higher number of cameras were installed (7+), our system showed an 88+\% MOTA score.
% %Especially for the region in our study site that has more cameras installed (7+), our system showed an 88+\% MOTA score.
% Our body orientation estimation method showed an average of 28.9\degree error %\yash{I would use the exact average pose estimation error that we calculated (e.g., 29.5\degree)}\hyeok{Done.}
% when compared against ground truth orientations collected from people walking in varying group formations. This is enough to sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis when multiple people were detected in a frame. % \yash{I would state more than one object was in the frame}.\hyeok{Done.}
% %Overall, our body orientation estimation method showed <30\degree error compared to ground truth collected from people walking in varying group formations, which could sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis.
% To provide practical guidelines when deploying the proposed system, we analyze key factors to consider when installing cameras, such as camera distances and viewpoints with respect to the captured person, and their impact on localization and orientation estimation errors.

% However, the framework presented in this article is rather general and could be used to analyze movement and interactions of individuals in many contexts, such as the emergency room, care homes,   
% It is expected that this work will promote the transformation of ordinary indoor spaces into smart indoor spaces with low costs to opportunistically provide services to improve people's well-being on a daily basis~\cite{haque2017towards,yang2020role,lopez2017human}, while providing feedback to improve built environments such as the healthcare setting where this study was carried out. 
% Notably, because the edge computing framework is privacy-preserving with processing at the edge, our proposed system addresses concerns over using tracking and video capture of individuals. 


==> sections/intro/main_alternate.tex <==
\section{Introduction}

%-----------------------------------------
% [] Importance of vision-based localization and tracking
% [] Limitation of Previous work
% [] Contribution of our work
% [] Major motivation of the proposed work
% major contribution and results of the proposed work
% broader impact of the proposed work
%-----------------------------------------

Indoor localization and tracking is an active research area to support various applications, such as smart hospitals~\cite{haque2017towards,yang2020role}, smart offices~\cite{lopez2017human}, or customer analysis in shopping mall~\cite{dogan2019analyzing}. 
A wide range of sensors has been used to simultaneously detect the whereabouts and movement of multiple people in indoor spaces over the past two decades, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR)~\cite{cheol2017using}, WiFi~\cite{van2016performance}, and Bluetooth~\cite{yoo2018real}.
Recent advances in multi-person pose estimation~\cite{dai2022survey,dos2021monocular} and tracking have led to the use of cameras to monitor indoor activities~\cite{tsai2016vision,cosma2019camloc}, and
vision-based approaches have proven to be very effective in capturing accurate and detailed movements continuously over time.
\revision{
However, most studies have only examined a few cameras in small rooms and have not studied a system that integrates localization, tracking, and body orientation estimation techniques in a large indoor space required to understand fine-grained activities comprehensively ~\cite{luo2018computer,xue2018vision,haque2017towards}. Advancements in edge computing now allow for low-cost, powerful devices to monitor activity in existing buildings~\cite{jin2022survey,suresha2022edge,barthelemy2019edge}. 
}

\revision{
The contribution of this work is two-fold. First, we propose an edge computing pipeline designed to localize, track and estimate the body-facing orientations of multiple individuals within a large indoor space using multiple cameras while prioritizing privacy. Second, we perform a feasibility study of the proposed pipeline, offering practical insights into the utilization of cameras for localization and tracking in indoor environments.}
\revision{
To this end, we deployed 39 cameras positioned throughout a 1700 square meter indoor space with diverse functional areas, such as a gym, library, and kitchen. These cameras were connected to edge computing units, specifically Raspberry Pi v4 B devices. To safeguard the privacy of individuals, we adopted a real-time processing approach using Google Coral Tensor Processing Units (TPUs) connected to the edge computing units. These TPUs automatically process raw color frames obtained from the cameras to detect 2D poses (as described in~\cite{papandreou2018personlab}). This information is then used to estimate the positions and orientations of people within the indoor space, and the original raw frames are discarded. The estimated positions and orientations from all the cameras are combined to track the movement of individuals.
Using our camera infrastructure, we aim to provide a comprehensive analysis of the camera installation and its relations with the performance of our system in various activity scenarios.
We expect this work to provide practical guidelines for practitioners when installing a multi-view camera-based activity monitoring system using edge computing frameworks in existing facilities.
}


%\revision{
%The physical environment of our study was designed to promote the engagement of older adults in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas). However, the system described in this work is applicable in any indoor scenario.
%}
%Notably, because the framework is privacy-preserving with processing at the edge, our proposed system addresses concerns about video capture of individuals. 

%The proposed system is easy to install in existing indoor environments and potentially useful for capturing, for example, critical behaviors in therapeutic units like our study site. 


% In this work, we propose a cost-effective, easy-to-install (with minimal modification of existing infrastructure) and privacy-preserving multi-person localization and tracking system over a wide indoor space (18000+ square feet) using distributed multi-camera networks installed using edge, fog, and cloud computing frameworks.
% The edge computing system consists of 39 edge compute unit, each comprising a Raspberry Pi (v4 B) with a camera and Google Coral TPU USB accelerator for a total cost of less than \$200 each~\cite{suresha2022edge}. Each edge unit is connected to an on-site `fog' server via a private network, rather than WiFi, to enable security. (The WiFi was disabled.)
% Raw color frames are processed automatically in real-time on the Coral TPU and edge computing system to detect 2D poses~\cite{papandreou2018personlab} and extract bounding boxes containing images of people present in the frame.
% The extracted information, which is used to simultaneously localize, track, and estimate the body orientation of multiple subjects, do not contain individually-specific information.
% To the best of our knowledge, this is the first work to simultaneously estimate the orientations, positions and trajectories of multiple people using an edge and fog/cloud computing framework for wide indoor space monitoring.

% For context, the physical environment where our study was carried out offers therapeutic activities for individuals with Mild Cognitive Impairment (MCI), a clinically-defined stage between normal aging and dementia characterized by a decline in cognitive functions, such as memory and attention~\cite{Gauthier2006_classic}. 
% This environment was designed to promote engagement of individuals with MCI in diverse therapeutic activities, such as exercise and memory training, while also creating opportunities for social interaction (e.g., during meals and in lounge areas).
%Observing how orientation of the head with respect to others varies over time is an important factor in understanding social interaction or human attention~\cite{hall1963system,cristani2011social}.
% In our experiment, our system demonstrates 62+\% Multiple-Object Tracking Accuracy (MOTA) score~\cite{bernardin2006multiple} on average for tracking people throughout the wide indoor space (18000+ square feet).
% Specifically, for regions in our study site where a higher number of cameras were installed (7+), our system showed an 88+\% MOTA score.
% %Especially for the region in our study site that has more cameras installed (7+), our system showed an 88+\% MOTA score.
% Our body orientation estimation method showed an average of 28.9\degree error %\yash{I would use the exact average pose estimation error that we calculated (e.g., 29.5\degree)}\hyeok{Done.}
% when compared against ground truth orientations collected from people walking in varying group formations. This is enough to sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis when multiple people were detected in a frame. % \yash{I would state more than one object was in the frame}.\hyeok{Done.}
% %Overall, our body orientation estimation method showed <30\degree error compared to ground truth collected from people walking in varying group formations, which could sufficiently distinguish eight cardinal directions (N, NE, E, SE, S, SW, W, NW) for downstream social interaction analysis.
% To provide practical guidelines when deploying the proposed system, we analyze key factors to consider when installing cameras, such as camera distances and viewpoints with respect to the captured person, and their impact on localization and orientation estimation errors.

% However, the framework presented in this article is rather general and could be used to analyze movement and interactions of individuals in many contexts, such as the emergency room, care homes,   
% It is expected that this work will promote the transformation of ordinary indoor spaces into smart indoor spaces with low costs to opportunistically provide services to improve people's well-being on a daily basis~\cite{haque2017towards,yang2020role,lopez2017human}, while providing feedback to improve built environments such as the healthcare setting where this study was carried out. 
% Notably, because the edge computing framework is privacy-preserving with processing at the edge, our proposed system addresses concerns over using tracking and video capture of individuals. 


==> sections/method/_main_20230329.tex <==
\section{Method}

In this work, distributed camera networks are installed with edge, fog, and cloud computing environments to locate and track multiple people with their body orientations in a built-in environment.
This section describes the overall computing environment of our system and describes the techniques to continuously monitor people's movements in space.

\subsection{Distributed Camera Network using Edge Computing}

\input{figure/camera_config}

\subsubsection{Camera Configuration}

\autoref{fig:camera_config} illustrates the camera installation of the study site, the area of which spans 18,286 square feet space. 
By using a low-cost (<\$500) Raspberry Pi
% \robert{The grammar here is off, but I'm not sure the best way to correct it; do we want to refer to just a single unit ["By using a low cost (<\$500) Raspberry Pi"] or the group of units as a whole ["By using low cost (<\$500) Raspgerry Pis"]?}\hyeok{A single unit}
, we installed 39 cameras in the study sites as shown in \autoref{fig:camera_config}, (a).
Raspberry Pis were placed and hidden on the ceiling panel and connected to power and network sources in the existing infrastructure.
The camera sensor (Sony IMX219 8-megapixel sensor) and Google Coral USB Accelerator were installed in the Raspberry Pi 4 to run a deep learning-based 2D pose estimation model in real time (\autoref{fig:camera_config} (c)).
Each camera is attached to the ceiling with the viewpoints toward the darker blue side (\autoref{fig:camera_config} (b)). 
With 39 cameras, our localization algorithm was able to detect and locate people across the large space with a 1.5-meter error 
% \robert{Should this also read "margin of error", or is that redundant because the phrase "error margin" is immediately referenced in the next clause?}\hyeok{Good point. Margin of error for the next clause.}
, which fits within the acceptable margin of error to understand activity in the studied area.

\input{figure/compute_config}

\subsubsection{Computing Network Architecture}

The overall configuration consists of 4 primary segments: the cloud server, the on-premise fog server, the private Pi networking infrastructure, and the Pis themselves.
Our computing environment is illustrated in \autoref{fig:compute_config}, which includes 39 Raspberry Pis, one Fog computing node on the study site, and one cloud computing node off the study site.
% \robert{Should the word "Each" be here, to quantify each Raspberry Pi?}\hyeok{Done.}
Each Raspberry Pi runs multi-person 2D pose estimation on the fly~\cite{papandreou2018personlab}, which reduces the risk of a data breach by not storing potentially sensitive video data on the device.
A 2D pose is estimated every second, resulting in a frame rate of 1 Hz, and if the 2D pose is detected on any Raspberry Pi, the 2D keypoint and human bounding box information is directly transferred and stored on a Health Insurance Portability and Accountability Act (HIPAA)-compliant data storage server at the study site.
% The human bounding box from detected 2D poses are additionally transferred to Fog computing node for analyzing the body orientation of the detected person~\cite{wu2020mebow}.
The bounding box images are only temporarily stored (one hour) in the Fog computing node
% \robert{The plural here makes it sound like we have more than one Fog node in our setup; not sure if this sentence is supposed to be referencing deployments of this infrastructure in general (in which case the wording's fine as-is) or specifically our infrastructure. All other references have just been singular, so I don't know if we want to maintain that consistently through the paper or not.}\hyeok{You are correct. It has to be specifically for our infrastructure. So, it has to be singular.} 
for data preprocessing and are not transferred to cloud computing nodes.
We store only the 2D keypoint information, which has 17 keypoints based on MS COCO format~\cite{lin2014microsoft}, 
% \yash{I would mention which version go Posenet we used and how many keypoints we can detect (e.g., maximum of 17 or 33 keypoints)}\hyeok{Done.} 
and the processed body orientation estimation results for permanent data management and analysis.

The fog computing node
% \yash{in the setting that we defined earlier, do we have more than single fog computing node(i.e., the server)?} \robert{In reply to Yash, we do not have anything other than the single server at the site}\hyeok{Correct. This is a typo.} 
store a day's worth of data between 8 AM and 7 PM, when visitors are present.
Additional activity analysis is carried out by fog computing node,
% \robert{Plural; same comments as Yash's and mine above}\hyeok{Corrected.}
which includes body orientation estimation, multi-person localization, and tracking of the previous day's data.
Data collected in the fog node and its analysis is synced nightly approximately between 12 PM and 7 AM. 
The duration for nightly sync can change depending on the data size collected over the day.
% \robert{Our sync's actually scheduled to start after midnight as it calculates the previous day's date in order to perform the sync; it also doesn't always finish before 7 AM if there's a lot of data...}\hyeok{Added 'approximate'} 
to a cloud node's HIPAA-compliant data server for permanent storage.
Our data management framework demonstrates that the activities in study sites are passively and continuously collected with minimal privacy risks.
Furthermore, the cameras installed above visitors' eyesight made it easier for visitors to comply with the proposed instrumentation of cameras for activity monitoring. 

The on-premise fog server for the Pi network contains 2 10Gb SFP+ Ethernet interfaces, which are bonded together into a single 20G interface and connected to the switches used for the private Pi network. 
This bonded interface is used to provide enough bandwidth that the multiple Pis deployed within the study site are able to write their collected data back to the on-premise fog server for storage without creating a severe network bottleneck due to the amount of devices that were planned for deployment. 
The networking infrastructure consists of a set of 2 interconnected Supermicro SSE-G3648B switches running Cumulus Linux 3.7.12, which have been programmatically bonded together so that they will act as a single large switch while improving throughput, as one half of the 20G bond is connected to each switch.
Thus, either one can be used to pass traffic between the on-premise fog server and the data collection Pis. 
Each Pi is connected to one of the two switches via a 1Gb Ethernet connection, as the maximum speed on the Network Interface Card built into the Pis is only 1Gb. 
To prevent data breaches or leaks of sensitive data, the entire Pi network is isolated from the on-premise network. 
% \robert{We may want to say that the Pi network is physically isolated from the on-prem network rather than the cloud network, as "cloud network" implies a network that is off-site and technically every other network would be just as isolated from it; the original wording of this referenced Emory's network, while BMI's is the "cloud" network.}\hyeok{Thank you for the clarification. Corrected it!}
The only connections to the switches are by the on-premise fog server and the Pis themselves.

To facilitate the operation of all the Pis on the data collection network, the on-premise fog server provides Dynamic Host Configuration Protocol (DHCP) and Network Time Protocol (NTP) services to assign the Pis with their appropriate Internet Protocol (IP) addresses and provide them with the correct date and time when they boot up; to ensure that the same Pi receives the same address each time, the addresses are manually specified in the DHCP server’s configuration based on the Media Access Control (MAC) address of the Pi. 
The on-premise fog server also acts as a gateway to allow the Pis to reach the cloud network if needed for software update purposes, while acting as a firewall to prevent others on the cloud network from having direct access to the Pis. 
A Network File System (NFS) volume is configured on the fog server and shared with the private Pi network so that the Pis can mount a shared network volume for the purposes of operation and data storage.
Each Pi’s base image is programmed to connect to the on-premise fog server at a known static IP address and mount the NFS volume at boot up. 
% \robert{Should we also mention that the Pis launch a shared bootstrapping script which is located on this NFS volume? It's referenced in the next sentence that the Pis "load the environment and run the script", but we haven't explained what the script is yet.}\hyeok{Done. Added this detail in the next sentence}
This allows for software and functionality changes in the on-premise fog server to be deployed across all Pis on the network by simply modifying the shared configuration to reflect the desired operation.
When Pis are rebooted, they launch a shared bootstrapping script, which is located on this NFS volume, so that it will load the environment and run the script.

For storage, the on-premise server has 6 $12TB$ storage disks configured in a RAID10 configuration for $\sim32TB$ of usable space.
RAID10 was selected to provide the fastest available speeds while still allowing for disk redundancy in the event of a failure. 
The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network.
% \robert{I'm pretty sure this should read "The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network." or something along those lines.}\hyeok{Reflected.}
As the on-premise fog server is deployed in the study site, it is not directly connected via 10G Ethernet to the cloud server’s private network. 
This makes the intermediate network links between the fog node and the cloud node's network not guaranteed to all be at the maximum speed supported by either endpoint, thereby, resulting in slower network speeds than a direct connection
% \robert{Probably don't need to mention 10G and can instead reword this to be something like "the intermediate network links between the fog node and the cloud node's network are not guaranteed to all be at the maximum speed supported by either endpoint, resulting in slower network speeds than a direct connection".}\hyeok{Done. and commented the next sentence, too.}
% This makes the data traverse the general virtual private network (VPN), which at this time only runs at 1G speeds. 
% \robert{Our deployment of this is not traversing a VPN at all; it's just going over the regular Emory network and encapsulated within a SSH connection. The equivalent for a generic deployment would be the fog node's site's network and/or the Internet depending on the location of the cloud node.}
The transfer process is performed from the on-premise fog server by using Tape ARchive (TAR) 
% \robert{Not sure if we need to bold/italicize/define/something the word "tar" to indicate that it's a system command. It's short for "Tape ARchive", just in case that's helpful.}\hyeok{Good!} 
to combine all of one day’s data collection files into a single data stream, which is then transmitted over Secure Shell (SSH) to a gateway server dedicated to large data transfers on the cloud server’s main network.
The data transfer stream is then untarred and the files are placed in the designated location on the cloud server’s filesystem. 
The usage of this single stream reduces the number of individual network I/O operations that need to be performed during the transfer process (thus improving performance) when compared to other transfer options like rsync or scp operating on individual files.
It also removes the need to manually stage the tar file on the server prior to transfer as the output of tar is piped directly to the remote system and an untar process via SSH. 

\subsection{Monitoring Activities in Built-in Environment}

\subsubsection{Overall Pipeline}

Here, we describe our approaches to continuously monitor the activities of multiple people in our study space with the abovementioned computing and camera infrastructure.
The overall approach for multi-view multi-person tracking is shown in \autoref{fig:overall_method}.
Based on pose detection and human bounding boxes, each person's location and body orientation are estimated and projected on a 2D coordinate system representing the study space.
Multiview integration then resolves duplicate samples across cameras from overlapping views by combining samples from 39 cameras.
Lastly, a multi-person tracking algorithm~\cite{li2010multiple} is used to track people across the frames.

\input{figure/overall_method.tex}

\subsubsection{Preprocessing 2D poses}
\label{sec:preproc_poses}

The 2D poses estimated on Raspberry Pi are first preprocessed to remove noisy samples.
Two major artifacts were observed for the detected poses from our model~\cite{papandreou2018personlab}: non-human poses and temporal inconsistencies.
First, the model considers patterns on the walls and floor as humans due to the way the camera views them from the ceiling.
These non-human poses remain stationary over time and do not change rapidly.
Thus, we remove those false positives (non-human samples) by identifying poses in subsequent frames where pose changes are near zeros.
Second, 2D poses lack temporal consistency since the model estimates poses frame-by-frame. 
It was observed that a number of poses had their left and right sides flipped or missing between frames (false negatives).
We used Kalman filter-based temporal smoothing to denoise and fill missing detections~\cite{10.1115/1.3662552}.
For Kalman filter, linear constant model was used for modeling temporal changes in keypoint locations of COCO pose, which has 17 joint keypoints~\cite{lin2014microsoft}, $X_t=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}, \dot{u}_1 \dot{v}_1, \dot{u}_2 \dot{v}_2, \cdots, \dot{u}_{17} \dot{v}_{17}]$, where $u$ and $v$ are $x$ and $y$ location of each keypoint and $\dot{u}$ and $\dot{v}$ are the velocity of location changes.

\input{figure/tracker}

Kalman smoothing for 2D poses is achieved by using Kalman filter-based multi-person tracking technique that has been widely adopted in the past~\cite{bewley2016simple}.
As shown in \autoref{fig:kalman_tracker} (a), the tracker follows predict, detect, match, update, and repeat operations.
Given multi-person tracking until time $t-1$, Kalman filter trackers make predictions of each person's location at time $t$. 
To update the prediction based on actual detections at time $t$, the Hungarian method is used to find matches between predictions and detections from 2D poses~\cite{kuhn1955hungarian} (\autoref{fig:kalman_tracker}, b).
Hungarian methods are widely used to find matches between two groups of samples because of their efficiency and effectiveness~\cite{perera2006multi,bewley2016simple,xu2020train}.
For Hungarian matching, we generate a bipartite graph where each node is 2D pose from prediction and detection at time $t$ and the edge is $L_2$-norm distance between those 2D poses.
The bipartite graph is represented as a matrix, where $C_{i,j}= \|P^i_{p} - P^j_{d} \|_2$ is $L_2$-norm distance between $i$th pose from predictions, $P_p$,  and $j$th pose from detections, $P_d$. 
% and $P=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}]$.
The Hungarian method then finds the matchings (or edges) with the smallest sum of distances between the samples from predictions and detections (\autoref{fig:kalman_tracker} (b), \textcolor{red}{red} lines).
Hungarian method optimizes:

\begin{equation}
    Y = \arg\min_{Y} \sum_i \sum_j C_{i,j} Y_{i,j}
\end{equation}

% \chaitra{I think we should explain what this equation is before introducing it. There is a discontinuity between the previous sentence and this one}\hyeok{Done.}
\noindent where $Y$ is a boolean matrix, showing assignment within $C$.
Next, The predictions get updated with the matched detections.
For the unmatched detections, a new tracker initiates.
In the case of false negatives (no detections in time $t$), we skip the update operation and continue with the prediction, which is kept alive for 10 seconds to handle potential false negatives.
Until the tracking is complete, this process is repeated.
Lastly, we apply kalman smoothing with Rauch-tung-Striebel (RTS) smoother to optimize the temporal consistency of estimated 2D pose movements based on all trackers over time~\cite{chan2011implementation}.
Using these processed 2D poses, we can now localize indoors and track multiple people based on multiple viewpoints.

\subsubsection{Indoor Localization}

An indoor localization technique aims to locate people within the study site in 2D coordinate space based on the 2D poses detected from each camera.
As a rule of thumb, the middle of the left and right feet is defined as the location of people in a scene.
As the floor in our study space is flat, any detected people in a scene are on the same plane.
With this in mind, we learn a perspective transformation matrix, $M\in \mathbb{R}^{3\times3}$, that can project the foot location from the floor in 2D camera space to the corresponding floor location in the 2D coordinate of the study site~\cite{sun2019see,cosma2019camloc}.

\begin{equation}
    \begin{bmatrix}
        x \\ y \\ 1
    \end{bmatrix}
    = \begin{bmatrix}
        m_{11} & m_{12} & m_{13} \\
        m_{21} & m_{22} & m_{23} \\
        m_{31} & m_{32} & m_{33}
    \end{bmatrix}
    \begin{bmatrix}
        u \\ v \\ 1
    \end{bmatrix}  
    \label{eqn:perspective_mat}
\end{equation}

\noindent where $[x, y]$ is the foot location in study site coordinate and $[u, v]$ is the foot pixel location in the camera.
From every 39 cameras, we learn $M$ by manually selecting 4 corresponding points in the 2D coordinate study site and the pixel locations in the field of view of a camera~\cite{abdel2015direct,shim2015mobile}.
Once $M$ is derived, they are used to localize the feet locations of detected 2D poses in the study space coordinate. 
% unless the camera location or orientation is changed.

\subsubsection{Body Orientation Estimation}

The facing orientation of people in a group activity gives important insights into their relationship and engagement with each other~\cite{cristani2011social,barua2021detecting}.
From the human bounding box detected by 2D pose detection models, we extract the facing direction of each person in the transverse plane, whose orientation is then transformed into the study site coordinates.
For estimating chest facing direction in a human bounding box image, we adopt the deep learning-based body orientation estimation method~\cite{wu2020mebow}. 
Wu~\etal~\cite{wu2020mebow} proposed a deep learning model that combines HRNet~\cite{sun2019deep} and ResNet~\cite{he2016deep} to predict chest facing orientation in 5\degree-intervals from human bounding box images.
The model was trained to learn from multiple tasks, including 2D pose, 3D pose, and body orientation prediction.
This enabled the model to learn the representation that considers 2D and 3D pose geometry and depth information for robustly estimating body orientation from 2D human bounding box images.
Here, we define a human bounding box as a tight square region that contains a detected 2D pose from Raspberry Pi.
The estimated chest orientation is represented as a 2D chest vector on a transverse plane.
Then, the 2D chest vector in camera space is transformed to the 2D orientation in study site coordinate, $\Vec{v}^t_{world} = R_{camera \rightarrow world}\Vec{v}^t_{world}$.
The rotation matrices, $R_{camera \rightarrow world}$, for each camera is manually defined according to the camera installation in the study site, where north is set as a reference orientation.

\subsubsection{Multi-view Integration}

\input{figure/multi-view_integration.tex}

The 39 cameras installed in the study site 
% \robert{Should "sites" be plural or singular? We're only talking about the one deployment, correct?}\hyeok{Yes. Correct. Haha I am keep making this typo for singular/plural.}
have partially overlapping field-of-views to continuously track people across the wide space.
Multiple cameras capture duplicate samples of the same person due to these overlaps.
In order to remove duplicated samples, we detect persons across cameras and integrate the detections into a single sample that potentially represents the true location of the person, as shown in \autoref{fig:muti-view_integration}.
To detect those duplicated samples, we generate a graph, $G=(V,E)$, where vertices, $V=\{v_{ci}=(x,y)|c=1,\cdots,39, i=1,\cdots\}$, are locations of all samples from all 39 cameras and edge, $E=\{v_{ci}v_{c'j} |\; c \neq c' \}$, is the connectivity between samples from different cameras that are sufficiently close in the distance.
We assume that duplicates are coming from the same person captured in different cameras, if their euclidean distance is within $\| v_{ci} - v_{c'j} \|_2 \leq 1.5 m$, considering the error margin of our localization technique.
It is possible for the same person located from a different camera to be in a slightly different location from our indoor localization due to lens distortions violating planar assumptions about the floor that can incur inaccuracies in perspective transformations.
% that is used for perspective transformation in our indoor localization technique.
Regardless, we empirically found that only 1.5 meters were sufficient for the margin of the localization error~\cite{zhang2000flexible}.

Once the graph $G$ is constructed, the duplicated samples are identified as those with linked vertices in a graph, which is also called connected components, $CC$, from graph theory~\cite{john1995first}.
Then, we integrate the locations of the duplicated samples considering the camera distance from the detected sample. 
Specifically, when integrating duplicated samples, the samples are penalized when the camera distance is far:

\begin{equation}
    L = \sum_{CC} \frac{1}{d_{ci}} v_{ci}
\end{equation}

\noindent where $L$ is the location of integrated sample and $d_{ci} = \| l_c - v_{ci} \|^2_2$ is the euclidean distance between the sample, $v_{ci}$, and the camera, $l_c$.
According to our findings, the localization error and the distance between the camera and the target person are strongly correlated.
Similarly, the orientation of the duplicated samples is integrated for the vertices in $CC$ considering camera distances.
The multi-view integration results in unique locations, $L=[l_x, l_y]$, and orientation vector, $o=[o_x, o_y]$, of each person at each time step.  

\subsubsection{Multi-person Tracking}

To understand detailed individual or group activities occurring in the study site, the locations of people needs to be tracked across time.
For multi-person tracking, we also apply Kalman filter-based tracking for the locations, $L=[l_x, l_y]$, and orientation vector, $O=[o_x, o_y]$, from multi-view integration~\cite{kuhn1955hungarian}.
The tracker follows predict, detect, match, update, and repeat steps used in Sec.~\ref{sec:preproc_poses}, but with some differences.
We again use a linear constant model for both location and orientation, where states are represented as location, $L=[l_x, l_y]$, orientation, $O=[o_x, o_y]$, velocity, $\dot{L}=[\dot{l}_x, \dot{l}_y]$, and angular velocity, $\dot{O}=[\dot{o}_x, \dot{o}_y]$.
Furthermore, we assume that people's facing orientation follows their walking direction closely.
Therefore, the tracker estimates facing orientation at time $t$ by summing up both moving directions, the velocity when 1 Hz, $\dot{L}$, and angular velocity, $\dot{O}$.

\begin{equation}
    O_t= O_{t-1} + w\cdot \dot{L}_{t-1} + dt\cdot \dot{O}_{t-1}
\end{equation}

\noindent where $w=0.1$ is a weighting of moving direction (or velocity) on current orientation and $dt$ is the time interval between frames, which is 1 sec.
When associating predictions and matching using Hungarian matching, the bipartite graph is represented as a matrix, where $C_{i,j}= \|L^i_{p} - L^j_{d} \|_2$ is euclidean distance between $i$th sample from prediction, $L_p$, and $j$th sample from detection, $L_d$.
Likewise earlier, we applied RTS smoothing for finished trackers to consider temporal dynamics across the entire trajectory of a person.



==> sections/method/_main_20231029.tex <==
\section{Method \& Materials}

\input{figure/ep6_func_spaces.tex}

In this work, multiple edge computing-based camera systems are integrated into a distributed network and are installed with edge, fog, and cloud computing environments to locate and track multiple people with their body orientations in a built environment.
This section provides a detailed account of our study site, the computing environment of our system, and the techniques employed to continuously monitor people's movements in a given space and an evaluation of the systems.

\subsection{Study Site}

The study site used in this work is a 18,286 square feet indoor environment consisting of various functioning spaces such as a library, kitchen, dining area, gym, etc., as shown in \autoref{fig:ep6_func}.
Referring \autoref{fig:ep6_func} and \autoref{fig:data_collection}, Activity Area (A) includes both the Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and left boundary of conversation room.
The left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor where the Lockers are left to the Innovation Theater. The lounge (D) includes the area between the elevator and the front door, and the Staff area (F) includes the region on the right side of the building where staff offices are located.

This study site is specifically designed to help individuals with MCI to lead better lives. It is a one-of-a-kind project designed based on a series of goals: promoting social interaction, environmental exploration, spatial flexibility, safety, independent learning of everyday tasks (e.g., cooking), contact with nature, exercise, and cognitive stimulation in individuals diagnosed with MCI. The study spaces is adjustable and equipped with technologies like tunable lighting and controllable zone-based sound systems to experiment with achieving these goals. Designing healthcare facilities for individuals living with MCI poses challenges for architects as it requires unique design considerations that differ from those required for cognitively healthy older adults and dementia patients~\cite{challenge_arch_2020}. 
While people with MCI also experience cognitive decline, their condition is less debilitating than that of dementia patients~\cite{Gauthier2006_classic}.

\subsection{Distributed Camera Network using Edge Computing}

\input{figure/camera_config}

Edge computing-based camera devices are installed in the ceiling of the study site and integrated with a server infrastructure. This system is described in this section. 

\subsubsection{Camera Configuration}
We installed 39 low-cost ($<\$500$) edge computing and camera devices in the study site as shown in \autoref{fig:camera_config}. The camera devices consist of a camera sensor (Sony IMX219 8-megapixel sensor) and a Google Coral TPU USB Accelerator attached to an edge computing system. The Google Coral TPU USB Accelerator enables deep learning models to run in real-time on the edge computing system. 

Each edge computing system and camera device runs a multi-person 2D pose estimation model~\cite{papandreou2018personlab} in real-time (\autoref{fig:camera_config}, b). Poses are estimated at a frame rate of 1Hz. The poses obtained from this pose estimation model, as well as human bounding box images, are stored for further downstream processing. The raw video frames are discarded. Thus, personally identifiable data is not stored or used for downstream computation, which preserves the privacy of individuals in the study site.  

The edge computing and camera devices are placed and hidden in the ceiling panel and connected to power and network sources using extension cables in the existing infrastructure (\autoref{fig:camera_config}, c).
Depending on the accessible power and network sources, some locations, such as kitchen or staff areas, are covered by multiple cameras, and other locations, such as long corridors, are covered by single or two cameras. 
Yet, the placement location (\autoref{fig:camera_config}, (a), \textcolor{blue}{BLUE}) and viewpoints (\autoref{fig:camera_config}, (a), \textcolor{red}{RED}) of 39 camera devices could still cover entire study site where subject agreed to monitor their activities.
% are shown in \autoref{fig:camera_config} (a), where the gradient from white to blue depicts the direction of viewpoits of the camera devices. \hyeok{Update with the new figure.}

% In total, 39 camera sensors (Sony IMX219 8-megapixel sensor; \textcolor{blue}{BLUE}) are installed with the field of views (\textcolor{red}{RED}) covering the entire indoor space

\input{figure/compute_config}

\input{figure/overall_method.tex}

\subsubsection{Secure Computing Network Architecture}

The overall computing configuration consists of 4 primary segments: the cloud server, the on-premise fog server, the private edge computing networking infrastructure, and the 39 edge computing camera devices. This configuration is shown in \autoref{fig:compute_config}.

The 2D poses, which consists of 17 keypoints based on the MS COCO format~\cite{lin2014microsoft}, and bounding boxes estimated by the edge computing camera devices are stored on a Health Insurance Portability and Accountability Act (HIPAA)-compliant and privacy-preserving data storage server at the study site.
The bounding box images are only temporarily stored for one hour on the fog computing node for estimating body orientations and are not transferred to the cloud computing nodes. However, the 2D poses and the processed body orientation estimation results are stored for permanent data management and analysis.

The fog computing node store one day's worth of data between 8 AM and 7 PM, when visitors are present.
In addition to body orientation estimation, additional activity analysis is carried out by fog computing node, which includes multi-person localization and tracking of the day's data.
The on-premise fog server for the edge computing network contains 2 10Gb SFP+ Ethernet interfaces, which are bonded together into a single 20G interface and connected to the switches used for the private edge computing network. 
This bonded interface is used to provide enough bandwidth that the multiple edge computing systems deployed within the study site are able to write the collected data back to the on-premise fog server for storage without creating a severe network bottleneck. 
The collected data and the performed analysis results are synced nightly approximately between 12 PM and 7 AM to a cloud node's privacy-preserving data server for permanent storage. The duration for nightly sync can change depending on the data size collected over the day.
Our data management framework demonstrates that the activities in study sites are passively and continuously collected with minimal privacy risks. Furthermore, the cameras installed above visitors' eyesight makes it easier for visitors to comply with the proposed instrumentation of cameras for activity monitoring. 

The networking infrastructure consists of a set of 2 interconnected Supermicro SSE-G3648B switches running Cumulus Linux 3.7.12, which have been programmatically bonded together so that they will act as a single large switch while improving throughput, as one half of the 20G bond is connected to each switch.
Thus, either one can be used to pass traffic between the on-premise fog server and the edge computing systems. 
Each edge computing system is connected to one of the two switches via a 1Gb Ethernet connection, as the maximum speed on the Network Interface Card built into the edge computing systems is only 1Gb. 
To prevent data breaches or leaks of sensitive data, the entire edge computing network is isolated from the on-premise network. The only connections to the switches are by the on-premise fog server and the edge computing systems themselves.

To facilitate the operation of all the edge computing systems on the data collection network, the on-premise fog server provides Dynamic Host Configuration Protocol (DHCP) and Network Time Protocol (NTP) services to assign the edge computing systems with their appropriate Internet Protocol (IP) addresses and provide them with the correct date and time when they boot up; to ensure that the same edge computing system receives the same address each time, the addresses are manually specified in the DHCP server’s configuration based on the Media Access Control (MAC) address of the edge computing system. 
The on-premise fog server also acts as a gateway to allow the edge computing systems to reach the cloud network if needed for software update purposes, while acting as a firewall to prevent others on the cloud network from having direct access to the edge computing systems. 
A Network File System (NFS) volume is configured on the fog server and shared with the private edge computing network so that the edge computing systems can mount a shared network volume for the purposes of operation and data storage.
Each edge computing system’s base image is programmed to connect to the on-premise fog server at a known static IP address and mount the NFS volume at boot-up. 
This allows for software and functionality changes in the on-premise fog server to be deployed across all edge computing systems on the network by simply modifying the shared configuration to reflect the desired operation.
When edge computing systems are rebooted, they launch a shared bootstrapping script, which is located on this NFS volume, so that they will load the environment and run the script.

For storage, the on-premise server has 6 $12TB$ storage disks configured in a RAID10 configuration for $\sim32TB$ of usable space.
RAID10 was selected to provide the fastest available speeds while still allowing for disk redundancy in the event of a failure. 
The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network.
As the on-premise fog server is deployed in the study site, it is not directly connected via 10G Ethernet to the cloud server’s private network. 
This means the intermediate network links between the fog node and the cloud node's network are not guaranteed to all be at the maximum speed supported by either endpoint, thereby resulting in slower network speeds than a direct connection.
The transfer process is performed from the on-premise fog server by using Tape ARchive (TAR) to combine all of one day’s data collection files into a single data stream, which is then transmitted over Secure Shell (SSH) to a gateway server dedicated to large data transfers on the cloud server’s main network.
The data transfer stream is then untarred and the files are placed in the designated location on the cloud server’s filesystem. 
The usage of this single stream reduces the number of individual network I/O operations that need to be performed during the transfer process (thus improving performance) when compared to other transfer options like rsync or scp operating on individual files.
It also removes the need to manually stage the tar file on the server prior to transfer as the output of tar is piped directly to the remote system and an untar process via SSH. 


\subsection{Monitoring Movement in Built-in Environment}

\subsubsection{Overall Pipeline}

Here, we describe our approaches to continuously localize and track multiple people in the study space with the abovementioned computing and camera infrastructure.
The overall approach for multi-view multi-person tracking is shown in \autoref{fig:overall_method}.
Based on pose detection and human bounding boxes, each person's location and body orientation are estimated and projected on a 2D coordinate system representing the study space.
Multiview integration then resolves duplicate samples across cameras from overlapping views by combining samples from 39 cameras.
Lastly, a multi-person tracking algorithm~\cite{li2010multiple} is used to track people across the frames.

\subsubsection{Preprocessing 2D poses}
\label{sec:preproc_poses}

\input{figure/tracker}

The 2D poses estimated on the edge computing systems are first preprocessed to remove noisy samples.
Two major artifacts were observed for the detected poses from the pose detection model~\cite{papandreou2018personlab}: non-human poses and temporal inconsistencies.
First, the model considers patterns on the walls and floor as humans due to the way the camera views the area from the ceiling.
These non-human poses remain stationary over time and do not change rapidly.
Thus, we remove those false positives (non-human samples) by identifying poses in subsequent frames where pose changes are near zeros.
Second, 2D poses lack temporal consistency since the model estimates poses frame-by-frame. 
It was observed that a number of poses had their left and right sides flipped or missing %\chaitra{Do you mean the pose was missing altogether?}\hyeok{yes.}
between frames (false negatives).
We used Kalman filter-based temporal smoothing to denoise and fill missing detections~\cite{10.1115/1.3662552}.
For the Kalman filter, linear constant model was used for modeling temporal changes in keypoint locations of COCO poses, which have 17 keypoints~\cite{lin2014microsoft}, $X_t=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}, \dot{u}_1 \dot{v}_1, \dot{u}_2 \dot{v}_2, \cdots, \dot{u}_{17} \dot{v}_{17}]$, where $u$ and $v$ are $x$ and $y$ location of each keypoint and $\dot{u}$ and $\dot{v}$ are the velocity of location changes.

Kalman smoothing for 2D poses is achieved by using Kalman filter-based multi-person tracking technique that has been widely adopted in the past~\cite{bewley2016simple}.
As shown in \autoref{fig:kalman_tracker} (a), the tracker follows predict, detect, match, update, and repeat operations.
Given multi-person tracking until time $t-1$, Kalman filter trackers make predictions of each person's location at time $t$. 
To update the prediction based on actual detections at time $t$, the Hungarian method is used to find matches between predictions and detections from 2D poses~\cite{kuhn1955hungarian} (\autoref{fig:kalman_tracker}, b).
Hungarian methods are widely used to find matches between two groups of samples because of their efficiency and effectiveness~\cite{perera2006multi,bewley2016simple,xu2020train}.
For Hungarian matching, we generate a bipartite graph where each node is 2D pose from prediction and detection at time $t$ and the edge is $L_2$-norm distance between those 2D poses.
The bipartite graph is represented as a matrix, where $C_{i,j}= \|P^i_{p} - P^j_{d} \|_2$ is $L_2$-norm distance between $i$th pose from predictions, $P_p$,  and $j$th pose from detections, $P_d$. 
% and $P=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}]$.
The Hungarian method then finds the matchings (or edges) with the smallest sum of distances between the samples from predictions and detections (\autoref{fig:kalman_tracker} (b), \textcolor{red}{red} lines).
Specifically, Hungarian method optimizes:

\begin{equation}
    Y = \arg\min_{Y} \sum_i \sum_j C_{i,j} Y_{i,j}
\end{equation}

\noindent where $Y$ is a boolean matrix, showing assignment within $C$.
Next, The predictions get updated with the matched detections.
For the unmatched detections, a new tracker is initiated (\autoref{fig:kalman_tracker} (a), \textcolor{red}{red}).
In the case of false negatives (no detections in time $t$), we skip the update operation and continue with the prediction, which is kept alive for 10 seconds to handle potential false negatives.
Until the tracking is complete, this process is repeated.
Lastly, we apply kalman smoothing with Rauch-Tung-Striebel (RTS) smoother to optimize the temporal consistency of estimated 2D pose movements based on all trackers over time~\cite{chan2011implementation}.
Using these processed 2D poses, we can now localize people for the corresponding locations in the study site and track them based on multiple viewpoints.

\subsubsection{Indoor Localization}

Our indoor localization technique aims to locate people within the study site in 2D coordinate space based on the 2D poses detected from each camera.
The middle of the left and right feet is defined as the location of people in a scene.
As the floor in our study space is flat, any detected people in a scene are on the same plane.
With this in mind, we learn a perspective transformation matrix, $M\in \mathbb{R}^{3\times3}$, that can project the foot location from the floor in 2D camera space to the corresponding floor location in the 2D coordinate of the study site~\cite{sun2019see,cosma2019camloc}.

\begin{equation}
    \begin{bmatrix}
        x \\ y \\ 1
    \end{bmatrix}
    = \begin{bmatrix}
        m_{11} & m_{12} & m_{13} \\
        m_{21} & m_{22} & m_{23} \\
        m_{31} & m_{32} & m_{33}
    \end{bmatrix}
    \begin{bmatrix}
        u \\ v \\ 1
    \end{bmatrix}  
    \label{eqn:perspective_mat}
\end{equation}

\noindent where $[x, y]$ is the foot location in study site coordinate and $[u, v]$ is the foot pixel location in the camera.
From every 39 cameras, we learn $M$ by manually selecting 4 corresponding points in the 2D coordinate study site and the pixel locations in the field of view of a camera~\cite{abdel2015direct,shim2015mobile}.
The derived $M$s for each camera are deployed to localize the feet locations of detected 2D poses in the study space coordinate. 
% unless the camera location or orientation is changed.

\subsubsection{Body Orientation Estimation}

\input{figure/multi-view_integration.tex}

The facing orientation of people in a group activity gives important insights into their relationship and engagement with each other~\cite{cristani2011social,barua2021detecting}.
From the human bounding box from 2D pose detection models, we extract the facing direction of each person in the transverse plane, whose orientation is then transformed into the study site coordinates.
For estimating chest facing direction in a human bounding box image, we adopt the deep learning-based body orientation estimation method~\cite{wu2020mebow}. 
Wu~\etal~\cite{wu2020mebow} proposed a deep learning model that combines HRNet~\cite{sun2019deep} and ResNet~\cite{he2016deep} to predict chest facing orientation in 5\degree-intervals from human bounding box images.
The model was trained to learn from multiple tasks, including 2D pose, 3D pose, and body orientation prediction.
This enabled the model to learn the representation that considers 2D and 3D pose geometry and depth information for robustly estimating body orientation from 2D human bounding box images.
Here, we define a human bounding box as a tight square region that contains a detected 2D pose from edge computing systems.
The estimated chest orientation is represented as a 2D chest vector on a transverse plane.
Then, the 2D chest vector in camera space is transformed to the 2D orientation in study site coordinate, $\Vec{v}^t_{world} = R_{camera \rightarrow world}\Vec{v}^t_{world}$.
The rotation matrices, $R_{camera \rightarrow world}$, for each camera is manually defined according to the camera installation in the study site, where north is set as a reference orientation.

\subsubsection{Multi-view Integration}

The 39 cameras installed in the study site have partially overlapping field-of-views to continuously track people across the wide space.
Multiple cameras capture duplicate samples of the same person due to these overlaps.
In order to remove duplicated samples, we detect people across cameras and integrate the detections into a single sample that potentially represents the true location of the person, as shown in \autoref{fig:muti-view_integration}.
To detect those duplicated samples, we generate a graph, $G=(V,E)$, where vertices, $V=\{v_{ci}=(x,y)|c=1,\cdots,39, i=1,\cdots\}$, are locations of all samples from all 39 cameras and edge, $E=\{v_{ci}v_{c'j} |\; c \neq c' \}$, is the connectivity between samples from different cameras that are sufficiently close in the distance.
We assume that duplicates are coming from the same person captured in different cameras, if their euclidean distance is within $\| v_{ci} - v_{c'j} \|_2 \leq 1.5 m$, considering the error margin of our localization technique.
It is possible for the same person located from a different camera to be in a slightly different location from our indoor localization due to lens distortions violating planar assumptions about the floor that can incur inaccuracies in perspective transformations.
% that is used for perspective transformation in our indoor localization technique.
Regardless, we empirically found that only 1.5 meters were sufficient for the margin of the localization error~\cite{zhang2000flexible}.

Once the graph $G$ is constructed, the duplicated samples are identified as those with linked vertices in a graph, which is also called connected components, $CC$, from graph theory~\cite{john1995first}.
Then, we integrate the locations of the duplicated samples considering the camera distance from the detected sample. 
Specifically, when integrating duplicated samples, the samples are penalized when the camera distance is far:

\begin{equation}
    L = \sum_{CC} \frac{1}{d_{ci}} v_{ci}
\end{equation}

\noindent where $L$ is the location of integrated sample and $d_{ci} = \| l_c - v_{ci} \|^2_2$ is the euclidean distance between the sample, $v_{ci}$, and the camera, $l_c$.
According to our findings, the localization error and the distance between the camera and the target person are strongly correlated.
Similarly, the orientation of the duplicated samples is integrated for the vertices in $CC$ considering camera distances.
The multi-view integration results in unique locations, $L=[l_x, l_y]$, and orientation vectors, $o=[o_x, o_y]$, of each person at each time step.  

\subsubsection{Multi-person Tracking}

\input{figure/data_collection.tex}

To understand detailed individual or group movements occurring in the study site, the locations of people need to be tracked across time.
For multi-person tracking, we apply Kalman filter-based tracking for the locations, $L=[l_x, l_y]$, and orientation vector, $O=[o_x, o_y]$, obtained after applying multi-view integration~\cite{kuhn1955hungarian}.
The tracker follows predict, detect, match, update, and repeat steps used in Sec.~\ref{sec:preproc_poses}, but with some differences.
We again use a linear constant model for both location and orientation, where states are represented as location, $L=[l_x, l_y]$, orientation, $O=[o_x, o_y]$, velocity, $\dot{L}=[\dot{l}_x, \dot{l}_y]$, and angular velocity, $\dot{O}=[\dot{o}_x, \dot{o}_y]$.
Furthermore, we assume that people's facing orientation follows their walking direction closely.
Therefore, the tracker estimates facing orientation at time $t$ by summing up both moving directions, the velocity when 1 Hz, $\dot{L}$, and angular velocity, $\dot{O}$.

\begin{equation}
    O_t= O_{t-1} + w\cdot \dot{L}_{t-1} + dt\cdot \dot{O}_{t-1}
\end{equation}

\noindent where $w=0.1$ is a weighting of moving direction (or velocity) on current orientation and $dt$ is the time interval between frames, which is 1 sec.
When associating predictions and matching using Hungarian matching, the bipartite graph is represented as a matrix, where $C_{i,j}= \|L^i_{p} - L^j_{d} \|_2$ is euclidean distance between $i$th sample from prediction, $L_p$, and $j$th sample from detection, $L_d$.
Likewise earlier, we applied RTS smoothing for finished trackers to consider temporal dynamics across the entire trajectory of a person.

\subsection{Benchmark Data Collection}\label{sec:benchmark_data_collection}

To evaluate the performance of the localization, body orientation estimation and tracking methods detailed above, we produced a manually annotated dataset which consists of four to five subjects moving and interacting in defined ways at the study site described above.
The benchmark dataset includes a group of people 1) walking together, 2) walking past each other, or 3) conversing in place while changing facing orientations. 
 
In order to accurately annotate the location and corresponding time stamp of the subjects, we taped the entire space with 1-meter markers. 
The subjects were asked to walk according to pre-planned group formations and walking paths.
While people were walking, an observer annotated the exact time and location of each subject at each second.
The observer manually annotated the body orientation of the subjects using north (upper direction for \autoref{fig:ep6_func}) as a reference.



Below we describe three datasets that we created to capture different types of activities in the space.

\subsubsection{4 People Walking around Entire Space}

Our first benchmark dataset has four people walking around the study site.
\autoref{fig:data_collection} describes the locations and paths taken by participants while collecting the benchmark datasets to consider the realistic use cases of the study site by visitors. For the benchmark datasets, we covered areas that are of interest for tracking behaviors in the study space (\autoref{fig:data_collection}, a). 
Those include locations mainly used by the visitors for eating (dining, kitchen), physical exercises, lounge, and staff zones (\autoref{fig:ep6_func}), where subjects agreed to their behaviors being captured.

For the annotation, we selected the closest 1-meter markers as the ground-truth location of the subjects while they were walking, which resolution was sufficient to consider the varying foot size and stride length of each participant.
While walking, we also changed the group formation to simulate realistic movement in the space (\autoref{fig:data_collection}, c).
For the wider corridors, group formations of two or three people walking side-by-side were used whereas in narrow corridors multiple subjects walked in straight lines. Walking in groups helped to test the effect of occlusions, where subjects are not seen from a camera viewpoint.

\subsubsection{5 People Walking Past Each other}

We also collected a benchmark dataset when multiple subjects show more complex movements.
Shown in \autoref{fig:data_collection} (b), we simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions that frequently occurs while performing dancing or group exercises.

\subsubsection{5 people Changing Orientations in Place}

\input{figure/orientation_inplace}

People often sit or stand stationary while having group conversations and only change facing directions to interact.
To this end, we collected a benchmark dataset to evaluate how well body orientation estimation performed when people make subtle changes in facing orientation in place, as shown in \autoref{fig:ori_in_place}.
From Session 1 to 3, we increased the size of the social group from two to five. 
A social group is defined as people actively communicating at a distance closer than 2 meters, considering social distancing due to the ongoing pandemic.
According to instructions, participants gradually changed the facing direction. 
%by switching whose members were communicating with whom.


\subsection{Evaluating Multi-person Tracking and Localization}

We evaluate our multi-view multi-person tracking systems with respect to localization, tracking, and body orientation estimation performances following the standard evaluation methods~\cite{bernardin2006multiple,wu2020mebow}.
As there is no single metric for evaluating multi-person tracking methods, we utilize the following metrics to understand the performance of the proposed system~\cite{dendorfer2020mot20}.
$\uparrow$ and $\downarrow$ are shown for the metrics that are higher or lower the better, respectively.

\begin{itemize}
    \item MOTA $\uparrow$ (Multi-Object Tracking Accuracy) combines three kinds of error sources, which are false positives, missed targets, and identity switches.    
    \item IDF1 $\uparrow$ (ID F1 score) is the ratio of correctly identified detections over the average number of ground-truth and computed detections.
    \item MT $\uparrow$ (Mostly Tracked targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at least 80\% of their respective life span.
    \item ML $\downarrow$ (Mostly Lost targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at most 20\% of their respective life span.
    \item FPR $\downarrow$ (False Positives Rate) measures the average number of false alarms per frame.
    \item FNR $\downarrow$ (False Negatives Rate) measures the average number of missed targets per frame.
    \item Rcll $\uparrow$ (Recall) measures the ratio of correct detections to the total number of ground-truth locations.
    \item Prcn $\uparrow$ (Precision) measures the number of detected objects over the sum of detected and false positives.
    \item IDSR $\downarrow$ (ID Switch Ratio) measures the number of ID switches (IDS) over recall.
    \item Frag $\downarrow$  (Fragmentation) measures the total number of times a trajectory is fragmented, which are interruptions during tracking.
\end{itemize}

Specifically, $MOTA=1-\frac{\sum_t FN_t + FP_t + IDS_t}{\sum_t GT_t}$,
where $FN_t$, $FP_t$, $IDS_t$, and $GT_t$ are false negatives (misses), false positives, ID switches, and ground-truths at time $t$.
One important evaluation that preceded tracking is detection. 
In this work, we define a ground-truth target at the time $t$ is detected if the estimated sample location is within 1.5 meters in euclidean distance.
Otherwise, the target is considered as \textit{missed}. 
The 1.5-meter reference is based on the fact that people rarely walk faster than 1.42 m/s on an everyday basis~\cite{browning2006effects,mohler2007visual,levine1999pace}.

To demonstrate the localization accuracy of the estimated samples, we also report multiple object tracking precision, $MOTP=\frac{\sum_{i,t} d^i_t}{\sum_t c_t}$.
$d^i_t$ is the euclidean distance between the $i$th detected ground-truth sample and estimated sample, and $c_t$ is the number of detection at time $t$. 
In other words, MOTP is the average euclidean distance error for the detected samples, which shows the performance of the proposed systems to estimate the precise location of target samples that is independent of tracking trajectories or ID switches.

\subsubsection{Multi-person Tracking Baseline}

Our proposed tracker is compared with a Hungarian matching-based tracker~\cite{kuhn1955hungarian}, which only considers frame-by-frame matching between 2D pose detections, in order to illustrate the importance of modeling temporal dynamics of 2D movements.
Based on the results of multiview multi-person localization at time $t$ and $t+1$, the Hungarian tracker generates a bipartite graph with nodes representing samples from two consecutive timesteps and edges representing Euclidean distances between samples. 
Since our tracking rate is 1 Hz, we remove any edge distance larger than 1.5 meters in the created bipartite graph, as people normally walk 1.42 m/s in everyday activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
Then, the Hungarian method finds the matchings (or edges) that have a minimum sum of Euclidean distances.
Potentially missing samples (false negatives) in a frame $t$ are filled in by linearly interpolating the matched detection from frame $t-1$ and $t+1$.
The Hungarian matching is applied until no matching is found any longer over time.

\subsection{Evaluating Body Orientation Estimation}

Our benchmark dataset and the proposed method represent the body orientation as a continuous angle.
Following the standard definition of body orientation in the previous work~\cite{wu2020mebow,yu2019continuous,andriluka2010monocular}, we defined the human orientation $\theta \in [0\degree, 360\degree)$ as the chest facing direction on the transverse plane that is projected to the 2D coordinate in the study site, where the north (top) direction is the reference with clock-wise rotation.
Following previous work, we use two metrics: Mean Absolute Error (MAE) of angular distance and Accuracy-$X\degree$~\cite{wu2020mebow}.
Accuracy-$X\degree$ is defined as the ratio of the samples that are predicted within the deviation of $X\degree$ according to the ground-truth orientation. 
By using $X\in [0\degree, 180\degree]$, Accuracy-$X\degree$ measures fine-grained model accuracy.

\subsubsection{Comparing Body Orientation Estimation Baselines}

Our body orientation method inherently learns the geometric relationship between 2D pose, 3D pose, and the corresponding body orientation of the observed human bounding box.
We compare the proposed method with two baselines that only use 2D information and then a baseline that only models the 3D geometry of detected 2D poses.
Through this practice, we will demonstrate the importance of modeling both 3D geometry and pose-body orientation relationships.

\noindent i) \textit{2D pose-based Heuristic Approach:}
This method uses a heuristic approach to estimate body orientation from only 2D pose information.
Specifically, it uses 2D facial keypoints, including nose, eyes, and ears, and estimates the 2D vector originating from the average of left and right eyes and ears keypoints to nose keypoints on 2D image pixels.
We directly project those 2D vectors from the image frame to the 2D coordinate space of the study site using a perspective transformation matrix, $M$, derived from \autoref{eqn:perspective_mat}.

\noindent ii) \textit{2D pose-based Deep Learning Approach:}
This baseline model applied a learning-based method, where the model directly estimates body orientation from 2D pose input.
We used a graphical convolutional network (GCN)~\cite{yan2018spatial} to process 2D pose data to predict body orientation angle in 5-\degree intervals.
For training the model, we used MS COCO 2D keypoints~\cite{lin2014microsoft} dataset and the corresponding body orientation annotation provided by  Wu~\etal~\cite{wu2020mebow}.
We augmented 2D keypoints input by randomly flipping horizontally or adding Gaussian noises to simulate noisy pose detections from our pipeline.

\noindent iii) \textit{ 2D-3D pose Geometric matching-based Approach:}
To model the 3D geometry of the human body pose~\cite{takahashi2018human}, we first estimated 3D pose information from the detected 2D poses from our pipeline.
We lift the estimated 2D poses to 3D poses by using the 3D pose estimation method~\cite{pavllo20193d}.
Then, the 3D poses are calibrated according to the camera viewpoint using Perspective-n-point projection technique~\cite{lepetit2009epnp}.
Specifically, at each time step $t$, we learn the extrinsic parameters, which are rotation and translation matrices, of the estimated 3D chest keypoints (left and right shoulders and left and right pelvis) for projecting 3D pose to the corresponding 2D keypoints in the image space. 

\begin{equation}
    [R|T]^t = \arg\min_{R,T}\| p^t_2 - sK[R|T]p^t_3 \|
\end{equation}

\noindent where $R\in\mathbb{R}^{3\times 3}$ is a rotation matrix subject to $R^TR=I\in\mathbb{R}^{3\times3}$ and $det(R) = 1$ and $T\in\mathbb{R}^{3\times 1}$ is a translation matrix that minimizes the projection error of chest keypoints of 3D pose, $p^t_3$, to 2D pose, $p^t_2$, at timestep $t$ given intrinsic camera lense parameter, $K\in\mathbb{R}^{3\times 3}$.
We fix the camera intrinsic matrix, $K$, with the parameters provided by the manufacturer~\cite{rpi_camera} and the scale parameter is arbitrarily set to $s=1$ as we do not require the absolute scale of the 3d pose size, but only the facing direction.
For each person, we smoothed $[R|T]^t$ over all time steps using moving SLERP filter~\cite{shoemake1985animating} and moving average filter for rotation and translation matrices, respectively, to keep the temporal consistency.
From the 3D pose calibrated according to the chest orientation, we acquire the 3D chest norm vector perpendicular to the left-to-right shoulder vector and left shoulder-to-left pelvis vector, $\Vec{v}^t_{chest} = \Vec{v}^t_{L.Shoulder \rightarrow R.Shoulder} \times \Vec{v}^t_{L.Shoulder \rightarrow L.Pelvis}$, at each timestep $t$.
The estimated 3D chest norm vector is projected to a 2D chest vector on a transverse plane, which represents the facing of each people in the scene with respect to the camera viewpoint.

\subsection{Impact of Camera Installation on Model Behavior}

\input{figure/cam_install_protocol}

In our study site, the camera installation is determined primarily by the power and network sources reachable using extension cables, with minimum modification to the existing building structure, resulting in 39 cameras unequally installed in the space.
In our experiment, we will examine this in more detail to understand the impact of camera installation on four different factors, shown in \autoref{fig:cam_install_protocol}, related to localization and body orientation estimation accuracy.

\subsubsection{Distance Between Camera and Person}

Across all cameras, we measured the distance between captured people from the camera center, as shown in \autoref{fig:cam_install_protocol} (a), that will be associated with localization and orientation errors.

\subsubsection{Facing Angle with respect to Camera Viewpoint}

We collected the degree of facing directions of the captured person deviating from camera viewpoints, as shown n \autoref{fig:cam_install_protocol} (b), and conducted correlation analysis with the corresponding localization and orientation errors.

\subsubsection{Horizontal Displacement from Camera Center}

We studied the impact of the horizontal displacement of the captured person from the camera center (\autoref{fig:cam_install_protocol}, c).
We quantified the horizontal displacement as the horizontal angle, $\theta\degree_H$, of the person from the camera center that is normalized by horizontal field-of-view, $\theta\degree_{H_{FOV}}$, which is normalized horizontal angle, $\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$.
As a person gets closer to the horizontal center of the camera, the normalized horizontal angle approaches zero.
The normalized horizontal angle increases to $1$ when the person is at the edge of the frame. 
When the value is larger than $1$, then only part of the body is observable from the camera.
We examine how localization and orientation errors vary with the degree of horizontal displacement.

\subsubsection{Vertical Displacement from Camera Center}

Following horizontal displacement, we studied the effect of vertical displacement of a person from the camera center (\autoref{fig:cam_install_protocol}, d).
The vertical displacement was quantified as a vertical angle, $\theta\degree_V$, of the person captured from the camera center that is normalized by vertical field-of-view, $\theta\degree_{V_{FOV}}$, referring to the camera datasheet, namely normalized vertical angle, $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$.
We specifically consider the foot location, which we use to localize, as a point of reference to calculate the normalized vertical angle.
When the person is closer to the camera, the normalized vertical angle increases, and only the upper body is partially captured by the camera due to the limited vertical field of view.
On the other hand, as the person moves away from the camera, the normalized vertical angle decreases and can capture the full body in the field of view, but with the cost of increased distance between the camera and the person.
Likewise, in the above-mentioned analysis, we will study the changes in localization and orientation errors based on the vertical displacement of the captured person.


==> sections/method/_main_old.tex <==
%-------------------
% Old method with Hungarian Tracking + Linear Interpolation + 2D-3D matching-based orientation estimation
%-------------------

\section{Method}

The proposed work localizes and tracks multiple people with their body orientations in a built-in environment by using distributed camera network installed with edge and fog computing environment.
In this section, we first provide overall computing environment in our system and describe the approach to continuously monitor people's movement in the space.

\subsection{Distributed Camera Network using Edge Computing}

\input{figure/camera_config}

\subsubsection{Camera Configuration}

\autoref{fig:camera_config} illustrates camera installation of the study site, which area spans 18,286 square feet space. 
The study site that is instrumented with 39 cameras to cover 18,286 square feet space (\autoref{fig:camera_config} (a)).
Each camera is attached in the ceiling with the viewpoints of darker blue side (\autoref{fig:camera_config} (b)). 
the camera sensor (Sony IMX219 8-megapixel sensor) is installed in the Raspberry Pi 4 that has Google Coral USB Accelerator to run deep learning-based 2D pose estimation model in real time (\autoref{fig:camera_config} (c)).
Raspberry Pis are place on the ceiling connect to the power and network source in the infrastructures.
By using a low cost (<\$500) Raspberry Pis having camera, we could install as many as possible cameras in the study sites with existing power and network ports.
39 cameras sufficiently cover the wide space, where our localization algorithm could detect and localize people across the space with around 1 meter error, which is within the acceptable error margin to understand activities in the study space.

\input{figure/compute_config}

\subsubsection{Computing Network Architecture}

The overall configuration consists of 4 primary segments: the cloud server, the on-premise fog server, the private Pi networking infrastructure, and the Pis themselves.
Our computing environment is illustrated in \autoref{fig:compute_config}, which include 39 Raspberry Pis, one Fog computing node on the study site, and one cloud computing node off the study site.
To preserve privacy of people in the space, Rapsberry Pi runs multi-person 2D pose estimation on the fly without storing the potentially sensitive video data on device, which can significantly reduce the risk of data breach.
The 2D pose estimation occurs every second, thus 1 Hz frame rate, and, if 2D pose detected from any of Raspberry Pi, the 2D keypoint information is directly transferred and stored into the Fog computing node that has HIPPA-compliant data storage server on the study site.
The Fog computing node stores a day volume of data typically between 8 AM to 7 PM, where visitors or staffs are active in the building.
Fog computing node also processes the additional activity analysis on the data collected in the previous day, including multi-person localization, tracking, and body-orientation estimation.
The collected data and resulting analysis in the Fog node is transferred to HIPPA-compliant data server in the cloud node for the permanent storage between 9 PM to 7 AM over the night.
As demonstrated in our data analysis and computing framework, the activities in study site is passively and continuously processed with minimum risk on privacy breach.
Additionally, the cameras installed above the height of eye sight during the activities in the space helped visitors and staffs being more compliant with the proposed instrumentation of cameras for activity monitoring.

The on-premise fog server for the Pi network contains 2 10Gb SFP+ Ethernet interfaces which are bonded together into a single 20G interface and connected to the switches used for the private Pi network. 
This bonded interface is used to provide enough bandwidth that the multiple Pis deployed within the study site are able to write their collected data back to the on-premise fog server for storage without creating a severe network bottleneck due to the amount of devices that were planned for deployment. 
The networking infrastructure consists of a set of 2 Supermicro SSE-G3648B switches running Cumulus Linux 3.7.12 which have been programmatically bonded together so that they will act as a single large switch while improving throughput, as one half of the 20G bond is connected to each switch and thus either one can be used to pass traffic between the on-premise fog server and the data collection Pis. 
Each Pi is connected to one of the two switches via a 1Gb Ethernet connection, as the maximum speed on the Network Interface Card built into the Pis is only 1Gb. 
The entire Pi network is isolated from the Cloud network and the only connections to the switches are by the on-premise fog server and the Pis themselves.

To facilitate the operation of all the Pis on the data collection network, the on-premise fog server provides DHCP and NTP services to assign the Pis with their appropriate IP addresses and provide them with the correct date and time when they boot up; to ensure that the same Pi receives the same address each time, the addresses are manually specified in the DHCP server’s configuration based on the MAC address of the Pi. 
The on-premise fog server also acts as a gateway to allow the Pis to reach the cloud network if needed for software update purposes, while acting as a firewall to prevent others on the cloud network from having direct access to the Pis. 
An NFS volume is configured on the server and shared with the private Pi network so that the Pis can mount a network volume in an on-premise fog server for the purposes of operation and data storage; each Pi’s base image is programmed to connect to the on-premise fog server at a known static IP address and mount network NFS volume at boot up. 
This allows for software and functionality changes in the on-premise fog server to be deployed across all Pis on the network by simply modifying the shared configuration to reflect the desired operation and then rebooting the Pi so that it will load the environment and run the script.

For storage, the server has 6 12TB storage disks configured in a RAID10 configuration for ~32T of usable space; RAID10 was selected to provide the fastest available speeds while still allowing for disk redundancy in the event of a failure. 
The largest hurdle in this process is the transfer of the collected data to the on-premise fog storage location on the cloud server’s main network; as the on-premise fog server is deployed in a remote location at the study site, it is not directly connected via 10G Ethernet to cloud server’s private network and the data must traverse the general virtual private network which at this time only runs at 1G speeds. 
The transfer process is performed from the on-premise fog server by using tar to combine all of a day’s data collection files into a single data stream which is then transmitted over SSH to a gateway server dedicated to large data transfers on the cloud server’s main network, where the stream is then untarred and the files placed in the appropriate location on the cloud server’s filesystem. 
The usage of this single stream reduces the number of individual I/O operations that need to be performed during the transfer process (thus improving performance) when compared to other transfer options like rsync or scp operating on individual files, while removing the need to manually stage the tar file on the server prior to transfer as the output of tar is piped directly to the remote system and an untar process via SSH. 

\subsection{Monitoring Activities in Built-in Environment}

\input{figure/overall_method.tex}

Here, we describe our approaches to continuously monitor activities of multiple people in our study space with the abovementioned computing and camera infrastructure.
The overall approach for multi-view multi-person tracking is shown in \autoref{fig:overall_method}.
From the pose detection samples from each camera, the location and body orientation of each person is estimated and projected on 2D coordinate of the study space.
Then, the multi-view integration combines the samples from 39 cameras to resolve duplicated samples across cameras.
Lastly, multi-person tracking algorithm~\cite{kuhn1955hungarian} is used to track people across the frames.

\subsubsection{Indoor Localization}

The aim of indoor localization is to find the exact location of person in the scene from each camera in 2D coordinate space of the study site.
Here, we define the middle of left and right feet locations as the location of people in the scene.
Our assumption in the the floor of the study site is flat, and we first learn a perspective transformation matrix, $M\in \mathbb{R}^{3\times3}$, that can project the foot location in the 2D camera space to the corresponding location in study site~\cite{sun2019see,cosma2019camloc}.
\begin{equation}
    \begin{bmatrix}
        x \\ y \\ 1
    \end{bmatrix}
    = \begin{bmatrix}
        m_{11} & m_{12} & m_{13} \\
        m_{21} & m_{22} & m_{23} \\
        m_{31} & m_{32} & m_{33}
    \end{bmatrix}
    \begin{bmatrix}
        u \\ v \\ 1
    \end{bmatrix}  
\end{equation}
where $[x, y]$ is the point location in study site coordinate and $[u, v]$ is the pixel location in the camera.
For 39 cameras, we select 4 corresponding points in study site and the pixel locations in the field of views to learn $M$~\cite{abdel2015direct,shim2015mobile}.
Once $M$ is derived, they are fixed and used to localize the feet locations of detected people in the study site unless the camera location or orientation is changed.

\subsubsection{Body Orientation Estimation}

Detecting the facing of people in group activity provides a important clue about the relationship and the engagement of each people in the social interaction.
From 2D poses detected from multiple people in the scene, we detect the facing of the chest direction with respect to the camera, which is then projected to the 2D coordinates for the study site.
Estimating the orientation in the space requires having 3D information.
We lift the estimated 2D poses to 3D pose by using 2D pose-based 3D pose estimation method~\cite{pavllo20193d}.
Then, the 3D poses are calibrated according to the camera viewpoint using Perspective-n-point projection technique~\cite{lepetit2009epnp}.
Specifically, at each time step $t$, we learn the extrinsic parameters, which are rotation and translation matrices, for the estimated chest keypoints, including left and right shoulders and left and right pelvis, of 3D pose to project to the corresponding 2D keypoints in the image space. 

\begin{equation}
    [R|T]^t = \arg\min_{R,T}\| p^t_2 - sK[R|T]p^t_3 \|
\end{equation}

\noindent where $R\in\mathbb{R}^{3\times 3}$ is a rotation matrix subject to $R^TR=I\in\mathbb{R}^{3\times3}$ and $det(R) = 1$ and $T\in\mathbb{R}^{3\times 1}$ is a translation matrix that minimizes the projection error of chest keypoints of 3D pose, $p^t_3$ to 2D pose, $p^t_2$ at timestep $t$ given intrinsic camera lense parameter, $K\in\mathbb{R}^{3\times 3}$.
We fix the camera intrinsic matrix, $K$, with the parameters provided from the manufacturer~\cite{rpi_camera} and scale parameter is arbitrarily set as $s=1$ as we do not require absolute scale of the 3d pose size, but only the facing direction instead.
For each person, we smoothed $[R|T]^t$ over all time steps using moving SLERP filter~\cite{shoemake1985animating} and average filter for rotation and translation matrices, respectively, to keep the temporal consistency.

From 3D pose calibrated according to the chest orientation, we acquire 3D chest norm vector perpendicular to left-to-right shoulder vector and left shoulder-to-left pelvis vector, $\Vec{v}^t_{chest} = \Vec{v}^t_{L.Shoulder \rightarrow R.Shoulder} \times \Vec{v}^t_{L.Shoulder \rightarrow L.Pelvis}$, at each timestep $t$.
The estimated 3D chest norm vector is projected to 2D chest vector on transverse plane, which represents the facing of each people in the scene with respect to camera view-point.
The 2D chest vector in camera space is transformed to the 2D orientation in study site coordinate, $\Vec{v}^t_{world} = R_{camera \rightarrow world}\Vec{v}^t_{world}$.
The rotation matrices, $R_{camera \rightarrow world}$, for each camera is manually defined according to the camera installation in the study site, where north is set as a reference orientation.

\subsubsection{Multi-view Integration}

\input{figure/multi-view_integration.tex}

39 cameras installed in study sites shares field-of-views to continuously track people over the space, and overlapping field-of-views generates duplicated samples of a same person across multiple cameras.
To remove duplicated samples, we detect those duplicates across cameras and integrate duplicated samples into a single sample that represents the corresponding person as shown in \autoref{fig:muti-view_integration}.
To detect those duplicated samples, we generate a graph, $G=(V,E)$, where vertices, $V=\{v_{ci}=(x,y)|c=1,\cdots,39, i=1,\cdots\}$, are locations of all samples from all 39 camera and edge, $E=\{v_{ci}v_{c'j} |\; c \neq c' \}$ is the connectivity between samples from different cameras that are close enough in distance, which samples can be considered to be originated from the same person captured in different cameras.
We use euclidean distance as a distance between two samples, and $\| v_{ci} - v_{c'j} \|_2 \leq 1.5 m$ is considered as threshold for the connectivity between the samples.

The same person from different camera can be in slightly different location from our indoor localization as the boundaries of field-of-view violates planar assumption of the floor of the study site captured in the camera image due to the lense distortions that is used for perspective transformation in our indoor localization technique.
We empirically found that 1.5 meter was sufficient margin of error regardless of those potential inaccuracies in perspective transformations~\cite{zhang2000flexible}.
Once the graph, $G$ is construct, the duplicated samples are linked vertices in a graph, which is also called connected components, $CC$, in graph theory~\cite{john1995first}.
Then, we integrate those duplicated samples by averaging the locations of the samples, $v_k = \frac{1}{N}\sum_{CC} v_{ci}$.
The orientation of the duplicated samples are averaged from the vertices in $CC$ likewise for the integrated sample.

\subsubsection{Multi-person Tracking}

To understand detailed activities across, the location of people in each time step needs to be tracked across time.
For multi-person tracking, we apply Hungarian method~\cite{kuhn1955hungarian}, which is widely used due to its extreme effectiveness and efficiency~\cite{perera2006multi,bewley2016simple,xu2020train}.
Given multi-view multi-person localization results in 2D coordinate of study site at time $t$ and $t+1$, we generate a bipartite graph where each node are samples at two consecutive timesteps and edge is the euclidean distance between samples. 
Specifically, our tracking rate is 1 Hz and we remove any edge distance larger then 1.5 meters in the created bipartite graph, as people normally walk 1.42 m/s in every day activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
The bipartite graph is represented as a matrix, where $C_{i,j}= \|x^i_{t} - x^j_{t+1} \|_2$ is euclidean distance between $i$th sample from time $t$ and $j$th sample from time $t+1$.
Then, Hungarian method finds the matchings (or edges) that has minimum sum of distance between samples from time $t$ and $t+1$.

\begin{equation}
    X = \arg\min_{X} \sum_i \sum_j C_{i,j} X_{i,j}
\end{equation}

\noindent where $X$ is a boolean matrix, showing assignment between $C$.
Lastly, we apply hungarian method along the time and track each person until no matching is found any longer.

The trajectory of a person walking in the space is also used to improve the temporal consistency of the facing orientation.
We integrate frame-by-frame orientation estimation from 3D-2D pose calibation with moving direction of the person.

\begin{equation}
    \Vec{v}^{i,t}_{refine} = w_1\; \Vec{v}^{i,t}_{frame} + w_2\; \Vec{v}^{i,t}_{track}
\end{equation}

\noindent where $w_1 + w_2 = 1$ and $w_1, w_2 \geq 0$.  
We set $w_1 \ll w_2$ as people normaly face to the walking direction while moving.
$\Vec{v}^{i,t}_{frame}$ and $ \Vec{v}^{i,t}_{track}$ are orientations at time $t$ for detected sample $i$ from frame-by-frame estimation and from trajectories, respectively.
The facing orientation from trajectories are derived from the consecutive location of a tracked sample, $\Vec{v}^{i,t}_{track}= \frac{x^i_{t+1} - x^i_t}{\|x^i_{t+1} - x^i_t\|_2} $, where $x^i_t$ and $x^i_{t+1}$ are locations of $i$th tracked sample at time $t$ and $t+1$.


==> sections/method/_main_old_2.tex <==
\section{Method \& Materials}

\input{figure/ep6_func_spaces.tex}

In this work, multiple Raspberry Pi based camera systems are integrated into a distributed network and are installed with edge, fog, and cloud computing environments to locate and track multiple people with their body orientations in a built environment.
This section provides a detailed account of our study site, the computing environment of our system, and the techniques employed to continuously monitor people's movements in a given space.

\subsection{Study Site with Patient-centered Design}
\chaitra{Is it necessary to talk about MCI or the real use case of EP6? I feel it might distract from what the paper is trying to do, which is localization and tracking in an indoor space}

The study site used in this work is a 18,286 square feet indoor environment consisting of various functioning spaces such as a library, kitchen, dining area and gym, as shown in \autoref{fig:ep6_func}.

Referring \autoref{fig:ep6_func} and \autoref{fig:data_collection}, Activity Area (A) includes both the Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and left boundary of conversation room.
The left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor where the Lockers are left to the Innovation Theater.
The lounge (D) includes the area between the elevator and the front door, 
% \chaitra{we have not shown anywhere what the front desk is. Should we change fig 6 to include this?}\hyeok{Replaced this with front door.}
and the Staff area (F) includes the region on the right side of the building where staff offices are located.

Designing healthcare facilities for individuals living with MCI poses challenges for architects as it requires unique design considerations that differ from those for cognitively healthy older adults and dementia patients~\cite{challenge_arch_2020}. 
While people with MCI also experience cognitive decline, their condition is less debilitating than that of dementia patients~\cite{Gauthier2006_classic}.
The study site was a one-of-a-kind project designed based on a series of goals: promoting social interaction, environmental exploration, spatial flexibility, safety, independent learning of everyday tasks (e.g., cooking), contact with nature, exercise, and cognitive stimulation. 
The designed spaces were adjustable and equipped with technologies like tunable lighting and controllable zone-based sound systems to experiment with achieving these goals. 

\subsection{Benchmark Data Collection}\label{sec:benchmark_data_collection}

\input{figure/data_collection.tex}

We produced a manually annotated dataset which consists of four to five subjects engaged in daily activities such as walking or conversing at the study site described above.
The benchmark dataset includes a group of people 1) walking together, 2) walking past each other, or 3) conversing in place while changing facing orientations. 
The proposed localization, tracking, and body orientation estimation system is evaluated using this benchmark dataset. 
In order to accurately annotate the location and corresponding time stamp of the subjects, we taped the entire space with 1-meter markers. 
The subjects were asked to walk according to pre-planned group formations and walking paths.
While people were walking, an observer annotated the exact time and location of each subject at each second.
The observer manually annotated the body orientation of the subjects using north (upper direction for \autoref{fig:ep6_func}) as a reference.

Below we describe three datasets that we created to capture different types of activities in the space.

\subsubsection{4 People Walking around Entire Space}

Our first benchmark dataset has four people walking around the study site.
\autoref{fig:data_collection} describes the locations and formation of groups taken by participants while collecting the benchmark dataset to consider the realistic use cases of the study site by visitors.
For the benchmark dataset, we covered areas that are of interest for tracking behaviors in the study space (\autoref{fig:data_collection}, a). 
Those include locations mainly used by the visitors for eating (dining, kitchen), physical exercises, lounge, and staff zones (\autoref{fig:ep6_func}), where subjects agreed to their behaviors being captured.

For the annotation, we selected the closest 1-meter markers as the ground-truth location of the subjects while they were walking, considering the varying foot size and stride length of each participant.
While walking, we also changed the group formation to simulate realistic movement in the space (\autoref{fig:data_collection}, c).
For the wider corridors, group formations of two or three people walking side-by-side were used whereas in narrow corridors multiple subjects walked in straight lines. Walking in groups helped to test the effect of occlusions, where subjects are not seen from a camera viewpoint.

\subsubsection{5 People Walking Past Each other}

We also collected a benchmark dataset when multiple subjects show more complex movements.
Shown in \autoref{fig:data_collection} (b), we simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions.

\subsubsection{5 people Changing Orientations in Place}

\input{figure/orientation_inplace}

People often sit or stand stationary while having group conversations and only change facing directions to interact.
To this end, we collected a benchmark dataset to evaluate how well body orientation estimation performed when people change orientation in place, as shown in \autoref{fig:ori_in_place}.
From Session 1 to 3, we increased the size of the social group from two to five. 
A social group is defined as people actively communicating at a distance closer than 2 meters, considering social distancing due to the ongoing pandemic.
According to instructions, participants gradually changed the facing direction. 
%by switching whose members were communicating with whom.


%----------

\subsection{Distributed Camera Network using Edge Computing}

\input{figure/camera_config}

\subsubsection{Camera Configuration}
We installed 39 low-cost (<\$500) Raspberry Pi camera systems in the study site
% \robert{The grammar here is off, but I'm not sure the best way to correct it; do we want to refer to just a single unit ["By using a low cost (<\$500) Raspberry Pi"] or the group of units as a whole ["By using low cost (<\$500) Raspgerry Pis"]?}\hyeok{A single unit}
as shown in \autoref{fig:camera_config}, (a).
Raspberry Pis were placed and hidden in the ceiling panel and connected to power and network sources using extension cables in the existing infrastructure.
Depending on the accessible power and network sources, some locations, such as kitchen or staff areas, are covered by multiple cameras, and other locations, such as long corridors, are covered by single or two cameras.
Each camera is attached to the ceiling with the viewpoints toward the darker blue side as shown in \autoref{fig:camera_config} (b). 
The camera sensor (Sony IMX219 8-megapixel sensor) and Google Coral USB Accelerator were installed in the Raspberry Pi 4 to run a deep learning-based 2D pose estimation model in real time (\autoref{fig:camera_config} (c)).
With 39 cameras, our localization algorithm was able to detect and locate people across the large space with a 1.5-meter error 
% \robert{Should this also read "margin of error", or is that redundant because the phrase "error margin" is immediately referenced in the next clause?}\hyeok{Good point. Margin of error for the next clause.}
, which fits within the acceptable margin of error to understand activity in the studied area.
% For the seating areas, we have also asked participants to sit naturally as they communicate with one another.

\input{figure/compute_config}

\subsubsection{Computing Network Architecture}

The overall configuration consists of 4 primary segments: the cloud server, the on-premise fog server, the private Pi networking infrastructure, and the Pis themselves.
Our computing environment is illustrated in \autoref{fig:compute_config}, which includes 39 Raspberry Pis, one fog computing node on the study site, and one cloud computing node off the study site.
% \robert{Should the word "Each" be here, to quantify each Raspberry Pi?}\hyeok{Done.}
Each Raspberry Pi runs multi-person 2D pose estimation on the fly~\cite{papandreou2018personlab}, which reduces the risk of a data breach by not storing potentially sensitive video data on the device.
2D poses are estimated every second, resulting in a frame rate of 1 Hz, and if the 2D pose is detected on any Raspberry Pi, the 2D keypoint and human bounding box \chaitra{note to self: define human bounding box or talk about it before} information is directly transferred and stored on a Health Insurance Portability and Accountability Act (HIPAA)-compliant data storage server at the study site.
% The human bounding box from detected 2D poses are additionally transferred to Fog computing node for analyzing the body orientation of the detected person~\cite{wu2020mebow}.
The bounding box images are only temporarily stored (one hour) in the fog computing node
% \robert{The plural here makes it sound like we have more than one Fog node in our setup; not sure if this sentence is supposed to be referencing deployments of this infrastructure in general (in which case the wording's fine as-is) or specifically our infrastructure. All other references have just been singular, so I don't know if we want to maintain that consistently through the paper or not.}\hyeok{You are correct. It has to be specifically for our infrastructure. So, it has to be singular.} 
for data preprocessing and are not transferred to cloud computing nodes.
We store only the 2D keypoint information, which has 17 keypoints based on MS COCO format~\cite{lin2014microsoft}, 
% \yash{I would mention which version go Posenet we used and how many keypoints we can detect (e.g., maximum of 17 or 33 keypoints)}\hyeok{Done.} 
and the processed body orientation estimation results for permanent data management and analysis.

The fog computing node
% \yash{in the setting that we defined earlier, do we have more than single fog computing node(i.e., the server)?} \robert{In reply to Yash, we do not have anything other than the single server at the site}\hyeok{Correct. This is a typo.} 
store a day's worth of data between 8 AM and 7 PM, when visitors are present.
Additional activity analysis is carried out by fog computing node,
% \robert{Plural; same comments as Yash's and mine above}\hyeok{Corrected.}
which includes body orientation estimation, multi-person localization, and tracking of the previous day's data.
Data collected in the fog node and its analysis is synced nightly approximately between 12 PM and 7 AM to a cloud node's HIPAA-compliant data server for permanent storage. 
The duration for nightly sync can change depending on the data size collected over the day.
% \robert{Our sync's actually scheduled to start after midnight as it calculates the previous day's date in order to perform the sync; it also doesn't always finish before 7 AM if there's a lot of data...}\hyeok{Added 'approximate'} 
Our data management framework demonstrates that the activities in study sites are passively and continuously collected with minimal privacy risks.
Furthermore, the cameras installed above visitors' eyesight made it easier for visitors to comply with the proposed instrumentation of cameras for activity monitoring. 

The on-premise fog server for the Pi network contains 2 10Gb SFP+ Ethernet interfaces, which are bonded together into a single 20G interface and connected to the switches used for the private Pi network. 
This bonded interface is used to provide enough bandwidth that the multiple Pis deployed within the study site are able to write their collected data back to the on-premise fog server for storage without creating a severe network bottleneck due to the amount of devices that were planned for deployment. 
The networking infrastructure consists of a set of 2 interconnected Supermicro SSE-G3648B switches running Cumulus Linux 3.7.12, which have been programmatically bonded together so that they will act as a single large switch while improving throughput, as one half of the 20G bond is connected to each switch.
Thus, either one can be used to pass traffic between the on-premise fog server and the data collection Pis. 
Each Pi is connected to one of the two switches via a 1Gb Ethernet connection, as the maximum speed on the Network Interface Card built into the Pis is only 1Gb. 
To prevent data breaches or leaks of sensitive data, the entire Pi network is isolated from the on-premise network. 
% \robert{We may want to say that the Pi network is physically isolated from the on-prem network rather than the cloud network, as "cloud network" implies a network that is off-site and technically every other network would be just as isolated from it; the original wording of this referenced Emory's network, while BMI's is the "cloud" network.}\hyeok{Thank you for the clarification. Corrected it!}
The only connections to the switches are by the on-premise fog server and the Pis themselves.

To facilitate the operation of all the Pis on the data collection network, the on-premise fog server provides Dynamic Host Configuration Protocol (DHCP) and Network Time Protocol (NTP) services to assign the Pis with their appropriate Internet Protocol (IP) addresses and provide them with the correct date and time when they boot up; to ensure that the same Pi receives the same address each time, the addresses are manually specified in the DHCP server’s configuration based on the Media Access Control (MAC) address of the Pi. 
The on-premise fog server also acts as a gateway to allow the Pis to reach the cloud network if needed for software update purposes, while acting as a firewall to prevent others on the cloud network from having direct access to the Pis. 
A Network File System (NFS) volume is configured on the fog server and shared with the private Pi network so that the Pis can mount a shared network volume for the purposes of operation and data storage.
Each Pi’s base image is programmed to connect to the on-premise fog server at a known static IP address and mount the NFS volume at boot up. 
% \robert{Should we also mention that the Pis launch a shared bootstrapping script which is located on this NFS volume? It's referenced in the next sentence that the Pis "load the environment and run the script", but we haven't explained what the script is yet.}\hyeok{Done. Added this detail in the next sentence}
This allows for software and functionality changes in the on-premise fog server to be deployed across all Pis on the network by simply modifying the shared configuration to reflect the desired operation.
When Pis are rebooted, they launch a shared bootstrapping script, which is located on this NFS volume, so that they will load the environment and run the script.

For storage, the on-premise server has 6 $12TB$ storage disks configured in a RAID10 configuration for $\sim32TB$ of usable space.
RAID10 was selected to provide the fastest available speeds while still allowing for disk redundancy in the event of a failure. 
The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network.
% \robert{I'm pretty sure this should read "The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network." or something along those lines.}\hyeok{Reflected.}
As the on-premise fog server is deployed in the study site, it is not directly connected via 10G Ethernet to the cloud server’s private network. 
This means the intermediate network links between the fog node and the cloud node's network are not guaranteed to all be at the maximum speed supported by either endpoint, thereby resulting in slower network speeds than a direct connection.
% \robert{Probably don't need to mention 10G and can instead reword this to be something like "the intermediate network links between the fog node and the cloud node's network are not guaranteed to all be at the maximum speed supported by either endpoint, resulting in slower network speeds than a direct connection".}\hyeok{Done. and commented the next sentence, too.}
% This makes the data traverse the general virtual private network (VPN), which at this time only runs at 1G speeds. 
% \robert{Our deployment of this is not traversing a VPN at all; it's just going over the regular Emory network and encapsulated within a SSH connection. The equivalent for a generic deployment would be the fog node's site's network and/or the Internet depending on the location of the cloud node.}
The transfer process is performed from the on-premise fog server by using Tape ARchive (TAR) 
% \robert{Not sure if we need to bold/italicize/define/something the word "tar" to indicate that it's a system command. It's short for "Tape ARchive", just in case that's helpful.}\hyeok{Good!} 
to combine all of one day’s data collection files into a single data stream, which is then transmitted over Secure Shell (SSH) to a gateway server dedicated to large data transfers on the cloud server’s main network.
The data transfer stream is then untarred and the files are placed in the designated location on the cloud server’s filesystem. 
The usage of this single stream reduces the number of individual network I/O operations that need to be performed during the transfer process (thus improving performance) when compared to other transfer options like rsync or scp operating on individual files.
It also removes the need to manually stage the tar file on the server prior to transfer as the output of tar is piped directly to the remote system and an untar process via SSH. 

\subsection{Monitoring Activities in Built-in Environment}

\input{figure/overall_method.tex}

\subsubsection{Overall Pipeline}

Here, we describe our approaches to continuously monitor the activities of multiple people in our study space with the abovementioned computing and camera infrastructure.
The overall approach for multi-view multi-person tracking is shown in \autoref{fig:overall_method}.
Based on pose detection and human bounding boxes, each person's location and body orientation are estimated and projected on a 2D coordinate system representing the study space.
Multiview integration then resolves duplicate samples across cameras from overlapping views by combining samples from 39 cameras.
Lastly, a multi-person tracking algorithm~\cite{li2010multiple} is used to track people across the frames.

\subsubsection{Preprocessing 2D poses}
\label{sec:preproc_poses}

The 2D poses estimated on Raspberry Pi are first preprocessed to remove noisy samples.
Two major artifacts were observed for the detected poses from our model~\cite{papandreou2018personlab}: non-human poses and temporal inconsistencies.
First, the model considers patterns on the walls and floor as humans due to the way the camera views them from the ceiling.
These non-human poses remain stationary over time and do not change rapidly.
Thus, we remove those false positives (non-human samples) by identifying poses in subsequent frames where pose changes are near zeros.
Second, 2D poses lack temporal consistency since the model estimates poses frame-by-frame. 
It was observed that a number of poses had their left and right sides flipped or missing between frames (false negatives).
We used Kalman filter-based temporal smoothing to denoise and fill missing detections~\cite{10.1115/1.3662552}.
For Kalman filter, linear constant model was used for modeling temporal changes in keypoint locations of COCO pose, which has 17 joint keypoints~\cite{lin2014microsoft}, $X_t=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}, \dot{u}_1 \dot{v}_1, \dot{u}_2 \dot{v}_2, \cdots, \dot{u}_{17} \dot{v}_{17}]$, where $u$ and $v$ are $x$ and $y$ location of each keypoint and $\dot{u}$ and $\dot{v}$ are the velocity of location changes.

Kalman smoothing for 2D poses is achieved by using Kalman filter-based multi-person tracking technique that has been widely adopted in the past~\cite{bewley2016simple}.
As shown in \autoref{fig:kalman_tracker} (a), the tracker follows predict, detect, match, update, and repeat operations.
Given multi-person tracking until time $t-1$, Kalman filter trackers make predictions of each person's location at time $t$. 
To update the prediction based on actual detections at time $t$, the Hungarian method is used to find matches between predictions and detections from 2D poses~\cite{kuhn1955hungarian} (\autoref{fig:kalman_tracker}, b).
Hungarian methods are widely used to find matches between two groups of samples because of their efficiency and effectiveness~\cite{perera2006multi,bewley2016simple,xu2020train}.
For Hungarian matching, we generate a bipartite graph where each node is 2D pose from prediction and detection at time $t$ and the edge is $L_2$-norm distance between those 2D poses.
The bipartite graph is represented as a matrix, where $C_{i,j}= \|P^i_{p} - P^j_{d} \|_2$ is $L_2$-norm distance between $i$th pose from predictions, $P_p$,  and $j$th pose from detections, $P_d$. 
% and $P=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}]$.
The Hungarian method then finds the matchings (or edges) with the smallest sum of distances between the samples from predictions and detections (\autoref{fig:kalman_tracker} (b), \textcolor{red}{red} lines).
Specifically, Hungarian method optimizes:

\begin{equation}
    Y = \arg\min_{Y} \sum_i \sum_j C_{i,j} Y_{i,j}
\end{equation}

% \chaitra{I think we should explain what this equation is before introducing it. There is a discontinuity between the previous sentence and this one}\hyeok{Done.}
\noindent where $Y$ is a boolean matrix, showing assignment within $C$.
Next, The predictions get updated with the matched detections.
For the unmatched detections, a new tracker initiates (\autoref{fig:kalman_tracker} (a), \textcolor{red}{red}).
In the case of false negatives (no detections in time $t$), we skip the update operation and continue with the prediction, which is kept alive for 10 seconds to handle potential false negatives.
Until the tracking is complete, this process is repeated.
Lastly, we apply kalman smoothing with Rauch-tung-Striebel (RTS) smoother to optimize the temporal consistency of estimated 2D pose movements based on all trackers over time~\cite{chan2011implementation}.
Using these processed 2D poses, we can now localize people for the corresponding locations in the study site and track them based on multiple viewpoints.

\subsubsection{Indoor Localization}

\input{figure/tracker}

An indoor localization technique aims to locate people within the study site in 2D coordinate space based on the 2D poses detected from each camera.
As a rule of thumb, the middle of the left and right feet is defined as the location of people in a scene.
As the floor in our study space is flat, any detected people in a scene are on the same plane.
With this in mind, we learn a perspective transformation matrix, $M\in \mathbb{R}^{3\times3}$, that can project the foot location from the floor in 2D camera space to the corresponding floor location in the 2D coordinate of the study site~\cite{sun2019see,cosma2019camloc}.

\begin{equation}
    \begin{bmatrix}
        x \\ y \\ 1
    \end{bmatrix}
    = \begin{bmatrix}
        m_{11} & m_{12} & m_{13} \\
        m_{21} & m_{22} & m_{23} \\
        m_{31} & m_{32} & m_{33}
    \end{bmatrix}
    \begin{bmatrix}
        u \\ v \\ 1
    \end{bmatrix}  
    \label{eqn:perspective_mat}
\end{equation}

\noindent where $[x, y]$ is the foot location in study site coordinate and $[u, v]$ is the foot pixel location in the camera.
From every 39 cameras, we learn $M$ by manually selecting 4 corresponding points in the 2D coordinate study site and the pixel locations in the field of view of a camera~\cite{abdel2015direct,shim2015mobile}.
Once $M$ is derived, they are used to localize the feet locations of detected 2D poses in the study space coordinate. 
% unless the camera location or orientation is changed.

\subsubsection{Body Orientation Estimation}

The facing orientation of people in a group activity gives important insights into their relationship and engagement with each other~\cite{cristani2011social,barua2021detecting}.
From the human bounding box detected by 2D pose detection models, we extract the facing direction of each person in the transverse plane, whose orientation is then transformed into the study site coordinates.
For estimating chest facing direction in a human bounding box image, we adopt the deep learning-based body orientation estimation method~\cite{wu2020mebow}. 
Wu~\etal~\cite{wu2020mebow} proposed a deep learning model that combines HRNet~\cite{sun2019deep} and ResNet~\cite{he2016deep} to predict chest facing orientation in 5\degree-intervals from human bounding box images.
The model was trained to learn from multiple tasks, including 2D pose, 3D pose, and body orientation prediction.
This enabled the model to learn the representation that considers 2D and 3D pose geometry and depth information for robustly estimating body orientation from 2D human bounding box images.
Here, we define a human bounding box as a tight square region that contains a detected 2D pose from Raspberry Pi.
The estimated chest orientation is represented as a 2D chest vector on a transverse plane.
Then, the 2D chest vector in camera space is transformed to the 2D orientation in study site coordinate, $\Vec{v}^t_{world} = R_{camera \rightarrow world}\Vec{v}^t_{world}$.
The rotation matrices, $R_{camera \rightarrow world}$, for each camera is manually defined according to the camera installation in the study site, where north is set as a reference orientation.

\subsubsection{Multi-view Integration}

\input{figure/multi-view_integration.tex}

The 39 cameras installed in the study site 
% \robert{Should "sites" be plural or singular? We're only talking about the one deployment, correct?}\hyeok{Yes. Correct. Haha I am keep making this typo for singular/plural.}
have partially overlapping field-of-views to continuously track people across the wide space.
Multiple cameras capture duplicate samples of the same person due to these overlaps.
In order to remove duplicated samples, we detect people across cameras and integrate the detections into a single sample that potentially represents the true location of the person, as shown in \autoref{fig:muti-view_integration}.
To detect those duplicated samples, we generate a graph, $G=(V,E)$, where vertices, $V=\{v_{ci}=(x,y)|c=1,\cdots,39, i=1,\cdots\}$, are locations of all samples from all 39 cameras and edge, $E=\{v_{ci}v_{c'j} |\; c \neq c' \}$, is the connectivity between samples from different cameras that are sufficiently close in the distance.
We assume that duplicates are coming from the same person captured in different cameras, if their euclidean distance is within $\| v_{ci} - v_{c'j} \|_2 \leq 1.5 m$, considering the error margin of our localization technique.
It is possible for the same person located from a different camera to be in a slightly different location from our indoor localization due to lens distortions violating planar assumptions about the floor that can incur inaccuracies in perspective transformations.
% that is used for perspective transformation in our indoor localization technique.
Regardless, we empirically found that only 1.5 meters were sufficient for the margin of the localization error~\cite{zhang2000flexible}.

Once the graph $G$ is constructed, the duplicated samples are identified as those with linked vertices in a graph, which is also called connected components, $CC$, from graph theory~\cite{john1995first}.
Then, we integrate the locations of the duplicated samples considering the camera distance from the detected sample. 
Specifically, when integrating duplicated samples, the samples are penalized when the camera distance is far:

\begin{equation}
    L = \sum_{CC} \frac{1}{d_{ci}} v_{ci}
\end{equation}

\noindent where $L$ is the location of integrated sample and $d_{ci} = \| l_c - v_{ci} \|^2_2$ is the euclidean distance between the sample, $v_{ci}$, and the camera, $l_c$.
According to our findings, the localization error and the distance between the camera and the target person are strongly correlated.
Similarly, the orientation of the duplicated samples is integrated for the vertices in $CC$ considering camera distances.
The multi-view integration results in unique locations, $L=[l_x, l_y]$, and orientation vectors, $o=[o_x, o_y]$, of each person at each time step.  

\subsubsection{Multi-person Tracking}

To understand detailed individual or group activities occurring in the study site, the locations of people needs to be tracked across time.
For multi-person tracking, we also apply Kalman filter-based tracking for the locations, $L=[l_x, l_y]$, and orientation vector, $O=[o_x, o_y]$, from multi-view integration~\cite{kuhn1955hungarian}.
The tracker follows predict, detect, match, update, and repeat steps used in Sec.~\ref{sec:preproc_poses}, but with some differences.
We again use a linear constant model for both location and orientation, where states are represented as location, $L=[l_x, l_y]$, orientation, $O=[o_x, o_y]$, velocity, $\dot{L}=[\dot{l}_x, \dot{l}_y]$, and angular velocity, $\dot{O}=[\dot{o}_x, \dot{o}_y]$.
Furthermore, we assume that people's facing orientation follows their walking direction closely.
Therefore, the tracker estimates facing orientation at time $t$ by summing up both moving directions, the velocity when 1 Hz, $\dot{L}$, and angular velocity, $\dot{O}$.

\begin{equation}
    O_t= O_{t-1} + w\cdot \dot{L}_{t-1} + dt\cdot \dot{O}_{t-1}
\end{equation}

\noindent where $w=0.1$ is a weighting of moving direction (or velocity) on current orientation and $dt$ is the time interval between frames, which is 1 sec.
When associating predictions and matching using Hungarian matching, the bipartite graph is represented as a matrix, where $C_{i,j}= \|L^i_{p} - L^j_{d} \|_2$ is euclidean distance between $i$th sample from prediction, $L_p$, and $j$th sample from detection, $L_d$.
Likewise earlier, we applied RTS smoothing for finished trackers to consider temporal dynamics across the entire trajectory of a person.

\subsection{Evaluating Multi-person Tracking and Localization}

We evaluate our multi-view multi-person tracking systems with respect to localization, tracking, and body orientation estimation performances following the standard evaluation methods~\cite{bernardin2006multiple,wu2020mebow}.
As there is no single metric for evaluating multi-person tracking methods, we utilize the following metrics to understand the performance of the proposed system~\cite{dendorfer2020mot20}.
$\uparrow$ and $\downarrow$ are shown for the metrics that are higher or lower the better, respectively.

\begin{itemize}
    \item MOTA $\uparrow$ (Multi-Object Tracking Accuracy) combines three kinds of error sources, which are false positives, missed targets, and identity switches.    
    \item IDF1 $\uparrow$ (ID F1 score) is the ratio of correctly identified detections over the average number of ground-truth and computed detections.
    \item MT $\uparrow$ (Mostly Tracked targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at least 80\% of their respective life span.
    \item ML $\downarrow$ (Mostly Lost targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at most 20\% of their respective life span.
    \item FPR $\downarrow$ (False Positives Rate) measures the average number of false alarms per frame.
    \item FNR $\downarrow$ (False Negatives Rate) measures the average number of missed targets per frame.
    \item Rcll $\uparrow$ (Recall) measures the ratio of correct detections to the total number of ground-truth locations.
    \item Prcn $\uparrow$ (Precision) measures the number of detected objects over the sum of detected and false positives.
    \item IDSR $\downarrow$ (ID Switch Ratio) measures the number of ID switches (IDS) over recall.
    \item Frag $\downarrow$  (Fragmentation) measures the total number of times a trajectory is fragmented, which are interruptions during tracking.
\end{itemize}

Specifically, $MOTA=1-\frac{\sum_t FN_t + FP_t + IDS_t}{\sum_t GT_t}$,
% \yash{This definition suggests that MOTA could potentially produce negative values, but earlier you mentioned that this metric is typically bounded between 0 and 1 unless we are forcing/constraining the algorithm to find/detect fixed number of objects/persons}\hyeok{As I clarified in the meeting. Yes. MOTA can go to negative but this means something is very wrong in the prediction.} 
where $FN_t$, $FP_t$, $IDS_t$, and $GT_t$ are false negatives (misses), false positives, ID switches, and ground-truths at time $t$.
One important evaluation that preceded tracking is detection. 
In this work, we define a ground-truth target at the time $t$ is detected if the estimated sample location is within 1.5 meters in euclidean distance.
Otherwise, the target is considered as \textit{missed}. 
The 1.5-meter reference is based on the fact that people rarely walk faster than 1.42 m/s on an everyday basis~\cite{browning2006effects,mohler2007visual,levine1999pace}.

To demonstrate the localization accuracy of the estimated samples, we also report multiple object tracking precision, $MOTP=\frac{\sum_{i,t} d^i_t}{\sum_t c_t}$.
$d^i_t$ is the euclidean distance between the $i$th detected ground-truth sample and estimated sample, and $c_t$ is the number of detection at time $t$. 
In other words, MOTP is the average euclidean distance error for the detected samples, which shows the performance of the proposed systems to estimate the precise location of target samples that is independent of tracking trajectories or ID switches.
% We will also evaluate the proposed kalman filter-based tracking model with Hungarian matching-based tracking approach, which only considers detections in subsequent frames ignoring temporal consistency over the time.. 
% Majority of multi-view multi-person tracking methods are based on RGB color or depth images, which is not available in our dataset~\cite{gan2021self,haque2017towards,guo2022review}.
% Also, previous multi-view multi-person tracking methods are based on 2D image planes, and the global coordinate was projected directly using the known relationship between camera intrinsic and extrinsic parameters~\cite{tang2017multiple,liem2014joint}.
% The proposed approach differs as only 2D poses are available to preserve the privacy of the visitors and staff in our study site.

\subsubsection{Multi-person Tracking Baseline}
% \yash{did we find baseline for multi-view position estimation by simply averaging the estimated location by each camera?}\hyeok{I have it in one of my experiments. But, didn't include in the paper due to page length and due to the lesser importance compared to the baselines in the paper.}
Our proposed tracker is compared with a Hungarian matching-based tracker~\cite{kuhn1955hungarian}, which only considers frame-by-frame matching between 2D pose detections, in order to illustrate the importance of modeling temporal dynamics of 2D movements.
Based on the results of multiview multi-person localization at time $t$ and $t+1$, the Hungarian tracker generates a bipartite graph with nodes representing samples from two consecutive timesteps and edges representing Euclidean distances between samples. 
Since our tracking rate is 1 Hz, we remove any edge distance larger than 1.5 meters in the created bipartite graph, as people normally walk 1.42 m/s in everyday activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
Then, the Hungarian method finds the matchings (or edges) that have a minimum sum of Euclidean distances.
Potentially missing samples (false negatives) in a frame $t$ are filled in by linearly interpolating the matched detection from frame $t-1$ and $t+1$.
The Hungarian matching is applied until no matching is found any longer along the time.

\subsection{Evaluating Body Orientation Estimation}

Our benchmark dataset and the proposed method represent the body orientation as a continuous angle.
Following the standard definition of body orientation in the previous work~\cite{wu2020mebow,yu2019continuous,andriluka2010monocular}, we defined the human orientation $\theta \in [0\degree, 360\degree)$ as the chest facing direction on the transverse plane that is projected to the 2D coordinate in the study site, where the north (top) direction is the reference with clock-wise rotation.
Following previous work, we use two metrics: Mean Absolute Error (MAE) of angular distance and Accuracy-$X\degree$~\cite{wu2020mebow}.
Accuracy-$X\degree$ is defined as the ratio of the samples that are predicted within the deviation of $X\degree$ according to the ground-truth orientation. 
By using $X\in [0\degree, 180\degree]$, Accuracy-$X\degree$ measures fine-grained model accuracy.
% compared to the discrete orientation classification methods based on either equally spaced four (N, E, S, W) or eight (N, NE, E, SE, S, SW, W, NW) orientations~\cite{yu2019continuous}.
% We will compare the proposed body orientation estimation method with a number of baseline methods that is based on 1) 2D pose only or 2) 3D human pose and projection geometry~\cite{takahashi2018human}.
% For discrete evaluation, the continuous values in ground truth and estimated orientations are mapped to the closed four or eight direction and the estimated orientation is considered correct if the value is mapped to the correct directional bin.
% Following the previous work, we will use $X=\{5, 15, 22.5, 30, 45\}$.

\subsubsection{Comparing Body Orientation Estimation Baselines}

Our body orientation method inherently learns the geometric relationship between 2D pose, 3D pose, and the corresponding body orientation of the observed human bounding box.
We compare the proposed method with two baselines that only use 2D information and then a baseline that only models the 3D geometry of detected 2D poses.
Through this practice, we will demonstrate the importance of modeling both 3D geometry and pose-body orientation relationships.

\noindent i) \textit{2D pose-based Heuristic Approach:}
This method uses a heuristic approach to estimate body orientation from only 2D pose information.
Specifically, it uses 2D facial keypoints, including nose, eyes, and ears, and estimates the 2D vector originating from the average of left and right eyes and ears keypoints to nose keypoints on 2D image pixels.
We directly project those 2D vectors from the image frame to the 2D coordinate space of the study site using a perspective transformation matrix, $M$, derived from \autoref{eqn:perspective_mat}.

\noindent ii) \textit{2D pose-based Deep Learning Approach:}
This baseline model applied a learning-based method, where the model directly estimates body orientation from 2D pose input.
We used a graphical convolutional network (GCN)~\cite{yan2018spatial} to process 2D pose data to predict body orientation angle in 5-\degree intervals.
For training the model, we used MS COCO 2D keypoints~\cite{lin2014microsoft} dataset and the corresponding body orientation annotation provided by  Wu~\etal~\cite{wu2020mebow}.
We augmented 2D keypoints input by randomly flipping horizontally or adding Gaussian noises to simulate noisy pose detections from our pipeline.

\noindent iii) \textit{ 2D-3D pose Geometric matching-based Approach:}
To model the 3D geometry of the human body pose~\cite{takahashi2018human}, we first estimated 3D pose information from the detected 2D poses from our pipeline.
We lift the estimated 2D poses to 3D poses by using the 3D pose estimation method~\cite{pavllo20193d}.
Then, the 3D poses are calibrated according to the camera viewpoint using Perspective-n-point projection technique~\cite{lepetit2009epnp}.
Specifically, at each time step $t$, we learn the extrinsic parameters, which are rotation and translation matrices, of the estimated 3D chest keypoints (left and right shoulders and left and right pelvis) for projecting 3D pose to the corresponding 2D keypoints in the image space. 

\begin{equation}
    [R|T]^t = \arg\min_{R,T}\| p^t_2 - sK[R|T]p^t_3 \|
\end{equation}

\noindent where $R\in\mathbb{R}^{3\times 3}$ is a rotation matrix subject to $R^TR=I\in\mathbb{R}^{3\times3}$ and $det(R) = 1$ and $T\in\mathbb{R}^{3\times 1}$ is a translation matrix that minimizes the projection error of chest keypoints of 3D pose, $p^t_3$, to 2D pose, $p^t_2$, at timestep $t$ given intrinsic camera lense parameter, $K\in\mathbb{R}^{3\times 3}$.
We fix the camera intrinsic matrix, $K$, with the parameters provided by the manufacturer~\cite{rpi_camera} and the scale parameter is arbitrarily set as $s=1$ as we do not require the absolute scale of the 3d pose size, but only the facing direction.
For each person, we smoothed $[R|T]^t$ over all time steps using moving SLERP filter~\cite{shoemake1985animating} and moving average filter for rotation and translation matrices, respectively, to keep the temporal consistency.
From the 3D pose calibrated according to the chest orientation, we acquire the 3D chest norm vector perpendicular to the left-to-right shoulder vector and left shoulder-to-left pelvis vector, $\Vec{v}^t_{chest} = \Vec{v}^t_{L.Shoulder \rightarrow R.Shoulder} \times \Vec{v}^t_{L.Shoulder \rightarrow L.Pelvis}$, at each timestep $t$.
The estimated 3D chest norm vector is projected to a 2D chest vector on a transverse plane, which represents the facing of each people in the scene with respect to the camera viewpoint.

\subsection{Impact of Camera Installation on Model Behavior}

\input{figure/cam_install_protocol}

In our study site, the camera installation is determined primarily by the power and network source reachable using extension cables, resulting in 39 cameras unequally installed in the space. %\yash{"uniformly installed throughout the space"}\hyeok{No. it is not true.}
In our experiment, we will examine this in more detail to understand the impact of camera installation on four different factors, shown in \autoref{fig:cam_install_protocol}, related to localization and body orientation estimation accuracy.

\subsubsection{Distance Between Camera and Person}

Across all cameras, we measured the distance between captured people from the camera center, as shown in \autoref{fig:cam_install_protocol} (a), that will be associated with localization and orientation errors.

\subsubsection{Facing Angle Away from Camera Viewpoint}

We collected the degree of facing directions of the captured person deviating from camera viewpoints, as shown n \autoref{fig:cam_install_protocol} (b), and conducted correlation analysis with the corresponding localization and orientation errors.

\subsubsection{Horizontal Displacement from Camera Center}

We studied the impact of the horizontal displacement of the captured person from the camera center (\autoref{fig:cam_install_protocol}, c).
We quantified the horizontal displacement as the horizontal angle, $\theta\degree_H$, of the person from the camera center that is normalized by horizontal field-of-view, $\theta\degree_{H_{FOV}}$, which is normalized horizontal angle, $\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$.
As a person gets closer to the horizontal center of the camera, the normalized horizontal angle approaches zero.
The normalized horizontal angle increases to $1$ when the person is at the edge of the frame. 
When the value is larger than $1$, then only part of the body is observable from the camera.
We examine how localization and orientation errors vary with the degree of horizontal displacement.

\subsubsection{Vertical Displacement from Camera Center}

Following horizontal displacement, we studied the effect of vertical displacement of a person from the camera center (\autoref{fig:cam_install_protocol}, d).
The vertical displacement was quantified as a vertical angle, $\theta\degree_V$, of the person captured from the camera center that is normalized by vertical field-of-view, $\theta\degree_{V_{FOV}}$, referring to the camera datasheet, namely normalized vertical angle, $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$.
We specifically consider the foot location, which we use to localize, as a point of reference to calculate the normalized vertical angle.
When the person is closer to the camera, the normalized vertical angle increases, and only the upper body is partially captured by the camera due to the limited vertical field of view.
On the other hand, as the person moves away from the camera, the normalized vertical angle decreases and can capture the full body in the field of view, but with the cost of increased distance between the camera and the person.
Likewise, in the above-mentioned analysis, we will study the changes in localization and orientation errors based on the vertical displacement of the captured person.


==> sections/method/main.tex <==
\section{Method \& Materials}

\input{figure/ep6_func_spaces.tex}

% In this work, multiple edge computing-based camera systems are integrated into a distributed network and are installed with edge, fog, and cloud computing environments to locate and track multiple people with their body orientations in a built environment.
% This section provides a detailed account of our study site, the computing environment of our system, the techniques employed to continuously monitor people's movements in a given space, and an evaluation of the systems.

\subsection{Study Site}

\revision{
The study site used is a 1700$m^2$ indoor environment consisting of various functioning spaces.
}
Referring \autoref{fig:ep6_func} and \autoref{fig:data_collection}, Activity Area (A) includes both the Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and left boundary of conversation room.
The left corridor (C) is the narrow corridor next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor where the Lockers are left to the Innovation Theater. The lounge (D) includes the area between the elevator and the front door, and the Staff area (F) includes the region on the right side of the building where staff offices are located.

% This study site is specifically designed to help individuals with MCI to lead better lives. It is a one-of-a-kind project designed based on a series of goals: promoting social interaction, environmental exploration, spatial flexibility, safety, independent learning of everyday tasks (e.g., cooking), contact with nature, exercise, and cognitive stimulation in individuals diagnosed with MCI. The study spaces is adjustable and equipped with technologies like tunable lighting and controllable zone-based sound systems to experiment with achieving these goals. Designing healthcare facilities for individuals living with MCI poses challenges for architects as it requires unique design considerations that differ from those required for cognitively healthy older adults and dementia patients~\cite{challenge_arch_2020}. 
% While people with MCI also experience cognitive decline, their condition is less debilitating than that of dementia patients~\cite{Gauthier2006_classic}.

\subsection{Distributed Camera Network using Edge Computing}

\input{figure/camera_config}

% Edge computing-based camera devices are installed in the ceiling of the study site and integrated with a server infrastructure. This system is described in this section. 

\subsubsection{Camera Configuration}

\revision{
\autoref{fig:camera_config}a shows the locations (\textcolor{blue}{BLUE}) of 39 low-cost ($<\$500$) edge computing and camera devices (\autoref{fig:camera_config}b) and their viewpoints (\textcolor{red}{RED}).
Sparsely distributed cameras could cover the entire study site where subjects agreed to monitor their activities.
\autoref{fig:camera_config}c shows the example of camera installation and edge computing devices connected to the closest power and network sources available in the ceiling through USB-C power cable and ethernet cable for data transfer. 
The cameras installed above visitors' eyesight make it easier for visitors to comply with the proposed instrumentation of cameras for activity monitoring. 
Depending on the accessible power and network sources, some locations, such as kitchen or staff areas, are covered by multiple cameras, and other locations, such as long corridors, are covered by single or two cameras. 
}

%------

% We installed 39 low-cost ($<\$500$) edge computing and camera devices in the study site as shown in \autoref{fig:camera_config}. The camera devices consist of a camera sensor (Sony IMX219 8-megapixel sensor) and a Google Coral TPU USB Accelerator attached to an edge computing system. The Google Coral TPU USB Accelerator enables deep learning models to run in real-time on the edge computing system. 

% Each edge computing system and camera device runs a multi-person 2D pose estimation model~\cite{papandreou2018personlab} in real-time (\autoref{fig:camera_config}, b). Poses are estimated at a frame rate of 1Hz. The poses obtained from this pose estimation model, as well as human bounding box images, are stored for further downstream processing. The raw video frames are discarded. Thus, personally identifiable data is not stored or used for downstream computation, which preserves the privacy of individuals in the study site.  

% The edge computing and camera devices are placed and hidden in the ceiling panel and connected to power and network sources using extension cables in the existing infrastructure (\autoref{fig:camera_config}, c).
% Depending on the accessible power and network sources, some locations, such as kitchen or staff areas, are covered by multiple cameras, and other locations, such as long corridors, are covered by single or two cameras. 
% Yet, the placement location (\autoref{fig:camera_config}, (a), \textcolor{blue}{BLUE}) and viewpoints (\autoref{fig:camera_config}, (a), \textcolor{red}{RED}) of 39 camera devices could still cover entire study site where subject agreed to monitor their activities.
% are shown in \autoref{fig:camera_config} (a), where the gradient from white to blue depicts the direction of viewpoits of the camera devices. \hyeok{Update with the new figure.}

% In total, 39 camera sensors (Sony IMX219 8-megapixel sensor; \textcolor{blue}{BLUE}) are installed with the field of views (\textcolor{red}{RED}) covering the entire indoor space

\input{figure/compute_config}

\input{figure/overall_method.tex}

\subsubsection{Secure Computing Network Architecture}

The overall computing configuration consists of 4 primary segments: the cloud server, the on-premise fog server, the private edge computing networking infrastructure, and the 39 edge computing camera devices. This configuration is shown in \autoref{fig:compute_config}.

\revision{
The 2D poses, which consist of 17 keypoints based on the MS COCO format~\cite{lin2014microsoft}, and bounding boxes are estimated at a frame rate of 1Hz in real-time using TPU, which data are stored on a Health Insurance Portability and Accountability Act (HIPAA)-compliant and secure data storage server at the study site.
To preserve privacy, the raw video frames are discarded after processing.
This was to prevent capturing, storing, and transmitting any sensitive or identifiable information over the network, such as face or nudity.
The bounding box images are temporarily stored for one hour on the fog computing node for estimating body orientations and are not transferred to the cloud computing nodes.
To prevent data breaches or leaks of sensitive data, the entire edge computing network is isolated from the on-premise network.
The 2D poses and the processed body orientation estimation results are stored for permanent data management and analysis.
The fog computing node store one day's worth of data between 8 AM and 7 PM and perform data analysis.
The collected data and the performed analysis results are synced nightly approximately between 12 PM and 7 AM to a cloud node's privacy-preserving data server for permanent storage. The duration for nightly sync can change depending on the data size collected over the day.
Our data management framework passively and continuously collects the activities in the study site with minimal privacy risks. 
}

% In addition to body orientation estimation, additional activity analysis is carried out by fog computing node, which includes multi-person localization and tracking of the day's data.
% The on-premise fog server for the edge computing network contains 2 10Gb SFP+ Ethernet interfaces, which are bonded together into a single 20G interface and connected to the switches used for the private edge computing network. 
% This bonded interface is used to provide enough bandwidth that the multiple edge computing systems deployed within the study site are able to write the collected data back to the on-premise fog server for storage without creating a severe network bottleneck. 

% The networking infrastructure consists of a set of 2 interconnected Supermicro SSE-G3648B switches running Cumulus Linux 3.7.12, which have been programmatically bonded together so that they will act as a single large switch while improving throughput, as one half of the 20G bond is connected to each switch.
% Thus, either one can be used to pass traffic between the on-premise fog server and the edge computing systems. 
% Each edge computing system is connected to one of the two switches via a 1Gb Ethernet connection, as the maximum speed on the Network Interface Card built into the edge computing systems is only 1Gb. 
% To prevent data breaches or leaks of sensitive data, the entire edge computing network is isolated from the on-premise network. The only connections to the switches are by the on-premise fog server and the edge computing systems themselves.

% To facilitate the operation of all the edge computing systems on the data collection network, the on-premise fog server provides Dynamic Host Configuration Protocol (DHCP) and Network Time Protocol (NTP) services to assign the edge computing systems with their appropriate Internet Protocol (IP) addresses and provide them with the correct date and time when they boot up; to ensure that the same edge computing system receives the same address each time, the addresses are manually specified in the DHCP server’s configuration based on the Media Access Control (MAC) address of the edge computing system. 
% The on-premise fog server also acts as a gateway to allow the edge computing systems to reach the cloud network if needed for software update purposes, while acting as a firewall to prevent others on the cloud network from having direct access to the edge computing systems. 
% A Network File System (NFS) volume is configured on the fog server and shared with the private edge computing network so that the edge computing systems can mount a shared network volume for the purposes of operation and data storage.
% Each edge computing system’s base image is programmed to connect to the on-premise fog server at a known static IP address and mount the NFS volume at boot-up. 
% This allows for software and functionality changes in the on-premise fog server to be deployed across all edge computing systems on the network by simply modifying the shared configuration to reflect the desired operation.
% When edge computing systems are rebooted, they launch a shared bootstrapping script, which is located on this NFS volume, so that they will load the environment and run the script.

% For storage, the on-premise server has 6 $12TB$ storage disks configured in a RAID10 configuration for $\sim32TB$ of usable space.
% RAID10 was selected to provide the fastest available speeds while still allowing for disk redundancy in the event of a failure. 
% The largest hurdle in this process is the transfer of the collected data from the on-premise fog node to the cloud node's network.
% As the on-premise fog server is deployed in the study site, it is not directly connected via 10G Ethernet to the cloud server’s private network. 
% This means the intermediate network links between the fog node and the cloud node's network are not guaranteed to all be at the maximum speed supported by either endpoint, thereby resulting in slower network speeds than a direct connection.
% The transfer process is performed from the on-premise fog server by using Tape ARchive (TAR) to combine all of one day’s data collection files into a single data stream, which is then transmitted over Secure Shell (SSH) to a gateway server dedicated to large data transfers on the cloud server’s main network.
% The data transfer stream is then untarred and the files are placed in the designated location on the cloud server’s filesystem. 
% The usage of this single stream reduces the number of individual network I/O operations that need to be performed during the transfer process (thus improving performance) when compared to other transfer options like rsync or scp operating on individual files.
% It also removes the need to manually stage the tar file on the server prior to transfer as the output of tar is piped directly to the remote system and an untar process via SSH. 


\subsection{Monitoring Movement in Built-in Environment}

\subsubsection{Overall Pipeline}

Here, we describe our approaches to continuously localize and track multiple people in the study space with the abovementioned computing and camera infrastructure.
The overall approach for multi-view multi-person tracking is shown in \autoref{fig:overall_method}.
Based on pose detection and human bounding boxes, each person's location and body orientation is estimated and projected on a 2D coordinate system representing the study space.
Multiview integration then resolves duplicate detections across cameras from overlapping views by combining samples from 39 cameras.
Lastly, a multi-person tracking algorithm~\cite{li2010multiple} is used to track people across the frames.

\subsubsection{Preprocessing 2D poses}
\label{sec:preproc_poses}

% \input{figure/tracker}

The 2D poses estimated on the edge computing systems are first preprocessed to remove noisy samples.
Two major artifacts were observed for the detected poses from the pose detection model~\cite{papandreou2018personlab}: non-human poses and temporal inconsistencies.
First, the model considers patterns on the walls and floor as humans due to the way the camera views the area from the ceiling.
These non-human poses remain stationary over time and do not change rapidly.
Thus, we remove those false positives (non-human samples) by identifying poses in subsequent frames where pose changes are near zeros.
Second, 2D poses lack temporal consistency since the model estimates poses frame-by-frame. 
It was observed that a number of poses had their left and right sides flipped or missing %\chaitra{Do you mean the pose was missing altogether?}\hyeok{yes.}
between frames (false negatives).
We used Kalman filter-based temporal smoothing to denoise and fill missing detections~\cite{10.1115/1.3662552,chan2011implementation}.
Using these processed 2D poses, we can now localize people for the corresponding locations in the study site and track them based on multiple viewpoints.

% For the Kalman filter, linear constant model was used for modeling temporal changes in keypoint locations of COCO poses, which have 17 keypoints~\cite{lin2014microsoft}, $X_t=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}, \dot{u}_1 \dot{v}_1, \dot{u}_2 \dot{v}_2, \cdots, \dot{u}_{17} \dot{v}_{17}]$, where $u$ and $v$ are $x$ and $y$ location of each keypoint and $\dot{u}$ and $\dot{v}$ are the velocity of location changes.

% Kalman smoothing for 2D poses is achieved by using Kalman filter-based multi-person tracking technique that has been widely adopted in the past~\cite{bewley2016simple}.
% As shown in \autoref{fig:kalman_tracker} (a), the tracker follows predict, detect, match, update, and repeat operations.
% Given multi-person tracking until time $t-1$, Kalman filter trackers make predictions of each person's location at time $t$. 
% To update the prediction based on actual detections at time $t$, the Hungarian method is used to find matches between predictions and detections from 2D poses~\cite{kuhn1955hungarian} (\autoref{fig:kalman_tracker}, b).
% Hungarian methods are widely used to find matches between two groups of samples because of their efficiency and effectiveness~\cite{perera2006multi,bewley2016simple,xu2020train}.
% For Hungarian matching, we generate a bipartite graph where each node is 2D pose from prediction and detection at time $t$ and the edge is $L_2$-norm distance between those 2D poses.
% The bipartite graph is represented as a matrix, where $C_{i,j}= \|P^i_{p} - P^j_{d} \|_2$ is $L_2$-norm distance between $i$th pose from predictions, $P_p$,  and $j$th pose from detections, $P_d$. 
% % and $P=[u_1 v_1, u_2 v_2, \cdots, u_{17} v_{17}]$.
% The Hungarian method then finds the matchings (or edges) with the smallest sum of distances between the samples from predictions and detections (\autoref{fig:kalman_tracker} (b), \textcolor{red}{red} lines).
% Specifically, Hungarian method optimizes:

% \begin{equation}
%     Y = \arg\min_{Y} \sum_i \sum_j C_{i,j} Y_{i,j}
% \end{equation}

% \noindent where $Y$ is a boolean matrix, showing assignment within $C$.
% Next, The predictions get updated with the matched detections.
% For the unmatched detections, a new tracker is initiated (\autoref{fig:kalman_tracker} (a), \textcolor{red}{red}).
% In the case of false negatives (no detections in time $t$), we skip the update operation and continue with the prediction, which is kept alive for 10 seconds to handle potential false negatives.
% Until the tracking is complete, this process is repeated.
% Lastly, we apply kalman smoothing with Rauch-Tung-Striebel (RTS) smoother to optimize the temporal consistency of estimated 2D pose movements based on all trackers over time~\cite{chan2011implementation}.

\subsubsection{Indoor Localization}
\label{sec:indoor_localization}

Our indoor localization technique aims to locate people within the study site in 2D coordinate space based on the 2D poses detected from each camera.
The middle of the left and right feet is defined as the location of people in a scene.
As the floor in our study space is flat, any detected people in a scene are on the same plane.
With this in mind, we learn a perspective transformation matrix, $M\in \mathbb{R}^{3\times3}$, that can project the foot location from the floor in 2D camera space to the corresponding floor location in the 2D coordinate of the study site~\cite{sun2019see,cosma2019camloc}.

% \begin{equation}
%     \begin{bmatrix}
%         x \\ y \\ 1
%     \end{bmatrix}
%     = \begin{bmatrix}
%         m_{11} & m_{12} & m_{13} \\
%         m_{21} & m_{22} & m_{23} \\
%         m_{31} & m_{32} & m_{33}
%     \end{bmatrix}
%     \begin{bmatrix}
%         u \\ v \\ 1
%     \end{bmatrix}  
%     \label{eqn:perspective_mat}
% \end{equation}

% \noindent where $[x, y]$ is the foot location in study site coordinate and $[u, v]$ is the foot pixel location in the camera.
% From every 39 cameras, we learn $M$ by manually selecting 4 corresponding points in the 2D coordinate study site and the pixel locations in the field of view of a camera~\cite{abdel2015direct,shim2015mobile}.
% The derived $M$s for each camera are deployed to localize the feet locations of detected 2D poses in the study space coordinate. 
% unless the camera location or orientation is changed.

\subsubsection{Body Orientation Estimation}
\label{sec:body_ori_est}

\input{figure/multi-view_integration.tex}

% The facing orientation of people in a group activity gives important insights into their relationship and engagement with each other~\cite{cristani2011social,barua2021detecting}.
From the human bounding box from 2D pose detection models, we extract the facing direction of each person in the transverse plane, whose orientation is then transformed into the study site coordinates.
For estimating chest facing direction in a human bounding box image, we adopt the deep learning-based body orientation estimation method~\cite{wu2020mebow}. 
% Wu~\etal~\cite{wu2020mebow} proposed a deep learning model that combines HRNet~\cite{sun2019deep} and ResNet~\cite{he2016deep} to predict chest facing orientation in 5\degree-intervals from human bounding box images.
% The model was trained to learn from multiple tasks, including 2D pose, 3D pose, and body orientation prediction.
% This enabled the model to learn the representation that considers 2D and 3D pose geometry and depth information for robustly estimating body orientation from 2D human bounding box images.
Here, we define a human bounding box as a tight square region that contains a detected 2D pose from edge computing systems.
The estimated chest orientation is represented as a 2D chest vector on a transverse plane.
Then, the 2D chest vector in camera space is transformed to the 2D orientation in study site coordinate, $\Vec{v}^t_{world} = R_{camera \rightarrow world}\Vec{v}^t_{world}$.
The rotation matrices, $R_{camera \rightarrow world}$, for each camera is manually defined according to the camera installation in the study site, where north is set as a reference orientation.

\subsubsection{Multi-view Integration}

% The 39 cameras installed in the study site have partially overlapping field-of-views to continuously track people across the wide space.
% Multiple cameras capture duplicate samples of the same person due to these overlaps.
In order to remove duplicated samples from overlapping field-of-views, we detect people across cameras and integrate the detections into a single sample that potentially represents the true location of the person, as shown in \autoref{fig:muti-view_integration}.
To detect duplicated detections, we generate a graph, $G=(V,E)$, where vertices, $V=\{v_{ci}=(x,y)|c=1,\cdots,39, i=1,\cdots\}$, are locations of all samples from all 39 cameras and edge, $E=\{v_{ci}v_{c'j} |\; c \neq c' \}$, is the connectivity between samples from different cameras that are sufficiently close in the distance.
We assume that duplicates are coming from the same person captured in different cameras, if their Euclidean distance is within $\| v_{ci} - v_{c'j} \|_2 \leq 1.5 m$, considering the error margin of our localization technique.
It is possible for the same person located from a different camera to be in a slightly different location from our indoor localization due to lens distortions violating planar assumptions about the floor that can incur inaccuracies in perspective transformations.
% that is used for perspective transformation in our indoor localization technique.
Regardless, we empirically found that only 1.5 meters were sufficient for the margin of the localization error~\cite{zhang2000flexible}.

Once the graph $G$ is constructed, the duplicated samples are identified as those with linked vertices in a graph, which is also called connected components, $CC$, from graph theory~\cite{john1995first}.
Then, we integrate the locations of the duplicated samples considering the camera distance from the detected sample. 
Specifically, when integrating duplicated samples, the samples are penalized when the camera distance is far, as the localization error and the distance between the camera and the target person were strongly correlated in our analysis.

\begin{equation}
    L = \sum_{CC} \frac{1}{d_{ci}} v_{ci}
\end{equation}

\noindent where $L$ is the location of integrated sample and $d_{ci} = \| l_c - v_{ci} \|^2_2$ is the euclidean distance between the sample, $v_{ci}$, and the camera, $l_c$.
% According to our findings, the localization error and the distance between the camera and the target person are strongly correlated.
Similarly, the orientation of the duplicated samples is integrated for the vertices in $CC$ considering camera distances.
The multi-view integration results in unique locations, $L=[l_x, l_y]$, and orientation vectors, $o=[o_x, o_y]$, of each person at each time step.  

\subsubsection{Multi-person Tracking}

\input{figure/data_collection.tex}

% To understand detailed individual or group movements occurring in the study site, the locations of people need to be tracked across time.
We apply Kalman filter-based tracking for the locations, $L=[l_x, l_y]$, and orientation vector, $O=[o_x, o_y]$, assuming that people's facing orientation follows their walking direction closely~\cite{kuhn1955hungarian}.

\begin{equation}
    O_t= O_{t-1} + w\cdot \dot{L}_{t-1} + dt\cdot \dot{O}_{t-1}
\end{equation}

\noindent where $w=0.1$ is a weighting of moving direction (or velocity) on current orientation and $dt$ is the time interval between frames, which is 1 sec.
% The tracker follows predict, detect, match, update, and repeat steps used in Sec.~\ref{sec:preproc_poses}, but with some differences.
% We again use a linear constant model for both location and orientation, where states are represented as location, $L=[l_x, l_y]$, orientation, $O=[o_x, o_y]$, velocity, $\dot{L}=[\dot{l}_x, \dot{l}_y]$, and angular velocity, $\dot{O}=[\dot{o}_x, \dot{o}_y]$.
We further applied RTS smoothing for finished trackers to consider temporal dynamics across the entire trajectory of a person.
% Therefore, the tracker estimates facing orientation at time $t$ by summing up both moving directions, the velocity when 1 Hz, $\dot{L}$, and angular velocity, $\dot{O}$.

% When associating predictions and matching using Hungarian matching, the bipartite graph is represented as a matrix, where $C_{i,j}= \|L^i_{p} - L^j_{d} \|_2$ is euclidean distance between $i$th sample from prediction, $L_p$, and $j$th sample from detection, $L_d$.
% Likewise earlier, we applied RTS smoothing for finished trackers to consider temporal dynamics across the entire trajectory of a person.

\subsection{Benchmark Data Collection}\label{sec:benchmark_data_collection}

To systematically evaluate the performance of the localization, body orientation estimation, and tracking system using edge computing platforms, we produced a manually annotated dataset that consists of four to five subjects moving and interacting at the study site.
The benchmark dataset includes a group of people 1) walking together, 2) walking past each other, or 3) conversing in place while changing facing orientations. 

\revision{
We taped the entire space with 1-meter markers for ground-truth annotation. 
}
The subjects were asked to walk according to pre-planned group formations and walking paths.
While people were walking, an observer annotated the exact time and location of each subject at each second.
The observer manually annotated the body orientation of the subjects using north (upper direction for \autoref{fig:ep6_func}) as a reference.



Below we describe three datasets that we created to capture different types of activities in the space.

\subsubsection{4 People Walking around Entire Space}

Our first benchmark dataset has four people walking around the study site.
\autoref{fig:data_collection} describes the locations and paths taken by participants to consider the realistic use cases of the study site by visitors. We covered areas that are of interest for tracking behaviors in the study space (\autoref{fig:data_collection}a). 
Those include locations mainly used by the visitors for eating (dining area and kitchen), physical exercises, lounge, and staff zones (\autoref{fig:ep6_func}), where subjects agreed to being captured.

For the annotation, we selected the closest 1-meter markers as the ground-truth location of the subjects while they were walking, which resolution was sufficient to consider the varying foot size and stride length of each participant.
While walking, we also changed the group formation to simulate realistic movement in the space (\autoref{fig:data_collection}c).
For the wider corridors, group formations of two or three people walking side-by-side were used whereas in narrow corridors multiple subjects walked in straight lines. Walking in groups helped to test the effect of occlusions, where subjects are not seen from a camera viewpoint.

\subsubsection{5 People Walking Past Each other}

We also collected a benchmark dataset when multiple subjects show more complex movements.
Shown in \autoref{fig:data_collection}b, we simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions that frequently occurs while performing dancing or group exercises.

\subsubsection{5 people Changing Orientations in Place}

\input{figure/orientation_inplace}
\input{figure/cam_install_protocol}

People often sit or stand stationary while having group conversations and only change facing directions to interact.
Shown in \autoref{fig:ori_in_place}, we collected a benchmark dataset, where people make subtle changes in facing orientation in place.
From Session 1 to 3, we increased the size of the social group from two to five. 
A social group is defined as people actively communicating at a distance closer than 2 meters, considering social distancing due to the ongoing pandemic.
According to instructions, participants gradually changed the facing direction. 
%by switching whose members were communicating with whom.


\subsection{Evaluating Multi-person Tracking and Localization}

We evaluate our activity monitoring system with respect to localization, tracking, and body orientation estimation performances following the standard evaluation methods~\cite{bernardin2006multiple,wu2020mebow}.
As there is no single metric for evaluating multi-person tracking methods, we utilize the following metrics to understand the performance of the proposed system~\cite{dendorfer2020mot20}.
$\uparrow$ and $\downarrow$ are shown for the metrics that are higher or lower the better, respectively.

\begin{itemize}
    \item MOTA $\uparrow$ (Multi-Object Tracking Accuracy) combines three kinds of error sources, which are false positives, missed targets, and identity switches.    
    \item IDF1 $\uparrow$ (ID F1 score) is the ratio of correctly identified detections over the average number of ground-truth and computed detections.
    \item MT $\uparrow$ (Mostly Tracked targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at least 80\% of their respective life span.
    \item ML $\downarrow$ (Mostly Lost targets) measures the ratio of ground-truth trajectories that are covered by a track hypothesis for at most 20\% of their respective life span.
    \item FPR $\downarrow$ (False Positives Rate) measures the average number of false alarms per frame.
    \item FNR $\downarrow$ (False Negatives Rate) measures the average number of missed targets per frame.
    \item Rcll $\uparrow$ (Recall) measures the ratio of correct detections to the total number of ground-truth locations.
    \item Prcn $\uparrow$ (Precision) measures the number of detected objects over the sum of detected and false positives.
    \item IDSR $\downarrow$ (ID Switch Ratio) measures the number of ID switches (IDS) over recall.
    \item Frag $\downarrow$  (Fragmentation) measures the total number of times a trajectory is fragmented, which are interruptions during tracking.
\end{itemize}

Specifically, $MOTA=1-\frac{\sum_t FN_t + FP_t + IDS_t}{\sum_t GT_t}$,
where $FN_t$, $FP_t$, $IDS_t$, and $GT_t$ are false negatives (misses), false positives, ID switches, and ground-truths at time $t$.
One important evaluation that preceded tracking is detection. 
In this work, we define a ground-truth target at the time $t$ is detected if the estimated sample location is within 1.5 meters in euclidean distance.
Otherwise, the target is considered as \textit{missed}. 
The 1.5-meter reference is based on the fact that people rarely walk faster than 1.42 m/s on an everyday basis~\cite{browning2006effects,mohler2007visual,levine1999pace}.

To demonstrate the localization accuracy of the estimated samples, we also report multiple object tracking precision, $MOTP=\frac{\sum_{i,t} d^i_t}{\sum_t c_t}$.
$d^i_t$ is the euclidean distance between the $i$th detected ground-truth sample and estimated sample, and $c_t$ is the number of detection at time $t$. 
In other words, MOTP is the average euclidean distance error for the detected samples, which shows the performance of the proposed systems to estimate the precise location of target samples that is independent of tracking trajectories or ID switches.

% \subsubsection{Multi-person Tracking Baseline}

% Our proposed tracker is compared with a Hungarian matching-based tracker~\cite{kuhn1955hungarian}, which only considers frame-by-frame matching between 2D pose detections, in order to illustrate the importance of modeling temporal dynamics of 2D movements.
% Based on the results of multiview multi-person localization at time $t$ and $t+1$, the Hungarian tracker generates a bipartite graph with nodes representing samples from two consecutive timesteps and edges representing Euclidean distances between samples. 
% Since our tracking rate is 1 Hz, we remove any edge distance larger than 1.5 meters in the created bipartite graph, as people normally walk 1.42 m/s in everyday activities~\cite{browning2006effects,mohler2007visual,levine1999pace}.
% Then, the Hungarian method finds the matchings (or edges) that have a minimum sum of Euclidean distances.
% Potentially missing samples (false negatives) in a frame $t$ are filled in by linearly interpolating the matched detection from frame $t-1$ and $t+1$.
% The Hungarian matching is applied until no matching is found any longer over time.

\subsection{Evaluating Body Orientation Estimation}

Following the standard definition of body orientation in the previous work~\cite{wu2020mebow,yu2019continuous,andriluka2010monocular}, we defined the human orientation $\theta \in [0\degree, 360\degree)$ as the chest facing direction on the transverse plane that is projected to the 2D coordinate in the study site, where the north (top) direction is the reference with clock-wise rotation.
We use two metrics as in previous works~\cite{wu2020mebow}: Mean Absolute Error (MAE) of angular distance and Accuracy-$X\degree$.
Accuracy-$X\degree$ is defined as the ratio of the samples that are predicted within the deviation of $X\degree$ according to the ground-truth orientation. 
By using $X\in [0\degree, 180\degree]$, Accuracy-$X\degree$ measures fine-grained model accuracy.
Specifically, we used $X\in\{5\degree, 15\degree, 22.5\degree, 30\degree, 45\degree, 90\degree\}$~\cite{wu2020mebow}.

% \subsubsection{Comparing Body Orientation Estimation Baselines}

% Our body orientation method inherently learns the geometric relationship between 2D pose, 3D pose, and the corresponding body orientation of the observed human bounding box.
% We compare the proposed method with two baselines that only use 2D information and then a baseline that only models the 3D geometry of detected 2D poses.
% Through this practice, we will demonstrate the importance of modeling both 3D geometry and pose-body orientation relationships.

% \noindent i) \textit{2D pose-based Heuristic Approach:}
% This method uses a heuristic approach to estimate body orientation from only 2D pose information.
% Specifically, it uses 2D facial keypoints, including nose, eyes, and ears, and estimates the 2D vector originating from the average of left and right eyes and ears keypoints to nose keypoints on 2D image pixels.
% We directly project those 2D vectors from the image frame to the 2D coordinate space of the study site using a perspective transformation matrix, $M$, derived from Sec.~\ref{sec:indoor_localization}.

% \noindent ii) \textit{2D pose-based Deep Learning Approach:}
% This baseline model applied a learning-based method, where the model directly estimates body orientation from 2D pose input.
% We used a graphical convolutional network (GCN)~\cite{yan2018spatial} to process 2D pose data to predict body orientation angle in 5-\degree intervals.
% For training the model, we used MS COCO 2D keypoints~\cite{lin2014microsoft} dataset and the corresponding body orientation annotation provided by  Wu~\etal~\cite{wu2020mebow}.
% We augmented 2D keypoints input by randomly flipping horizontally or adding Gaussian noises to simulate noisy pose detections from our pipeline.

% \noindent iii) \textit{2D-3D pose Geometric matching-based Approach:}
% To model the 3D geometry of the human body pose~\cite{takahashi2018human}, we first estimated 3D pose information from the detected 2D poses from our pipeline.
% We lift the estimated 2D poses to 3D poses by using the 3D pose estimation method~\cite{pavllo20193d}.
% Then, the 3D poses are calibrated according to the camera viewpoint using Perspective-n-point projection technique~\cite{lepetit2009epnp}.
% Specifically, at each time step $t$, we learn the extrinsic parameters, which are rotation and translation matrices, of the estimated 3D chest keypoints (left and right shoulders and left and right pelvis) for projecting 3D pose to the corresponding 2D keypoints in the image space. 

% \begin{equation}
%     [R|T]^t = \arg\min_{R,T}\| p^t_2 - sK[R|T]p^t_3 \|
% \end{equation}

% \noindent where $R\in\mathbb{R}^{3\times 3}$ is a rotation matrix subject to $R^TR=I\in\mathbb{R}^{3\times3}$ and $det(R) = 1$ and $T\in\mathbb{R}^{3\times 1}$ is a translation matrix that minimizes the projection error of chest keypoints of 3D pose, $p^t_3$, to 2D pose, $p^t_2$, at timestep $t$ given intrinsic camera lense parameter, $K\in\mathbb{R}^{3\times 3}$.
% We fix the camera intrinsic matrix, $K$, with the parameters provided by the manufacturer~\cite{rpi_camera} and the scale parameter is arbitrarily set to $s=1$ as we do not require the absolute scale of the 3d pose size, but only the facing direction.
% For each person, we smoothed $[R|T]^t$ over all time steps using moving SLERP filter~\cite{shoemake1985animating} and moving average filter for rotation and translation matrices, respectively, to keep the temporal consistency.
% From the 3D pose calibrated according to the chest orientation, we acquire the 3D chest norm vector perpendicular to the left-to-right shoulder vector and left shoulder-to-left pelvis vector, $\Vec{v}^t_{chest} = \Vec{v}^t_{L.Shoulder \rightarrow R.Shoulder} \times \Vec{v}^t_{L.Shoulder \rightarrow L.Pelvis}$, at each timestep $t$.
% The estimated 3D chest norm vector is projected to a 2D chest vector on a transverse plane, which represents the facing of each people in the scene with respect to the camera viewpoint.

\subsection{Impact of Camera Installation}

% In our study site, the camera installation is determined primarily by the power and network sources reachable using extension cables, with minimum modification to the existing building structure, resulting in 39 cameras unequally installed in the space.
\revision{
We also quantitatively examine the impact of camera installation in more detail on four different factors on the performance of our system, shown in \autoref{fig:cam_install_protocol}.
Specifically, we demonstrate the relationship between the location and facing orientation of the subjects captured in the video frame from each camera relating to localization and body orientation estimation accuracy.
This analysis demonstrates the error budget from per-camera indoor localization (Sec.~\ref{sec:indoor_localization}) and body orientation estimation (Sec.~\ref{sec:body_ori_est}) with respect to the final performance of our system.
}

\subsubsection{Distance Between Camera and Person}

Across all cameras, we measured the distance between captured people from the camera center, as shown in \autoref{fig:cam_install_protocol}a, that will be associated with localization and orientation errors.

\subsubsection{Facing Angle with respect to Camera Viewpoint}

\input{figure/mot_result}
\input{table/mot_fpr_fnr_onlyKF_captionShort}

We collected the degree of facing directions of the captured person deviating from camera viewpoints, as shown n \autoref{fig:cam_install_protocol}b, and conducted correlation analysis with the corresponding localization and orientation errors.

\subsubsection{Horizontal Displacement from Camera Center}

We studied the impact of the horizontal displacement of the captured person from the camera center (\autoref{fig:cam_install_protocol}c).
We quantified the horizontal displacement as the horizontal angle, $\theta\degree_H$, of the person from the camera center that is normalized by horizontal field-of-view, $\theta\degree_{H_{FOV}}$, which is normalized horizontal angle, $\sfrac{\theta\degree_H}{\theta\degree_{H_{FOV}}}$.
As a person gets closer to the horizontal center of the camera, the normalized horizontal angle approaches zero.
The normalized horizontal angle increases to $1$ when the person is at the edge of the frame. 
When the value is larger than $1$, then only part of the body is observable from the camera.
We examine how localization and orientation errors vary with the degree of horizontal displacement.

\subsubsection{Vertical Displacement from Camera Center}

Following horizontal displacement, we studied the effect of vertical displacement of a person from the camera center (\autoref{fig:cam_install_protocol}d).
The vertical displacement was quantified as a vertical angle, $\theta\degree_V$, of the person captured from the camera center that is normalized by vertical field-of-view, $\theta\degree_{V_{FOV}}$, referring to the camera datasheet, namely normalized vertical angle, $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$.
We specifically consider the foot location, which we use to localize, as a point of reference to calculate the normalized vertical angle.
When the person is closer to the camera, the normalized vertical angle increases, and only the upper body is partially captured by the camera due to the limited vertical field of view.
On the other hand, as the person moves away from the camera, the normalized vertical angle decreases and can capture the full body in the field of view, but with the cost of increased distance between the camera and the person.
We will study the changes in localization and orientation errors based on the vertical displacement of the captured person.


==> sections/related/main.tex <==
\section{Related Work}

%We propose a privacy-preserving indoor localization and tracking system using a distributed multi-camera network. Here, we will introduce a general overview of indoor localization techniques. We will then discuss approaches for processing image and video data on edge devices while preserving provacy for subjects.

\subsection{Indoor Localization and Tracking}

Passive and continuous monitoring of patient movement can significantly reduce the operational costs for nurses and prevent in-hospital infections in smart hospitals~\cite{kwon2022review}.
Further, tracking patients' movements can also provide clues about their mental and physical health, such as how much social interaction they have on a daily basis or how physically active they are.
% However, it is challenging to run a tracking system for multiple patients and staffs throughout days across the wide built-in space.
Various sensors are used to track movements indoors, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR) sensors~\cite{cheol2017using}, WiFi~\cite{van2016performance}, BlueTooth~\cite{yoo2018real}, or ultra-wideband (UWB)~\cite{kearns2016decreased}.
However, those techniques are either short-ranged or based on proximity detection, which can only coarsely monitor the patients' whereabouts, such as room-level localization~\cite{bazo2021survey}.
Those sensors has to be very densely installed in indoor environment, which requires significant modification of the existing infrastructure, to capture the continuous trajectory of patients and staff across entire indoor spaces with fine-granularity.
Our work, however, aims to monitor detail locations and trajectories throughout interior spaces using sparsely distributed multiple cameras with low-cost edge computing systems, which is also very easy to install in existing indoor environments.
The proposed system is potentially useful for capturing, for example, critical behaviors in therapeutic units like our study site. 
It is possible for patients with cognitive impairment to gradually lose spatial and temporal awareness and get confused about their location, even in familiar surroundings.
It is important to detect such moments early on to prevent severe consequences, such as eloping and getting lost~\cite{haslam2022real}.%\yash{I would refer to high-impact non-biomedical engineering works on indoor localization and tracking too. Here is one for marketing purposes~\cite{basiri2017indoor}}\hyeok{Yash, sorry, but I don't understand your comments here. The reference you shared is also based on technological solutions. I will just keep this section as it is now.}
%contact tracing in hospitals to prevent in-hospital transmission of infectious diseases~\cite{hellmich2017contact} 

\subsection{Vision-based Localization and Tracking}

There have been a number of studies using camera-based passive monitoring systems to capture detailed activities related to health.
With the recent advances in multi-person pose estimation and tracking methods~\cite{dai2022survey,dos2021monocular}, many works used cameras to detect daily routines~\cite{luo2018computer} or gait-related~\cite{xue2018vision} activities to monitor the health of seniors or patient mobilization at intensive care units~\cite{yeung2019computer}.
These studies had the major limitation of requiring subjects to perform activities inside the room where the camera was installed, making it difficult to monitor activities continuously across large areas.

A recent study used multiple distributed depth cameras to track staff and patient movements across an entire hospital floor, thereby detecting potential hospital-acquired infections~\cite{haque2017towards}.
This type of system is highly effective, but requires the installation of depth sensors in hospital infrastructure for data capture and transfer, which can be time-consuming and expensive.
In this work, we propose a multi-person localization and tracking system using distributed camera network with edge computing framework that is easy-to-install and low-cost, making it possible to turn any ordinary indoor space into a smart environment to support advanced patient behavior analysis.

\subsection{Privacy-preserving Video Analysis}

An ambient camera provides rich information on the context of subject's behavior in the scene.
% And, many breakthroughs in computer vision technology is capable of using those rich context to serve users, such as in-patient monitoring~\cite{} or mental health detection~\cite{}.
This, however, comes with the risk of privacy breaches.
There have been several attempts to use videos while protecting user privacy.
For privacy-preserving computer vision, there are essentially two approaches, one at the hardware level and one at the software level.
Studies using hardware-based approaches have rarely
% \yash{I would use rarely}\hyeok{done}
used color cameras. 
To safeguard the privacy of monitored subjects, those works used depth or thermal
% \yash{how about LiDAR?}\hyeok{LiDAR is the depth sensor.} 
cameras that is installed in one corner of the room~\cite{martinez2018real,xue2018vision}.
In contrast to color cameras, depth map cameras measure the distance between an object and the camera center, while thermal cameras measure the scene's heat signature.
Others, however, still proposed privacy-preserving color cameras through the significant degradation at the image-sensing stages.
% \chaitra{what has also been explored using color cameras?}\hyeok{addressed.}
The techniques include applying low-resolution images, defocusing the lens, and modulating the lens phase, as well as implementing a coded aperture system to hide sensitive information~\cite{ryoo2017privacy,hinojosa2022privhar,purwanto2019extreme,pittaluga2015privacy,pittaluga2016pre,wang2019privacy}

Software-level approaches removed sensitive information from the video frames after the acquisition, while retaining the crucial information for downstream analysis. 
Numerous works, for instance, use human or face detection and tracking to continuously blur or cover privacy-invasive information~\cite{agrawal2011person,chen2007tools,padilla2015visual}.
In recent years, generative model-based approaches have been proposed to replace sensitive information with unidentifiable data, based on generic privacy factors (skin color, face, gender, nudity, and relationship)~\cite{wu2020privacy,brkic2017know,pittaluga2019learning,ren2018learning,wu2018towards}.
In our work, we use a software-level approach in order to use the standard camera for estimating location and orientation over time. Unlike previous work that uses image degradation or image generation, we use real-time pose estimation on the edge computing system without saving raw frames, and only transmit multi-person pose estimations over the secure network.
% Privacy is compromised when sensitive data is stored (data breach) or communicated over the open network (data leak)\yash{Since we've already mentioned this sentence and plan to elaborate on it in the next one, I think the sentence is redundant}.\hyeok{Agreed.}
% Our proposed system is secure, as we do not transmit raw data, but only pose information based on computing on the network edge.

\subsection{Intelligent System on Edge Devices}

As smartphones and wearables become more common, machine learning at the network edge is becoming increasingly important to support various analytical tasks~\cite{jin2022survey,suresha2022edge,barthelemy2019edge}.
For intelligent ambient sensing, edge computing devices, such as Raspberry Pi~\cite{rpi}, can attach a variety of sensors, including a camera, microphone, temperature sensor, and humidity sensor, using General-Purpose Input/Output (GPIO).
With dedicated machine learning frameworks and computing units, such as TensorFlow Lite~\cite{tflite} and Google Coral TPU USB Accelerator~\cite{tpu}, on-device machine learning has become feasible~\cite{baller2021deepedgebench}.
Many types of intelligent systems operate at the edge of networks, including image recognition~\cite{wang2018bandwidth,kang2018c}, ECG classification~\cite{mohandas2021use}, speech recognition~\cite{lin2018edgespeechnets,chen2014small}, and more.
Similarly, this work uses a multi-person pose estimation model~\cite{papandreou2018personlab} run on 39 edge computing systems with Google Coral TPU USB Accelerator using Tensorflow lite framework to estimate poses in real-time.

==> sections/related/main_20230329.tex <==
\section{Related Work}

We propose a privacy-preserving indoor localization and tracking system using a distributed multi-camera network.
Here, we will introduce a general overview of indoor localization techniques.
We will then discuss approaches for processing image and video data on edge devices while keeping users' privacy.

\subsection{Indoor Localization and Tracking}

Passive and continuous monitoring of patient movement can significantly reduce the operational costs for nurses and prevent in-hospital infections in smart hospitals~\cite{kwon2022review}.
Further, tracking patients' movements can also provide clues about their mental and physical health, such as how much social interaction they have on a daily basis or how physically active they are.
% However, it is challenging to run a tracking system for multiple patients and staffs throughout days across the wide built-in space.
Various sensors are used to track movements indoors, including radio-frequency identification (RFID)~\cite{vuong2014automated}, infrared (IR) sensors~\cite{cheol2017using}, WiFi~\cite{van2016performance}, BlueTooth~\cite{yoo2018real}, or ultra-wideband (UWB)~\cite{kearns2016decreased}.
However, those techniques are either short-ranged or based on proximity detection, which can only coarsely monitor the patients' whereabouts, such as room-level localization~\cite{bazo2021survey}, that can limit the ability to capture the continuous trajectory of patients and staff across entire indoor spaces with fine-granularity.
Our work, however, aims to monitor detail locations and trajectories throughout interior spaces using multiple cameras, which will potentially be useful for capturing, for example, critical behaviors in clinics. 
It is possible for patients with cognitive impairment to gradually lose spatial and temporal awareness and get confused about their location, even in familiar surroundings.
It is important to detect such moments early on to prevent severe consequences, such as eloping and getting lost~\cite{haslam2022real}.%\yash{I would refer to high-impact non-biomedical engineering works on indoor localization and tracking too. Here is one for marketing purposes~\cite{basiri2017indoor}}\hyeok{Yash, sorry, but I don't understand your comments here. The reference you shared is also based on technological solutions. I will just keep this section as it is now.}
%contact tracing in hospitals to prevent in-hospital transmission of infectious diseases~\cite{hellmich2017contact} 

\subsection{Vision-based Localization and Tracking}

There have been a number of studies using camera-based passive monitoring systems to capture detailed activities related to health.
With the recent advances in multi-person pose estimation and tracking methods~\cite{dai2022survey,dos2021monocular}, many works used cameras to detect daily routines~\cite{luo2018computer} or gait-related~\cite{xue2018vision} activities to monitor the health of seniors or patient mobilization at intensive care units~\cite{yeung2019computer}.
These studies had the major limitation of requiring users to perform activities inside the room where the camera was installed, making it difficult to monitor activities continuously across large areas.

A recent study used multiple distributed depth cameras to track staff and patient movements across an entire hospital floor, thereby detecting potential hospital-acquired infections~\cite{haque2017towards}.
This type of system is highly effective, but requires the installation of depth sensors in hospital infrastructure for data capture and transfer, which can be time-consuming and expensive.
In this work, we propose a multi-person localization and tracking system using distributed camera network with edge computing framework that is easy-to-install and low-cost, making it possible to turn any ordinary indoor space into a smart environment to support advanced user behavior analysis.

\subsection{Privacy-preserving Video Analysis}

The ambient camera provides rich information on the context of users' behavior in the scene.
% And, many breakthroughs in computer vision technology is capable of using those rich context to serve users, such as in-patient monitoring~\cite{} or mental health detection~\cite{}.
This, however, comes with the risk of privacy breaches.
There have been several attempts to use videos while protecting user privacy.
For privacy-preserving computer vision, there are essentially two approaches, one at the hardware level and one at the software level.
Studies using hardware-based approaches have rarely
% \yash{I would use rarely}\hyeok{done}
used color cameras. 
To safeguard the privacy of users, those works used depth or thermal
% \yash{how about LiDAR?}\hyeok{LiDAR is the depth sensor.} 
cameras that is installed in one corner of the room~\cite{martinez2018real,xue2018vision}.
In contrast to color cameras, depth map cameras measure the distance between an object and the camera center, while thermal cameras measure the scene's heat signature.
Others, however, still proposed privacy-preserving color cameras through the significant degradation at the image-sensing stages.
% \chaitra{what has also been explored using color cameras?}\hyeok{addressed.}
The techniques include applying low-resolution images, defocusing the lens, and modulating the lens phase, as well as implementing a coded aperture system to hide sensitive information~\cite{ryoo2017privacy,hinojosa2022privhar,purwanto2019extreme,pittaluga2015privacy,pittaluga2016pre,wang2019privacy}

Software-level approaches removed sensitive information from the video frames after the acquisition, while retaining the crucial information for downstream analysis. 
Numerous works, for instance, use human or face detection and tracking to continuously blur or cover privacy-invasive information~\cite{agrawal2011person,chen2007tools,padilla2015visual}.
In recent years, generative model-based approaches have been proposed to replace sensitive information with unidentifiable data, based on generic privacy factors (skin color, face, gender, nudity, and relationship)~\cite{wu2020privacy,brkic2017know,pittaluga2019learning,ren2018learning,wu2018towards}.
In our work, we use a software-level approach in order to use the standard camera.
To estimate location and orientation over time, however, we don't use image degradation or image generation as in previous work.
Instead, we use real-time pose estimation on the device without saving raw frames and only send multi-person pose estimations over the network.
% Privacy is compromised when sensitive data is stored (data breach) or communicated over the open network (data leak)\yash{Since we've already mentioned this sentence and plan to elaborate on it in the next one, I think the sentence is redundant}.\hyeok{Agreed.}
Our proposed system is secure, as we do not transmit raw data, but only pose information based on computing on the network edge.

\subsection{Intelligent System on Edge Devices}

As smartphones and wearables become more common, machine learning at the network edge is becoming increasingly important to support various analytical tasks~\cite{jin2022survey,suresha2022edge,barthelemy2019edge}.
For intelligent ambient sensing, edge computing devices, such as Raspberry Pi~\cite{rpi}, can attach a variety of sensors, including a camera, microphone, temperature sensor, and humidity sensor, using General-Purpose Input/Output (GPIO).
With dedicated machine learning frameworks and computing units, such as TensorFlow Lite~\cite{tflite} and Google Coral TPU USB Accelerator~\cite{tpu}, on-device machine learning has become feasible~\cite{baller2021deepedgebench}.
Many types of intelligent systems operate at the edge of networks, including image recognition~\cite{wang2018bandwidth,kang2018c}, ECG classification~\cite{mohandas2021use}, speech recognition~\cite{lin2018edgespeechnets,chen2014small}, and more.
Similarly, this work uses a multi-person pose estimation model~\cite{papandreou2018personlab} run on 39 Raspberry Pis with Google Coral TPU USB Accelerator using Tensorflow lite framework to estimate poses in real-time.

==> sections/result/_main_20230329.tex <==
\section{Result}

In this section, we demonstrate the performance of the localization, tracking, and body orientation estimation of the proposed system based on the metric described earlier, which is also compared with the baseline methods.
% The performances are evaluated at different locations separately in the study site, including the activity area (A), kitchen (B), left corridor (C), right corridor (E), lobby (D), and staff area (F) as shown in \autoref{fig:data_collection}.
% For body orientation estimation, we show additional performance on various group formation in activity area where majority of group activities are performed in the study site.

\subsection{Multi-person Tracking and Localization}

\input{figure/mot_result}

\subsubsection{4 People Walking around Entire Space}

Here, we show overall performance while four people walk together in the entire area of the study site.
\autoref{fig:mot_result} and \autoref{tab:mot} show the result of multi-person tracking and localization at each functional area.
Referring \autoref{fig:ep6_func} and \autoref{fig:data_collection}, Activity Area (A) includes both the Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and left boundary of conversation room.
The left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor where the Lockers are left to the Innovation Theater.
The lounge (D) includes the area between the elevator and the front door, 
% \chaitra{we have not shown anywhere what the front desk is. Should we change fig 6 to include this?}\hyeok{Replaced this with front door.}
and the Staff area (F) includes the region on the right side of the building where staff offices are located.
Different locations have varying sizes of captured area of the study space shown as shown in te 2nd column of \autoref{tab:mot}, and varying number of cameras as shown in the 3rd column of \autoref{tab:mot} which shows the number of cameras that were capturing the 85\% of the samples.

Let's first look into the performance of the Hungarian tracker (\autoref{tab:mot}, upper 1-7 rows), which only considers matching between subsequent frames.
Overall MOTA 
% \yash{I think it is misleading to use \% for MOTA metric}\hyeok{I know ... but, that is a convention ...}
and IDF1 scores (\autoref{tab:mot}, upper 7th row) are not robust to noisy detections and false negative samples showing only 47.6\% MOTA, 36.6\% IDF1, and 49\% Recall.
The major source of error was in high False negative rate (FNR=1.8) and ID switch rate (IDSR=41.47), showing that carefully handling noisy detections is critical when especially using 2D pose estimation models on edge devices.
This demonstrates the importance of considering temporal dynamics over time given noisy and missing detections from our 2D pose detector.
To run the pose detection model on Raspberry Pi, a resource-constrained 
% \robert{Just want to make sure we didn't mean to say "constrained" here instead}\hyeok{I learned something!}
% device, we are currently using the model that is specifically tailored to emphasize efficiency over performance compared to the state-of-the-art models~\cite{dos2021monocular}. \robert{Pretty sure this needs to say "state-of-the-art" unless I've misunderstood something.}\hyeok{Good eyes!}
The model showed low reliability across all study sites.
For the locations where only a single camera was available, 
% \robert{Should this read "for the locations where only a single camera was available", or "for the location where only a single camera was available"?}\hyeok{former!}
for example, the Lounge area (D) had the lowest MOTA score (19.2\%).
% This demonstrates the significance of capturing temporal dynamics of movements to handle noisy detections, even when multiple (seven in Activity Area) cameras are covering the capture space.
For Activity Area (A), where seven cameras were tracking movements, the model shows 77.6\% MOTA.
This shows that the density of the camera is especially important when detections are noisy, as overlapping viewpoints help to capture people from the front, back, and side while walking, as shown in \autoref{fig:camera_config}. 

\input{table/mot_fpr_fnr}

In the bottom half of \autoref{tab:mot}, our proposed model significantly outperformed the Hungarian tracker (\autoref{tab:mot}, bottom 7th row).
MOTA and IDF1 were significantly higher than the Hungarian-based tracker, having an absolute increase of 15.3\% and  14.6\%, respectively.
The overall MOTA score was 62.9\%, showing that our system could track people accurately over 60\%  cases considering FP, FN, and IDS all combined.
The performance increase compared to Hungarian tracker came from significantly decreased False negative rate (FNR=34\%) and increased Recall (69\%).
This again shows capturing temporal dynamics to handle noisy detections is critical in our edge computing framework.
The localization performance (MOTP) was $1.41m$, which was within a reasonable error range considering $1Hz$ while walking.
As noted earlier, people normally walk $1.42m/s$ in everyday activities, and our ground truth annotations have a margin of 1-meter error as the participants' locations were labeled as the closest 1-meter interval marker in the space.
Overall evaluation shows that when the proposed model detects and tracks the person the model can consistently track people over the sequence, and can also handle certain degree of missing detections (FNs) due to the limitations in multi-person pose detection model.
This was also reflected in high Precision (93.48\%), high MT (1.83), and low ML (0.33).
The results demonstrate that modeling temporal dynamics of movement is crucial for accurate multi-person tracking. 
MOTA and IDF1 scores increased significantly when compared to the Hungarian-based tracker, although MOTPs were similar between the two models.

% Major source of error was from high FNs (490; \autoref{tab:mot}, 7th row) compared to reasonable FPs(103; \autoref{tab:mot}, 7th row) and IDS (9.58; \autoref{tab:mot}, 7th row).
% We will later demonstrate the severity of FNs, when using a tracker that does not handle missing detections considering temporal dynamics in Sec.~\autoref{sec:mot_cmp}.

The performance of the model varied depending on the areas but again with significantly increased performance compared to the Hungarian tracker.
% \yash{whats your take on having almost similar MOTP but observing meaningfully better MOTA?} \hyeok{I added a summary sentence in the end of the previous paragraph.}
For the Activity area, where most physical activity happens in the study site, MOTA score was 88.63\%, 
% \yash{I would change the Recall, Precision, MOTA, and etc represention to either \% or decimal}\hyeok{Thanks. Kept everything to \%}
and MOTP was $1.38m$ with high Precision (95.6\%) and Recall (93.62\%), which is sufficient to detect, track and understand group activity and space usage behavior in this area.
The lower MOTA was observed when only a few (two or three) cameras were available to cover the wide captured space.
Kitchen, Left Corridor, or Right Corridor had 67.16\%, 54.53\%, 60.25\% MOTA and $1.48m$, $1.92m$, and $1.75m$ MOTP, respectively.
The Kitchen, Left Corridor, and Right Corridor had long corridors, which are $24m\times 3m$, $33m\times 2m$, and $33m\times 1.5m$, respectively.
Having few cameras for those regions to capture people from far was severely hampered by the occlusion and challenges in detecting poses, due to too small pixel region for each person, resulting in high FNRs (1.01, 1.53, 1.56, respectively). 
However, our system still showed high Precision (95.6\%, 91.3\%, 100\%) in those regions, showing that detected objects are mostly correct detections.

Staff Zone has four cameras installed to capture movements from the sides (left and right) while walking.
The size of the staff zone ($14m\times 3m$) is the smallest compared to other areas, which also makes cameras capture people closer in the distance.
This resulted in a higher MOTA score (73.47\%) with a lower MOTP score ($1.11m$) and lower FNRs (0.40) compared to other areas.
The Lounge area only has one camera covering the space and had the lowest performance with a MOTA score of 33.44\%. 
This was mainly due to the shortage of power and network source near the lounge area, where only a single camera was available to cover the entire space. Additionally, there are occlusions from the front desk, chairs, and stems.
In summary, our experiment results show that 1) modeling temporal dynamics is important in multi-person tracking when using noisy detections and that 2) denser camera installation with closer distance to people with multiple view can result in highly accurate localization and tracking performance (low MOTP and high MOTA scores).
In Sec.~\ref{sec:cam_install}, we will demonstrate further the correlation between camera installation and localization accuracy.


% the multi-person localization tracking performance shows the importance of the distance between the object and camera and the number of cameras with different views covering the area.
% Person closer to the camera were more accurately localized and tracked (low MOTP and high MOTA scores).

\subsubsection{5 People Walking Past Each other}

% \input{table/mot_traj}

We evaluated multi-person tracking performance when multiple people were showing more complex movements.
We simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions.
As mentioned earlier, Activity Area is the location where most physical activities are occurring in the study space, and also the region where our pipeline showed the highest accuracy due to denser camera installation.
The qualitative and quantitative results are shown in \autoref{fig:mot_result}, (b) and \autoref{tab:mot}, last row, respectively.
Even in such challenging cases, the MOTA score, MOTP socre, and IDF1 score were 79.8\%, 1.44m, and 70\% score, showing robust performance with low ID switch errors when people were passing by one another.
Our observation found that having four cameras capturing the activities from different views could compensate for occlusions while people actively move.

\subsection{Body Orientation Estimation}

\input{table/orientation.tex}

The body orientation estimation results are shown in \autoref{tab:orientation}.
Here, we demonstrate the body orientation estimation evaluation from two datasets used for evaluating multi-person tracking performance, which are four people walking around the entire space, and five people moving passed each other in Activity Area.
In addition, we evaluated body orientation when five people formed in varying groups remained stationary while changing orientation.

\subsubsection{4 People Walking around Entire Space}

While four participants walk, the overall (\autoref{tab:orientation}, 7th row) MAE was 28.97$\degree$ and Acc.-45\degree as 78.9\%, which is sufficient to tell eight (N, NE, E, SE, S, SW, W, NW) orientations reliably. 
% \yash{We need some explanation about how we found the ground truth labels to body orientation?}\hyeok{Added this in the Sec.~\ref{sec:benchmark_data_collection}}
Similarly to the previous experiment, the performance of orientation estimation varied across the study space, depending on the captured area size and the number of cameras covering the space.
Activity Area (\autoref{tab:orientation}, 1st row), having seven cameras from the front, back, and sides with the most overlapping views, had errors showing 25.91$\degree$ MAE, and, Staff Zone (\autoref{tab:orientation}, 6th row) also had comparably lower MAE (32.41\degree) as this area has four cameras installed with overlapping field-of-views with close distance to people.
Left and Right Corridors (\autoref{tab:orientation}, 3rd and 5th rows), where low MOTA score was observed, surprisingly had low errors as well, 21.68\degree and 32.41\degree MAEs, respectively.
These areas had challenges in localization and tracking due to lower number of cameras covering the narrow and long distances.
But, for body orientation estimation, due to the narrow width of the corridor, it was easy for the model to estimate body orientations from human bounding box images since people tend to face forward or opposite to the camera viewpoints when they are moving. 
For the Lounge area (\autoref{tab:orientation}, 4th rows), where only a single camera is covering the space, it was very difficult to accurately identify body orientations, with 47.37\degree\; MAE and Acc.-45\degree\; of 55.4\%.
Similar to localization and tracking analysis, the occlusions and people far from the camera were challenging for body orientation. 
In Sec.~\ref{sec:cam_install}, we will investigate further the correlation between the camera installation and body orientation estimation.

\subsubsection{5 People Walking Past Each other}

The body orientation estimation model was significantly confused by the occlusions for a more challenging movement scenario (\autoref{tab:orientation}, 8th rows).
When people are walking past each other and close to one another, multiple people with different orientations can be captured in a human bounding box.
This resulted in a high MAE of 48.33\degree and low Acc.-45\degree (62.9\%).
These findings provide a baseline for group activity analysis in a crowded area, as understanding group activity requires finding group formation and facing directions while moving.
Yet, Acc.-90\degree showed 81.4\%, where our model can identify equally spaced four cardinal directions (N, E, S, W) at minimum, even when people are closely located together and dynamically changing group formations.

\subsubsection{5 people Changing Orientations in Place}

\input{figure/orientation_inplace}

People often sit or stand stationary in daily social interactions, such as group conversations, and only change facing directions to interact.
We evaluated how well body orientation estimation performed when people moved in place, as shown in \autoref{fig:ori_in_place}.
From Session 1 to 3, we increased the size of the social group from two to five. 
A social group is defined as people actively communicating at a distance closer than 2 meters, considering social distancing due to the ongoing pandemic.
According to instructions, participants gradually changed the facing direction. 
%by switching whose members were communicating with whom.
When evaluating this scenario, the model demonstrated a significant error rate (\autoref{tab:orientation}, last row), in which MAE was 63.4\degree.
Similarly, in the five-person experiment, the model was able to identify equally spaced four directions (N, E, S, W) at minimum, showing Acc.-90\degree of 69.3\%.
The major source of error was coming from the occlusions between people close in the distance, as multiple people were captured in a human bounding box challenging the body orientation estimating of the target person.
% These findings were consistent with the analysis observed in the experiment, where five people were moving passed each other, having significant occlusions across samples.
Furthermore, our body orientation estimation model found it difficult to detect slight changes in facing direction between subsequent frames, as the model makes frame-by-frame estimation.
This also shows that our model performed better when people were walking as the Kalman Filter updates the orientation information to incorporate moving directions as the user moves.

The accuracy of each session also showed differences according to the number of cameras and the size of captured areas covered by those cameras.
Session 1 (\autoref{tab:orientation}, 9th row), where three cameras were covering $55m^2$ space, showed MAE of 73.7\degree, although the samples only had small size groups having two or three members.
The MAE (65.2\degree) was lower in Session 2 (\autoref{tab:orientation}, 10th row), where members had a group size of four, but the capture area ($28m^2$) was smaller than that of Session 1, clearly demonstrating the importance of camera density.
This was more apparent for Session 3 (\autoref{tab:orientation}, 11th row), which has a social group size of 5 people, but with the lowest MAE (50.4\degree) amongst all three sessions.
The capture space was only $15m^2$ and four cameras were available.
To summarize, our body orientation estimation pipeline performed more reliably when more cameras were available to handle confusion from occlusions. 
Also, the Kalman filter-based tracker demonstrated a greater degree of accuracy when people were moving in a consistent direction, even when occlusions were present in the human bounding boxes, since the state transition considers movement directions across time.

\subsubsection{Comparing Body Orientation Estimation Baselines}

\input{table/orientation_compare}

\autoref{tab:ori_compare} shows the performance of the proposed body orientation model compared with three different baseline models, when tested on four people walking around the study site.

i) \textit{2D pose-based heuristic approach}: It showed a significantly high error showing an overall MAE of 130.34\degree (\autoref{tab:ori_compare}, 1st row).
The high error came from the lack of depth information in 2D poses and noisy 2D pose detections.
This heuristic method worked only when the person was facing toward the camera point of view, and slight rotation significantly decreased accuracy.

ii) \textit{2D pose-based Deep Learning Approach}: The trained model showed a Mean Absolute Error (MAE) of 17.2\degree for the MS COCO validation dataset.
When the trained model was deployed to our pipeline, the model demonstrated a MAE of 108.34\degree (\autoref{tab:ori_compare}, 2nd row).
Directly modeling complex function that maps 2D poses to facing orientation in the traverse plane outperformed the heuristic method.
Nevertheless, the lack of depth and 3D modeling significantly impacted the performance of the application.
In addition, the domain shift from clean and manually annotated MS COCO keypoints to noisy pose detections, such as unrealistically twisted or wide 2D poses, made generalizing the model extremely difficult.

iii) \textit{2D-3D pose Geometric matching-based Approach}: Using 3D information significantly improved the performance, which resulted in an MAE of 74.59\degree (\autoref{tab:ori_compare}, 3rd row) compared to 2D-based approaches above.
This demonstrates that body orientation estimation inherently requires 3D information.
Because of noisy 2D poses, which also degraded the accuracy of lifted 3D poses, the model could not capture facing orientations sufficiently well.
This resulted in inaccurate perspective projection between 3D and 2D poses, which is already an ill-posed problem.
Some samples were estimated to have nearly 180\degree errors.

Compared to all baseline models, the proposed method (MAE of 28.97\degree; \autoref{tab:ori_compare}, 4th row) demonstrated the best performance, showing an absolute decrease of 45.6\degree\; from the 3D-Geometry-based method.
The proposed body orientation estimation model is trained to inherently learn 3D and 2D poses and their complex relationships regarding body orientation directly from human bounding box images.
This complemented the limitation of the 2D-Learning-based approach and 3D-Geometry-based approach demonstrating best-performing method among all.

%-----

% \input{figure/orientation.tex}

% We also show the Accuracy-$X\degree$ results for each location in \autoref{fig:ori-accuracy-x}.
% The $X\degree=45,\; 90\; 120$ from \autoref{tab:orientation} are highlighted with \textcolor{red}{RED}, \textcolor{green}{GREEN}, and \textcolor{blue}{BLUE} for each area.
% Considering the error limit of 90\degree to tell four-way directions, Activity Area and Staff Zone, where multiple cameras are installed, shows Acc.-90\degree $\approx 65\%$.
% For the other locations (Kitchen, Left Corridor, Right Corridor, and Lounge), where the cameras are fewer, the accuracy was lower showing Acc.-90\degree $\leq 50\%$.
% Especially for Lounge area, the accuracy was especially lower showing Acc.-120\degree $\leq 45\%$.
% We observed that the distance of people from the camera and occlusions resulted in significantly distorted 2D poses, which accumulated the error across orientation estimation pipeline (\textcolor{red}{Figure required})
% Overall, our model is expected to provide how the facing direction of people changes, although coarse estimate of four-way directions (N,E,S,W), along with the location changes and tracking during group activities in the study site.


==> sections/result/_main_chaitra_20231029.tex <==
\section{Result}

In this section, we demonstrate the performance of the proposed localization, tracking, and body orientation estimation methods using the metrics described earlier. We also compare our methods with the baseline methods.

\subsection{Multi-person Tracking and Localization}

\input{figure/mot_result}
\input{table/mot_fpr_fnr}

\subsubsection{4 People Walking around Entire Space}

\input{table/orientation.tex}

Here, we show overall performance while four people walk together in the entire area of the study site.
\autoref{fig:mot_result} and \autoref{tab:mot} show the result of multi-person tracking and localization at each functional area.
Different locations have varying sizes of the captured area (\autoref{tab:mot}, 2nd column) and varying numbers of cameras (\autoref{tab:mot}, 3rd column) that were capturing 85\% of the samples.

Let's first look into the performance of the Hungarian tracker (\autoref{tab:mot}, upper 1-7 rows), which only considers matching between subsequent frames.
Overall MOTA and IDF1 scores (\autoref{tab:mot}, upper 7th row) shows that the model is not robust to noisy detections and false negative samples, resulting in only 47.6\% MOTA, 36.6\% IDF1, and 49\% recall.
The major source of error was in high False negative rate (FNR=1.8) and ID switch rate (IDSR=41.47), showing that carefully handling noisy detections is critical when using 2D pose estimation models on edge devices.
To run the pose detection model on edge computing system, a resource-constrained device, we are currently using the model that is specifically tailored to emphasize efficiency over performance compared to the state-of-the-art models~\cite{dos2021monocular}. 
The model showed low reliability across all study sites.
For the locations where only a single camera was available low MOTA scores were obtained. For example the MOTA score obtained in the Lounge area (D) was the lowest at 19.2\%.
For the Activity Area (A), where seven cameras were tracking movements, the model showed 77.6\% MOTA.
This shows that the density of the camera is especially important when detections are noisy, as overlapping viewpoints help to capture people from the front, back, and side while walking, as shown in \autoref{fig:camera_config}. 

In the bottom half of \autoref{tab:mot}, our proposed model significantly outperformed the Hungarian tracker (\autoref{tab:mot}, bottom 7th row).
MOTA and IDF1 were significantly higher than the Hungarian-based tracker, having an absolute increase of 15.3\% and  14.6\%, respectively.
The overall MOTA score was 62.9\%, showing that our system could track people accurately over 60\%  cases considering FP, FN, and IDS all combined.
The performance increase compared to Hungarian tracker came from significantly decreased False negative rate (FNR=1.24) and increased Recall (69\%).
This demonstrates the importance of considering temporal dynamics over time given noisy and missing detections from our 2D pose detector.

The localization performance (MOTP) was $1.41m$, which was within a reasonable error range considering $1Hz$ while walking.
As noted earlier, people normally walk $1.42m/s$ in everyday activities, and our ground truth annotations have a margin of 1-meter error as the participants' locations were labeled as the closest 1-meter interval marker in the space.
Overall evaluation shows that the proposed model can consistently track people over the sequence if the person is detected,
% \chaitra{can you specify what this sentence is trying to imply? I think there's a gramatical error but I'm not sure what the sentence is trying to convey}\hyeok{done.}
and can also handle certain degree of missing detections (FNs) coming from the limitations in the multi-person pose detection model on edge computing systems.
This was also reflected in high Precision (93.48\%), high MT (1.83), and low ML (0.33).
The results demonstrate that modeling temporal dynamics of movement is crucial for accurate multi-person tracking. 
MOTA and IDF1 scores increased significantly when compared to the Hungarian-based tracker, although MOTPs were similar between the two models.

The performance of the model varied depending on the areas in the study space but again with significantly increased performance compared to the Hungarian tracker.
For the Activity area, where most physical activity happens in the study site, MOTA score was 88.63\%, and MOTP was $1.38m$ with high Precision (95.6\%) and Recall (93.62\%), which is sufficient to detect, track and understand group activity and space usage behavior in this area.
The lower MOTA was observed when only a few (two or three) cameras were available to cover the wide capture space.
Kitchen, Left Corridor, or Right Corridor had 67.16\%, 54.53\%, 60.25\% MOTA and $1.48m$, $1.92m$, and $1.75m$ MOTP, respectively.
The Kitchen, Left Corridor, and Right Corridor had long corridors, which are $24m\times 3m$, $33m\times 2m$, and $33m\times 1.5m$, respectively.
Having few cameras for those regions to capture people from far was severely hampered by the occlusion and challenges in detecting poses, due to too small pixel region for each person, resulting in high FNRs (1.01, 1.53, 1.56, respectively). 
However, our system still showed high Precision (95.6\%, 91.3\%, 100\%) in those regions, showing that detected objects are mostly correctly localized.

Staff Zone has four cameras installed to capture movements from the sides (left and right) while walking.
The size of the staff zone ($14m\times 3m$) is the smallest compared to other areas, which also makes cameras capture people closer in the distance.
This resulted in a higher MOTA score (73.47\%) with a lower MOTP score ($1.11m$) and lower FNRs (0.40) compared to other areas.
The Lounge area only has one camera covering the space and had the lowest performance with a MOTA score of 33.44\%. 
This was mainly due to the shortage of power and network source near the lounge area, where only a single camera was available to cover the entire space. Additionally, there are occlusions from the front desk, chairs, and other items.
In summary, our experiment results show that 1) modeling temporal dynamics is important in multi-person tracking when using noisy detections and that 2) denser camera installation with closer distance to people with multiple view can result in highly accurate localization and tracking performance (low MOTP and high MOTA scores).
In Sec.~\ref{sec:cam_install}, we will demonstrate further the correlation between camera installation and localization accuracy.


% the multi-person localization tracking performance shows the importance of the distance between the object and camera and the number of cameras with different views covering the area.
% Person closer to the camera were more accurately localized and tracked (low MOTP and high MOTA scores).

\subsubsection{5 People Walking Past Each other}

% \input{table/mot_traj}

We evaluated multi-person tracking performance when multiple people were showing more complex movements.
We simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions.
As mentioned earlier, Activity Area is the location where most physical activities are occurring in the study space, and also the region where our pipeline showed the highest accuracy due to denser camera installation.
The qualitative and quantitative results are shown in \autoref{fig:mot_result}, (b) and \autoref{tab:mot}, last row, respectively.
Even in such challenging cases, the MOTA score, MOTP socre, and IDF1 score were 79.8\%, 1.44m, and 70\% score, showing robust performance with low ID switch errors when people were passing by one another.
Our observation found that having four cameras capturing the activities from different views could compensate for occlusions while people actively move.

\subsection{Body Orientation Estimation}

Here, the body orientation estimation results on our benchmark dataset are shown in \autoref{tab:orientation}.
We first demonstrate evaluations from two datasets used for evaluating multi-person tracking performance, which are four people walking around the entire space, and five people moving past each other in Activity Area.
Then, we additionally show evaluated body orientation when five people formed in varying groups remained stationary while changing orientation.

\subsubsection{4 People Walking around Entire Space}

\input{table/orientation_compare}

While four participants walk, the overall (\autoref{tab:orientation}, 7th row) MAE was 28.97$\degree$ and Acc.-45\degree as 78.9\%, which is sufficient to tell eight (N, NE, E, SE, S, SW, W, NW) orientations reliably. 
Similar to the previous experiment, the performance of orientation estimation varied across the study space, depending on the captured area size and the number of cameras covering the space.
Activity Area (\autoref{tab:orientation}, 1st row), having seven cameras from the front, back, and sides with the most overlapping views, had errors showing 25.91$\degree$ MAE, and, Staff Zone (\autoref{tab:orientation}, 6th row) also had comparably lower MAE (32.41\degree) as this area has four cameras installed with overlapping field-of-views with close distance to people.
Left and Right Corridors (\autoref{tab:orientation}, 3rd and 5th rows), where low MOTA score was observed, surprisingly had low errors as well, 21.68\degree and 32.41\degree MAEs, respectively.
These areas had challenges in localization and tracking due to lower number of cameras covering the narrow and long distances.
But, for body orientation estimation, due to the narrow width of the corridor, it was easy for the model to estimate body orientations from human bounding box images since people tend to face forward or opposite to the camera viewpoints when they are moving. 
For the Lounge area (\autoref{tab:orientation}, 4th rows), where only a single camera is covering the space, it was very difficult to identify body orientations, with 47.37\degree\; MAE and Acc.-45\degree\; of 55.4\%.
Similar to localization and tracking analysis, the occlusions and people far from the camera were challenging for body orientation. 
In Sec.~\ref{sec:cam_install}, we will investigate further the correlation between the camera installation and body orientation estimation.

\subsubsection{5 People Walking Past Each other}

The body orientation estimation model was significantly confused by the occlusions for a more challenging movement scenario (\autoref{tab:orientation}, 8th rows).
When people are walking past each other and close to one another, multiple people with different orientations can be captured in a human bounding box.
This resulted in a high MAE of 48.33\degree and low Acc.-45\degree (62.9\%).
These findings provide a baseline for group activity analysis in a crowded area, as understanding group activity requires finding group formation and facing directions while moving.
Yet, Acc.-90\degree showed 81.4\%, where our model can identify four equally spaced cardinal directions (N, E, S, W) at minimum, even when people are closely located together and dynamically changing group formations.

\subsubsection{5 people Changing Orientations in Place}

When evaluating this scenario, the model demonstrated a significant error rate (\autoref{tab:orientation}, last row), in which MAE was 63.4\degree.
Similarly, in the five-person experiment, the model was able to identify equally spaced four directions (N, E, S, W) at minimum, showing Acc.-90\degree of 69.3\%.
The major source of error was coming from the occlusions between people close in the distance, as multiple people were captured in a human bounding box challenging the body orientation estimating of the target person.
Furthermore, our body orientation estimation model found it difficult to detect slight changes in facing direction between subsequent frames, as the model makes frame-by-frame estimation.
This also shows that our model performed better when people were walking as the Kalman Filter updates the orientation information to incorporate moving directions as the person moves.

The accuracy of each session also showed differences according to the number of cameras and the size of captured areas covered by those cameras.
Session 1 (\autoref{tab:orientation}, 9th row), where three cameras were covering $55m^2$ space, showed MAE of 73.7\degree, although the samples only had small size groups having two or three members.
The MAE (65.2\degree) was lower in Session 2 (\autoref{tab:orientation}, 10th row), where members had a group size of four, but the capture area ($28m^2$) was smaller than that of Session 1, clearly demonstrating the importance of camera density.
This was more apparent for Session 3 (\autoref{tab:orientation}, 11th row), which has a social group size of 5 people, but with the lowest MAE (50.4\degree) amongst all three sessions.
The capture space was only $15m^2$ and four cameras were available.
To summarize, our body orientation estimation pipeline performed more reliably when more cameras were available to handle confusion from occlusions. 
Also, the Kalman filter-based tracker demonstrated a greater degree of accuracy when people were moving in a consistent direction, even when occlusions were present in the human bounding boxes, since the state transition considers movement directions across time.

\subsubsection{Comparing Body Orientation Estimation Baselines}

\input{figure/discuss_cam_install_corr_only}

\autoref{tab:ori_compare} shows the performance of the proposed body orientation model compared with three different baseline models, when tested on four people walking around the study site.

\noindent i) \textit{2D pose-based heuristic approach}: It showed a significantly high error showing an overall MAE of 130.34\degree (\autoref{tab:ori_compare}, 1st row).
The high error came from the lack of depth information in 2D poses and noisy 2D pose detections.
This heuristic method worked only when the person was facing toward the camera point of view, and slight rotation significantly decreased accuracy.

\noindent ii) \textit{2D pose-based Deep Learning Approach}: The trained model showed a Mean Absolute Error (MAE) of $17.2\degree$ for the MS COCO validation dataset.
However, when the trained model was deployed to our pipeline, the model demonstrated a MAE of $108.34\degree$ (\autoref{tab:ori_compare}, 2nd row).
Directly modeling complex function that maps 2D poses to facing orientation in the transverse plane outperformed the heuristic method.
Nevertheless, the lack of depth and 3D modeling significantly impacted the performance of the application.
In addition, the domain shift from clean and manually annotated MS COCO keypoints to noisy pose detections, such as unrealistically twisted or wide 2D poses, made generalizing the model extremely difficult.

\noindent iii) \textit{2D-3D pose Geometric matching-based Approach}: Using 3D information significantly improved the performance, which resulted in an MAE of $74.59\degree$ (\autoref{tab:ori_compare}, 3rd row) compared to 2D-based approaches above.
This demonstrates that body orientation estimation inherently requires 3D information.
Because of noisy 2D poses, which also degraded the accuracy of lifted 3D poses, the model could not capture facing orientations sufficiently well.
This resulted in inaccurate perspective projection between 3D and 2D poses, which is already an ill-posed problem.
Some samples were estimated to have nearly $180\degree$ errors.

Compared to all baseline models, the proposed method (MAE of 28.97\degree; \autoref{tab:ori_compare}, 4th row) demonstrated the best performance, showing an absolute decrease of $45.6\degree$ from the 3D-Geometry-based method.
The proposed body orientation estimation model is trained to inherently learn 3D and 2D poses and their complex relationships regarding body orientation directly from human bounding box images.
This complemented the limitation of the 2D-Learning-based approach and 3D-Geometry-based approach demonstrating best-performing method among all.

%-----

\subsection{Impact of Parameters of Camera Installation on Model Behavior}
\label{sec:cam_install}

From our localization and body orientation analysis, we observed that the density of the cameras (number of cameras per captured area size) is highly correlated with the localization and orientation estimation accuracy.
Here, we examine this in more detail to understand the impact of four different factors of camera installation related to localization and body orientation estimation accuracy.
\autoref{fig:corr_analysis} shows Pearson correlation analysis for each factor we study, where denser samples are colored more \textcolor{blue}{BLUE}.

\subsubsection{Distance Between Camera and Person}

In \autoref{fig:corr_analysis} (1st col), localization error (1st row) showed that the majority of our samples were within $\sim2$ meters error when the distance between the person and camera was within 15 meters.
A strong positive correlation exists between the localization error and camera distance as the distance increases beyond 20 meters ($R=0.823$, $p<0.005$). 
Orientation error (1st col, 2nd row) also demonstrated a positive correlation with increase in distance of the captured person from the camera ($R=0.335$, $p < 0.005$).
The majority of orientation errors were less than $25\degree$ when the location of captured person was less than 15 meters from the camera.
This shows that the edge computing camera (Sony IMX219 8-megapixel sensor) can capture objects well within 15 meters, which is large enough for our pose estimation and body orientation estimation models to make accurate predictions.
As a result of the person being further away from the camera, the pixel region that constitutes the person decreases significantly, which increases the errors in body orientation and localization.
The models was more confused when people were occluding each other, as multiple people looked like a single person from a distance.

\subsubsection{Facing Angle with Respect to Camera Viewpoint}

The facing direction of the captured person had a significant impact on the accuracy of both localization and body orientation estimation (\autoref{fig:corr_analysis}; 2nd col).
Facing angles within $50\degree$ of the camera line-of-sight were found to be crucial to ensuring a $<2m$ localization error and a $<25\degree$ body orientation error.
Specifically, the 2D pose estimation model performed best when the person was facing the camera, and as the person turned away from the camera, more distortions were introduced to the estimated keypoint locations, which affected localization accuracy.
This was similar to the body orientation estimation model, as the confidence of the model was high when the person was facing forward. 
The model had more confusion as the person started facing away from the camera.
Many times, pose estimation models confused frontal and rear views of the person, especially when the person was farther than $20m$ from the camera, resulting in unrealistically twisted keypoints.
There was a strong positive correlation between the facing angle with respect to camera viewpoint and both localization ($R=0.375$, $p<0.005$) and body orientation estimation ($R=0.436$, $p<0.005$) errors.

\subsubsection{Horizontal Displacement from Camera Center}

According to our analysis, a person must be captured within 30\% of the horizontal field of view 
% \chaitra{What is horizontal camera displacement?}\hyeok{I updated this to horizontal field of view}
to have a localization error of less than $2m$ and an orientation error of less than 25\degree, as shown in \autoref{fig:corr_analysis} (3rd col.).
The localization and body orientation estimation errors increased with strong positive correlations as the captured person moved away from the horizontal center, $R=0.681 (p<0.005)$ and $R=0.467 (p<0.005)$, respectively.
Again, this illustrates the advantage of densely installing cameras to capture people with overlapping viewpoints of $30\degree$ horizontal angle displacements.

\subsubsection{Vertical Displacement from Camera Center}

Shown in \autoref{fig:corr_analysis} (4th col.), with our edge computing camera module, the foot locations of people with $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \geq 0.8$ were not captured sufficiently, and the pose estimation model could not detect the person.
For $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$ closer to zero, localization and body orientation error increased significantly, with the increased distance between the captured person and the camera.
On the whole, as the person approached the vertical camera center the localization and orientation estimation errors decreased due to the increase in coverage of more body parts, with a strong negative correlation $R=-0.495 (p<0.005)$ and $R=-0.317 (p<0.005)$ for localization and orientation estimation respectively.
The optimal range of normalized vertical angle was between $0.05\leq \sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \leq 0.2$, which were equivalent of $6m$ to $23m$ distance between the captured person and the camera, which draws a similar conclusion from camera horizontal distance analysis earlier.

==> sections/result/_main_old.tex <==
\section{Result}

In this section, we demonstrate the performance of the localization, tracking, and body orientation estimation of the proposed system based on the metric described earlier, which is also compared with the baseline methods.
% The performances are evaluated at different locations separately in the study site, including the activity area (A), kitchen (B), left corridor (C), right corridor (E), lobby (D), and staff area (F) as shown in \autoref{fig:data_collection}.
% For body orientation estimation, we show additional performance on various group formation in activity area where majority of group activities are performed in the study site.

\subsection{Multi-person Tracking and Localization}

\input{figure/mot_result}

\subsubsection{4 People Walking around Entire Space}

Here, we show overall performance while four people walk together in the entire area of the study site.
\autoref{fig:mot_result} and \autoref{tab:mot} show the result of multi-person tracking and localization at each functional area.
Different locations have varying sizes of the captured area (\autoref{tab:mot}, 2nd column) and varying numbers of cameras (\autoref{tab:mot}, 3rd column) that were capturing the 85\% of the samples.

Let's first look into the performance of the Hungarian tracker (\autoref{tab:mot}, upper 1-7 rows), which only considers matching between subsequent frames.
Overall MOTA 
% \yash{I think it is misleading to use \% for MOTA metric}\hyeok{I know ... but, that is a convention ...}
and IDF1 scores (\autoref{tab:mot}, upper 7th row) shows that the model is not robust to noisy detections and false negative samples, resulting in only 47.6\% MOTA, 36.6\% IDF1, and 49\% Recall.
The major source of error was in high False negative rate (FNR=1.8) and ID switch rate (IDSR=41.47), showing that carefully handling noisy detections is critical when especially using 2D pose estimation models on edge devices.
To run the pose detection model on Raspberry Pi, a resource-constrained 
% \robert{Just want to make sure we didn't mean to say "constrained" here instead}\hyeok{I learned something!}
device, we are currently using the model that is specifically tailored to emphasize efficiency over performance compared to the state-of-the-art models~\cite{dos2021monocular}. 
% \robert{Pretty sure this needs to say "state-of-the-art" unless I've misunderstood something.}\hyeok{Good eyes!}
The model showed low reliability across all study sites.
For the locations where only a single camera was available, 
% \robert{Should this read "for the locations where only a single camera was available", or "for the location where only a single camera was available"?}\hyeok{former!}
for example, the Lounge area (D) had the lowest MOTA score (19.2\%).
% This demonstrates the significance of capturing temporal dynamics of movements to handle noisy detections, even when multiple (seven in Activity Area) cameras are covering the capture space.
For Activity Area (A), where seven cameras were tracking movements, the model shows 77.6\% MOTA.
This shows that the density of the camera is especially important when detections are noisy, as overlapping viewpoints help to capture people from the front, back, and side while walking, as shown in \autoref{fig:camera_config}. 

\input{table/mot_fpr_fnr}

In the bottom half of \autoref{tab:mot}, our proposed model significantly outperformed the Hungarian tracker (\autoref{tab:mot}, bottom 7th row).
MOTA and IDF1 were significantly higher than the Hungarian-based tracker, having an absolute increase of 15.3\% and  14.6\%, respectively.
The overall MOTA score was 62.9\%, showing that our system could track people accurately over 60\%  cases considering FP, FN, and IDS all combined.
The performance increase compared to Hungarian tracker came from significantly decreased False negative rate (FNR=1.24) and increased Recall (69\%).
This demonstrates the importance of considering temporal dynamics over time given noisy and missing detections from our 2D pose detector.
% This again shows capturing temporal dynamics to handle noisy detections is critical in our edge computing framework.
The localization performance (MOTP) was $1.41m$, which was within a reasonable error range considering $1Hz$ while walking.
As noted earlier, people normally walk $1.42m/s$ in everyday activities, and our ground truth annotations have a margin of 1-meter error as the participants' locations were labeled as the closest 1-meter interval marker in the space.
Overall evaluation shows that when the proposed model detects and tracks the person the model can consistently track people over the sequence, and can also handle certain degree of missing detections (FNs) coming from the limitations in multi-person pose detection model.
This was also reflected in high Precision (93.48\%), high MT (1.83), and low ML (0.33).
The results demonstrate that modeling temporal dynamics of movement is crucial for accurate multi-person tracking. 
MOTA and IDF1 scores increased significantly when compared to the Hungarian-based tracker, although MOTPs were similar between the two models.

% Major source of error was from high FNs (490; \autoref{tab:mot}, 7th row) compared to reasonable FPs(103; \autoref{tab:mot}, 7th row) and IDS (9.58; \autoref{tab:mot}, 7th row).
% We will later demonstrate the severity of FNs, when using a tracker that does not handle missing detections considering temporal dynamics in Sec.~\autoref{sec:mot_cmp}.

The performance of the model varied depending on the areas but again with significantly increased performance compared to the Hungarian tracker.
% \yash{whats your take on having almost similar MOTP but observing meaningfully better MOTA?} \hyeok{I added a summary sentence in the end of the previous paragraph.}
For the Activity area, where most physical activity happens in the study site, MOTA score was 88.63\%, 
% \yash{I would change the Recall, Precision, MOTA, and etc represention to either \% or decimal}\hyeok{Thanks. Kept everything to \%}
and MOTP was $1.38m$ with high Precision (95.6\%) and Recall (93.62\%), which is sufficient to detect, track and understand group activity and space usage behavior in this area.
The lower MOTA was observed when only a few (two or three) cameras were available to cover the wide capture space.
Kitchen, Left Corridor, or Right Corridor had 67.16\%, 54.53\%, 60.25\% MOTA and $1.48m$, $1.92m$, and $1.75m$ MOTP, respectively.
The Kitchen, Left Corridor, and Right Corridor had long corridors, which are $24m\times 3m$, $33m\times 2m$, and $33m\times 1.5m$, respectively.
Having few cameras for those regions to capture people from far was severely hampered by the occlusion and challenges in detecting poses, due to too small pixel region for each person, resulting in high FNRs (1.01, 1.53, 1.56, respectively). 
However, our system still showed high Precision (95.6\%, 91.3\%, 100\%) in those regions, showing that detected objects are mostly correct detections.

Staff Zone has four cameras installed to capture movements from the sides (left and right) while walking.
The size of the staff zone ($14m\times 3m$) is the smallest compared to other areas, which also makes cameras capture people closer in the distance.
This resulted in a higher MOTA score (73.47\%) with a lower MOTP score ($1.11m$) and lower FNRs (0.40) compared to other areas.
The Lounge area only has one camera covering the space and had the lowest performance with a MOTA score of 33.44\%. 
This was mainly due to the shortage of power and network source near the lounge area, where only a single camera was available to cover the entire space. Additionally, there are occlusions from the front desk, chairs, and stems.
In summary, our experiment results show that 1) modeling temporal dynamics is important in multi-person tracking when using noisy detections and that 2) denser camera installation with closer distance to people with multiple view can result in highly accurate localization and tracking performance (low MOTP and high MOTA scores).
In Sec.~\ref{sec:cam_install}, we will demonstrate further the correlation between camera installation and localization accuracy.


% the multi-person localization tracking performance shows the importance of the distance between the object and camera and the number of cameras with different views covering the area.
% Person closer to the camera were more accurately localized and tracked (low MOTP and high MOTA scores).

\subsubsection{5 People Walking Past Each other}

% \input{table/mot_traj}

We evaluated multi-person tracking performance when multiple people were showing more complex movements.
We simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions.
As mentioned earlier, Activity Area is the location where most physical activities are occurring in the study space, and also the region where our pipeline showed the highest accuracy due to denser camera installation.
The qualitative and quantitative results are shown in \autoref{fig:mot_result}, (b) and \autoref{tab:mot}, last row, respectively.
Even in such challenging cases, the MOTA score, MOTP socre, and IDF1 score were 79.8\%, 1.44m, and 70\% score, showing robust performance with low ID switch errors when people were passing by one another.
Our observation found that having four cameras capturing the activities from different views could compensate for occlusions while people actively move.

\subsection{Body Orientation Estimation}

\input{table/orientation.tex}

Here, the body orientation estimation results on our benchmark dataset are shown in \autoref{tab:orientation}.
We first demonstrate evaluations from two datasets used for evaluating multi-person tracking performance, which are four people walking around the entire space, and five people moving passed each other in Activity Area.
Then, we additionally show evaluated body orientation when five people formed in varying groups remained stationary while changing orientation.

\subsubsection{4 People Walking around Entire Space}

While four participants walk, the overall (\autoref{tab:orientation}, 7th row) MAE was 28.97$\degree$ and Acc.-45\degree as 78.9\%, which is sufficient to tell eight (N, NE, E, SE, S, SW, W, NW) orientations reliably. 
% \yash{We need some explanation about how we found the ground truth labels to body orientation?}\hyeok{Added this in the Sec.~\ref{sec:benchmark_data_collection}}
Similarly to the previous experiment, the performance of orientation estimation varied across the study space, depending on the captured area size and the number of cameras covering the space.
Activity Area (\autoref{tab:orientation}, 1st row), having seven cameras from the front, back, and sides with the most overlapping views, had errors showing 25.91$\degree$ MAE, and, Staff Zone (\autoref{tab:orientation}, 6th row) also had comparably lower MAE (32.41\degree) as this area has four cameras installed with overlapping field-of-views with close distance to people.
Left and Right Corridors (\autoref{tab:orientation}, 3rd and 5th rows), where low MOTA score was observed, surprisingly had low errors as well, 21.68\degree and 32.41\degree MAEs, respectively.
These areas had challenges in localization and tracking due to lower number of cameras covering the narrow and long distances.
But, for body orientation estimation, due to the narrow width of the corridor, it was easy for the model to estimate body orientations from human bounding box images since people tend to face forward or opposite to the camera viewpoints when they are moving. 
For the Lounge area (\autoref{tab:orientation}, 4th rows), where only a single camera is covering the space, it was very difficult to identify body orientations, with 47.37\degree\; MAE and Acc.-45\degree\; of 55.4\%.
Similar to localization and tracking analysis, the occlusions and people far from the camera were challenging for body orientation. 
In Sec.~\ref{sec:cam_install}, we will investigate further the correlation between the camera installation and body orientation estimation.

\subsubsection{5 People Walking Past Each other}

The body orientation estimation model was significantly confused by the occlusions for a more challenging movement scenario (\autoref{tab:orientation}, 8th rows).
When people are walking past each other and close to one another, multiple people with different orientations can be captured in a human bounding box.
This resulted in a high MAE of 48.33\degree and low Acc.-45\degree (62.9\%).
These findings provide a baseline for group activity analysis in a crowded area, as understanding group activity requires finding group formation and facing directions while moving.
Yet, Acc.-90\degree showed 81.4\%, where our model can identify equally spaced four cardinal directions (N, E, S, W) at minimum, even when people are closely located together and dynamically changing group formations.

\subsubsection{5 people Changing Orientations in Place}

When evaluating this scenario, the model demonstrated a significant error rate (\autoref{tab:orientation}, last row), in which MAE was 63.4\degree.
Similarly, in the five-person experiment, the model was able to identify equally spaced four directions (N, E, S, W) at minimum, showing Acc.-90\degree of 69.3\%.
The major source of error was coming from the occlusions between people close in the distance, as multiple people were captured in a human bounding box challenging the body orientation estimating of the target person.
% These findings were consistent with the analysis observed in the experiment, where five people were moving passed each other, having significant occlusions across samples.
Furthermore, our body orientation estimation model found it difficult to detect slight changes in facing direction between subsequent frames, as the model makes frame-by-frame estimation.
This also shows that our model performed better when people were walking as the Kalman Filter updates the orientation information to incorporate moving directions as the person moves.

The accuracy of each session also showed differences according to the number of cameras and the size of captured areas covered by those cameras.
Session 1 (\autoref{tab:orientation}, 9th row), where three cameras were covering $55m^2$ space, showed MAE of 73.7\degree, although the samples only had small size groups having two or three members.
The MAE (65.2\degree) was lower in Session 2 (\autoref{tab:orientation}, 10th row), where members had a group size of four, but the capture area ($28m^2$) was smaller than that of Session 1, clearly demonstrating the importance of camera density.
This was more apparent for Session 3 (\autoref{tab:orientation}, 11th row), which has a social group size of 5 people, but with the lowest MAE (50.4\degree) amongst all three sessions.
The capture space was only $15m^2$ and four cameras were available.
To summarize, our body orientation estimation pipeline performed more reliably when more cameras were available to handle confusion from occlusions. 
Also, the Kalman filter-based tracker demonstrated a greater degree of accuracy when people were moving in a consistent direction, even when occlusions were present in the human bounding boxes, since the state transition considers movement directions across time.

\subsubsection{Comparing Body Orientation Estimation Baselines}

\input{table/orientation_compare}

\autoref{tab:ori_compare} shows the performance of the proposed body orientation model compared with three different baseline models, when tested on four people walking around the study site.

\noindent i) \textit{2D pose-based heuristic approach}: It showed a significantly high error showing an overall MAE of 130.34\degree (\autoref{tab:ori_compare}, 1st row).
The high error came from the lack of depth information in 2D poses and noisy 2D pose detections.
This heuristic method worked only when the person was facing toward the camera point of view, and slight rotation significantly decreased accuracy.

\noindent ii) \textit{2D pose-based Deep Learning Approach}: The trained model showed a Mean Absolute Error (MAE) of $17.2\degree$ for the MS COCO validation dataset.
However, when the trained model was deployed to our pipeline, the model demonstrated a MAE of $108.34\degree$ (\autoref{tab:ori_compare}, 2nd row).
Directly modeling complex function that maps 2D poses to facing orientation in the traverse plane outperformed the heuristic method.
Nevertheless, the lack of depth and 3D modeling significantly impacted the performance of the application.
In addition, the domain shift from clean and manually annotated MS COCO keypoints to noisy pose detections, such as unrealistically twisted or wide 2D poses, made generalizing the model extremely difficult.

\noindent iii) \textit{2D-3D pose Geometric matching-based Approach}: Using 3D information significantly improved the performance, which resulted in an MAE of $74.59\degree$ (\autoref{tab:ori_compare}, 3rd row) compared to 2D-based approaches above.
This demonstrates that body orientation estimation inherently requires 3D information.
Because of noisy 2D poses, which also degraded the accuracy of lifted 3D poses, the model could not capture facing orientations sufficiently well.
This resulted in inaccurate perspective projection between 3D and 2D poses, which is already an ill-posed problem.
Some samples were estimated to have nearly $180\degree$ errors.

Compared to all baseline models, the proposed method (MAE of 28.97\degree; \autoref{tab:ori_compare}, 4th row) demonstrated the best performance, showing an absolute decrease of $45.6\degree$ from the 3D-Geometry-based method.
The proposed body orientation estimation model is trained to inherently learn 3D and 2D poses and their complex relationships regarding body orientation directly from human bounding box images.
This complemented the limitation of the 2D-Learning-based approach and 3D-Geometry-based approach demonstrating best-performing method among all.

%-----

% \input{figure/orientation.tex}

% We also show the Accuracy-$X\degree$ results for each location in \autoref{fig:ori-accuracy-x}.
% The $X\degree=45,\; 90\; 120$ from \autoref{tab:orientation} are highlighted with \textcolor{red}{RED}, \textcolor{green}{GREEN}, and \textcolor{blue}{BLUE} for each area.
% Considering the error limit of 90\degree to tell four-way directions, Activity Area and Staff Zone, where multiple cameras are installed, shows Acc.-90\degree $\approx 65\%$.
% For the other locations (Kitchen, Left Corridor, Right Corridor, and Lounge), where the cameras are fewer, the accuracy was lower showing Acc.-90\degree $\leq 50\%$.
% Especially for Lounge area, the accuracy was especially lower showing Acc.-120\degree $\leq 45\%$.
% We observed that the distance of people from the camera and occlusions resulted in significantly distorted 2D poses, which accumulated the error across orientation estimation pipeline (\textcolor{red}{Figure required})
% Overall, our model is expected to provide how the facing direction of people changes, although coarse estimate of four-way directions (N,E,S,W), along with the location changes and tracking during group activities in the study site.

\subsection{Impact of Camera Installation on Model Behavior}
\label{sec:cam_install}

\input{figure/discuss_cam_install_corr_only}

From our localization and body orientation analysis, we observed the density of the cameras (number of cameras per captured area size) is highly correlated with the accuracy of the model.
Here, we examine this in more detail to understand the impact of camera installation on four different factors related to localization and body orientation estimation accuracy.
\autoref{fig:corr_analysis} shows Pearson correlation analysis for each factor we study, where denser samples are colored more \textcolor{blue}{BLUE}.

\subsubsection{Distance Between Camera and Person}

% Across all cameras, we measured the distance between captured people from the camera location and the corresponding localization errors (\autoref{fig:corr_analysis}; 1st col).
In \autoref{fig:corr_analysis} (1st col), localization error (1st row) showed that the majority of our samples were within ~ 2 meters error when the distance between the person and camera was within 15 meters.
A strong positive correlation exists between the localization error and camera distance as the distance increases from 20 meters ($R=0.823$, $p<0.005$). %\yash{whats the null hypothesis here?}\hyeok{null hypothesis is that no correlation exists.}
Orientation error (2nd row) also demonstrated a positive correlation with the increasing distance of the captured person from the camera ($R=0.335$, $p < 0.005$).
The majority of orientation errors were less than $25\degree$ when the location of captured person was below 15 meters.
This shows that the Raspberry Pi camera (Sony IMX219 8-megapixel sensor) can capture objects well within 15 meters, which is large enough for our pose estimation and body orientation estimation model to make accurate predictions.
As a result of the person being further away from the camera, the pixel region that constitutes the person decreases significantly, which increases the errors in body orientation and localization.
The model was more confused when people were occluding each other, as multiple people looked like a single person from a distance.

\subsubsection{Facing Angle Away from Camera Viewpoint}

The facing direction of the captured person had a significant impact on the accuracy of both localization and body orientation estimation (\autoref{fig:corr_analysis}; 2nd col).
The facing angles within $50\degree$ were found to be crucial to ensuring a $<2m$ localization error and a $<25\degree$ body orientation error.
Specifically, the 2D pose estimation model performed best when the person was facing the camera, and as the person turned, more distortions were introduced to the estimated keypoint locations, which affected localization accuracy.
This was similar to the body orientation estimation model, as the confidence of the model was high when the person was facing forward. 
The model had more confusion as the person started facing away from the camera.
Many times, pose estimation models confused frontal and rear views of the person, especially when the person was farther than $20m$ from the camera, resulting in unrealistically twisted keypoints.
There was a strong positive correlation between the facing angle and both localization ($R=0.375$, $p<0.005$) and body orientation estimation ($R=0.436$, $p<0.005$) errors.

\subsubsection{Horizontal Displacement from Camera Center}

According to our analysis, the person must be captured within 30\% of horizontal camera displacement to have a localization error of less than $2m$ and an orientation error of less than 25\degree, as shown in \autoref{fig:corr_analysis} (3rd col.).
The localization and body orientation errors increased with strong positive correlations as the captured person moved away from the horizontal center, $R=0.681 (p<0.005)$ and $R=0.467 (p<0.005)$, respectively.
Again, this illustrates the advantage of densely installing camera to capture people with overlapping viewpoints of $30\degree$ horizontal angle displacements.

\subsubsection{Vertical Displacement from Camera Center}

Shown in \autoref{fig:corr_analysis} (4th col.), with our Raspberry Pi Camera module, the foot locations of people with $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \geq 0.8$ were not captured sufficiently, and the pose estimation model could not detect the person.
For $\sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}}$ closer to zero, localization and body orientation error increased significantly, with the increased distance between the captured person and the camera.
On the whole, as the person approached the vertical camera center, localization and orientation errors decreased, due to the increasing coverage of more body parts, with a strong negative correlation, $R=-0.495 (p<0.005)$ and $R=-0.317 (p<0.005)$, respectively.
The optimal range of normalized vertical angle was between $0.05\leq \sfrac{\theta\degree_V}{\theta\degree_{V_{FOV}}} \leq 0.2$, which were equivalent of $6m$ to $23m$ distance between the captured person and the camera, which draws a similar conclusion from camera distance analysis earlier.

==> sections/result/main.tex <==
\section{Results}

% In this section, we demonstrate the performance of the proposed localization, tracking, and body orientation estimation methods using the metrics described earlier. 
% We also compare our methods with the baseline methods.

\subsection{Multi-person Tracking and Localization}

\subsubsection{4 People Walking around Entire Space}

\input{table/orientation_captionShort}

Here, we show overall performance while four people walk together in the entire area of the study site.
\autoref{fig:mot_result} and \autoref{tab:mot} show the result of multi-person tracking and localization at each functional area.
Different locations have varying sizes of the captured area (\autoref{tab:mot}, 2nd column) and varying numbers of cameras (\autoref{tab:mot}, 3rd column) that were capturing 85\% of the samples.
The overall MOTA score was 62.9\% and localization performance (MOTP) was $1.41m$, showing that our system could localize and track people accurately over 60\%  cases considering FP, FN, and IDS all combined.
In Sec.~\ref{sec:cam_install}, we further demonstrate a detailed analysis of the impact of camera installation on localization accuracy.

% Let's first look into the performance of the Hungarian tracker (\autoref{tab:mot}, upper 1-7 rows), which only considers matching between subsequent frames.
% Overall MOTA and IDF1 scores (\autoref{tab:mot}, upper 7th row) shows that the model is not robust to noisy detections and false negative samples, resulting in only 47.6\% MOTA, 36.6\% IDF1, and 49\% recall.
% The major source of error was in high False negative rate (FNR=1.8) and ID switch rate (IDSR=41.47), showing that carefully handling noisy detections is critical when using 2D pose estimation models on edge devices.
% To run the pose detection model on edge computing system, a resource-constrained device, we are currently using the model that is specifically tailored to emphasize efficiency over performance compared to the state-of-the-art models~\cite{dos2021monocular}. 
% The model showed low reliability across all study sites.
% For the locations where only a single camera was available low MOTA scores were obtained. For example the MOTA score obtained in the Lounge area (D) was the lowest at 19.2\%.
% For the Activity Area (A), where seven cameras were tracking movements, the model showed 77.6\% MOTA.
% This shows that the density of the camera is especially important when detections are noisy, as overlapping viewpoints help to capture people from the front, back, and side while walking, as shown in \autoref{fig:camera_config}. 

% In the bottom half of \autoref{tab:mot}, our proposed model significantly outperformed the Hungarian tracker (\autoref{tab:mot}, bottom 7th row).
% MOTA and IDF1 were significantly higher than the Hungarian-based tracker, having an absolute increase of 15.3\% and  14.6\%, respectively.
% The overall MOTA score was 62.9\%, showing that our system could track people accurately over 60\%  cases considering FP, FN, and IDS all combined.
% The performance increase compared to Hungarian tracker came from significantly decreased False negative rate (FNR=1.24) and increased Recall (69\%).
% This demonstrates the importance of considering temporal dynamics over time given noisy and missing detections from our 2D pose detector.

% The localization performance (MOTP) was $1.41m$, which was within a reasonable error range considering $1Hz$ while walking.
% As noted earlier, people normally walk $1.42m/s$ in everyday activities, and our ground truth annotations have a margin of 1-meter error as the participants' locations were labeled as the closest 1-meter interval marker in the space.
% Overall evaluation shows that the proposed model can consistently track people over the sequence if the person is detected,
% \chaitra{can you specify what this sentence is trying to imply? I think there's a gramatical error but I'm not sure what the sentence is trying to convey}\hyeok{done.}
% and can also handle certain degree of missing detections (FNs) coming from the limitations in the multi-person pose detection model on edge computing systems.
% This was also reflected in high Precision (93.48\%), high MT (1.83), and low ML (0.33).
% The results demonstrate that modeling temporal dynamics of movement is crucial for accurate multi-person tracking. 
% MOTA and IDF1 scores increased significantly when compared to the Hungarian-based tracker, although MOTPs were similar between the two models.

% The performance of the model varied depending on the areas in the study space but again with significantly increased performance compared to the Hungarian tracker.

% 1) multi-veiww  temporal dynamics is important in multi-person tracking when using noisy detections and that 2) denser camera installation with closer distance to people with multiple view can result in highly accurate localization and tracking performance (low MOTP and high MOTA scores).


% the multi-person localization tracking performance shows the importance of the distance between the object and camera and the number of cameras with different views covering the area.
% Person closer to the camera were more accurately localized and tracked (low MOTP and high MOTA scores).

\subsubsection{5 People Walking Past Each other}

% \input{table/mot_traj}

% We evaluated multi-person tracking performance when multiple people were showing more complex movements.
% We simulated a scenario in the activity area where multiple people walk toward and past each other with occlusions.
% As mentioned earlier, Activity Area is the location where most physical activities are occurring in the study space, and also the region where our pipeline showed the highest accuracy due to denser camera installation.
The qualitative and quantitative results are shown in \autoref{fig:mot_result}b and \autoref{tab:mot}, last row, respectively.
Even in this challenging cases, the MOTA score, MOTP socre, and IDF1 score were 79.8\%, 1.44m, and 70\% score, showing robust performance with low ID switch errors when people were passing by one another.

\subsection{Body Orientation Estimation}

The body orientation estimation results are shown in \autoref{tab:orientation}.
We first demonstrate evaluations from four people walking around the entire space and five people moving past each other in the Activity Area.
Then, we evaluated body orientation when five people remained stationary while changing orientation in varying group formations.

\subsubsection{4 People Walking around Entire Space}


While four participants walk, the overall (\autoref{tab:orientation}, 7th row) MAE was 28.97$\degree$ and Acc.-45\degree as 78.9\%.
In Sec.~\ref{sec:cam_install}, we will investigate further the correlation between the camera installation and body orientation estimation in detail.

\subsubsection{5 People Walking Past Each other}

When people are walking past and close to one another, multiple people with different orientations were captured in a same human bounding box challenging our body-orientation estimation technique.
As shown in \autoref{tab:orientation}, 8th rows, this resulted in a high MAE of 48.33\degree and low Acc.-45\degree (62.9\%).

\subsubsection{5 people Changing Orientations in Place}

The last four rows in \autoref{tab:orientation} show the estimation performance when a person stands in space but rotates only their orientations.
The overall performance showed an MAE of 63.40$\degree$.

% To summarize, our body orientation estimation pipeline performed more reliably when more cameras were available to handle confusion from occlusions. 
% Also, the Kalman filter-based tracker demonstrated a greater degree of accuracy when people were moving in a consistent direction, even when occlusions were present in the human bounding boxes, since the state transition considers movement directions across time.

% \subsubsection{Comparing Body Orientation Estimation Baselines}

% \input{table/orientation_compare}

% \autoref{tab:ori_compare} shows the performance of the proposed body orientation model compared with three different baseline models, when tested on four people walking around the study site.

% \noindent i) \textit{2D pose-based heuristic approach}: It showed a significantly high error showing an overall MAE of 130.34\degree (\autoref{tab:ori_compare}, 1st row).
% The high error came from the lack of depth information in 2D poses and noisy 2D pose detections.
% This heuristic method worked only when the person was facing toward the camera point of view, and slight rotation significantly decreased accuracy.

% \noindent ii) \textit{2D pose-based Deep Learning Approach}: The trained model showed a Mean Absolute Error (MAE) of $17.2\degree$ for the MS COCO validation dataset.
% However, when the trained model was deployed to our pipeline, the model demonstrated a MAE of $108.34\degree$ (\autoref{tab:ori_compare}, 2nd row).
% Directly modeling complex function that maps 2D poses to facing orientation in the transverse plane outperformed the heuristic method.
% Nevertheless, the lack of depth and 3D modeling significantly impacted the performance of the application.
% In addition, the domain shift from clean and manually annotated MS COCO keypoints to noisy pose detections, such as unrealistically twisted or wide 2D poses, made generalizing the model extremely difficult.

% \noindent iii) \textit{2D-3D pose Geometric matching-based Approach}: Using 3D information significantly improved the performance, which resulted in an MAE of $74.59\degree$ (\autoref{tab:ori_compare}, 3rd row) compared to 2D-based approaches above.
% This demonstrates that body orientation estimation inherently requires 3D information.
% Because of noisy 2D poses, which also degraded the accuracy of lifted 3D poses, the model could not capture facing orientations sufficiently well.
% This resulted in inaccurate perspective projection between 3D and 2D poses, which is already an ill-posed problem.
% Some samples were estimated to have nearly $180\degree$ errors.

% Compared to all baseline models, the proposed method (MAE of 28.97\degree; \autoref{tab:ori_compare}, 4th row) demonstrated the best performance, showing an absolute decrease of $45.6\degree$ from the 3D-Geometry-based method.
% The proposed body orientation estimation model is trained to inherently learn 3D and 2D poses and their complex relationships regarding body orientation directly from human bounding box images.
% This complemented the limitation of the 2D-Learning-based approach and 3D-Geometry-based approach demonstrating best-performing method among all.

%-----

\input{figure/discuss_cam_install_corr_only}

\subsection{Impact of Parameters of Camera Installation}
\label{sec:cam_install}

\autoref{fig:corr_analysis} shows Pearson correlation analysis for each factor from \autoref{fig:cam_install_protocol} with localization and orientation error, where denser samples are colored more \textcolor{blue}{BLUE}.

\subsubsection{Distance Between Camera and Person}

In \autoref{fig:corr_analysis}; 1st col, a strong positive correlation exists between the localization error (1st row) and camera distance as the distance increases beyond 20 meters ($R=0.823$, $p<0.005$). 
Orientation error (1st col, 2nd row) also demonstrated a positive correlation with increases in the distance of the captured person from the camera ($R=0.335$, $p < 0.005$).

\subsubsection{Facing Angle with Respect to Camera Viewpoint}

In \autoref{fig:corr_analysis}; 2nd col, there exists a strong positive correlation between the facing angle with respect to camera viewpoint and both localization ($R=0.375$, $p<0.005$) and body orientation estimation ($R=0.436$, $p<0.005$) errors.

% , and as the person turned away from the camera, more distortions were introduced to the estimated keypoint locations, which affected localization accuracy.
% This was similar to the body orientation estimation model, as the confidence of the model was high when the person was facing forward. 
% The model had more confusion as the person started facing away from the camera.

\subsubsection{Horizontal Displacement from Camera Center}

As shown in \autoref{fig:corr_analysis}; 3rd col., the localization and body orientation estimation errors increased with strong positive correlations as the captured person moved away from the horizontal center, $R=0.681 (p<0.005)$ and $R=0.467 (p<0.005)$, respectively.

% Again, this illustrates the advantage of densely installing cameras to capture people with overlapping viewpoints of $30\degree$ horizontal angle displacements.

\subsubsection{Vertical Displacement from Camera Center}

As the person approached the vertical camera center, the localization and orientation estimation errors decreased due to the increase in coverage of more body parts, with a strong negative correlation $R=-0.495 (p<0.005)$ and $R=-0.317 (p<0.005)$ for localization and orientation estimation respectively.


==> table/mot.tex <==
\begin{table}[t]
    \centering
    \caption{
    Multi-object localization and tracking performance at each area section at the study site when four participants walked around.
    The area sizes for each section are shown with height and width in meters.
    \faCamera\;
    % \yash{did we use all the cameras for all the captured frame. Let's say we have 7 cameras in the activity area, do we have footage from all 7 cameras in our dataset? if not, probably we need to point this out in the text.}\hyeok{Yes. We have footage of course and we use all of them as discussed in the method section.}
    shows the number of cameras that were covering the movement over 85\% of trajectories.
    Localization performance is measured by multiple object tracking precision (MOTP) and tracking performance was measured by multiple metrics to capture the detailed behavior of the proposed method.
    Each area is annotated referring to \autoref{fig:ep6_func} and \autoref{fig:data_collection}.
    Activity Area (A) includes both Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and the left boundary of the conversation room.
    The Left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor left of the Innovation Theater.
    Lounge (D) includes the area between the elevator and the reservation desk.
    Staff area (F) is in the right region where staff offices are located.
    Here we demonstrate the performance of both our baseline (Hungarian) and proposed (Kalman Filter) trackers. 
    \textit{Overall} performance shows average metrics across all areas combined.
    Compared to Kalman Filter-based trackers, Hungarian-based trackers do not take into account temporal dynamics of detections over time and are significantly affected by ID switching and missing samples.
    For Kalman Filter-based tracker, the last row additionally shows the quantitative results for simulating complex movements from five people with occlusions in Activity Area.
    \hyeok{Update FP and FN to per frame average}
    }
    \vspace{-0.1in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c ||c|c||c|c|c|c|c|c|c|c|c|c|c|c}          
            &
            Area & 
            Size ($H\times W$) &
            \faCamera &
            MOTP $\downarrow$ &
            MOTA $\uparrow$ & 
            IDF1 $\uparrow$ & 
            MT $\uparrow$ & 
            ML $\downarrow$ & 
            FP $\downarrow$ & 
            FN $\downarrow$ & 
            Rcll $\uparrow$ & 
            Prcn $\uparrow$ & 
            FAR $\downarrow$ & 
            IDSR $\downarrow$ & 
            Frag $\downarrow$ \\
            \hline\hline
            \multicolumn{16}{c}{Hungarian-based Tracker}\\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.25m$ & % MOTP $\downarrow$
            0.776 & % MOTA $\uparrow$  
            0.530 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            8 & % FP $\downarrow$  
            457 & % FN $\downarrow$  
            0.788 & % Rcll $\uparrow$  
            0.995 & % Prcn $\uparrow$  
            1.478 & % FAR $\downarrow$  
            22.81 & % IDSR $\downarrow$ 
            16 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.39m$ & % MOTP $\downarrow$
            0.486 & % MOTA $\uparrow$  
            0.311 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            34 & % FP $\downarrow$  
            1117 & % FN $\downarrow$  
            0.510 & % Rcll $\uparrow$  
            0.971 & % Prcn $\uparrow$  
            5.954 & % FAR $\downarrow$  
            43.05 & % IDSR $\downarrow$ 
            17 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.55m$ & % MOTP $\downarrow$
            0.496 & % MOTA $\uparrow$  
            0.360 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            13 & % FP $\downarrow$  
            1074 & % FN $\downarrow$  
            0.512 & % Rcll $\uparrow$  
            0.988 & % Prcn $\uparrow$  
            2.359 & % FAR $\downarrow$  
            44.86 & % IDSR $\downarrow$ 
            16 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.70m$ & % MOTP $\downarrow$
            0.192 & % MOTA $\uparrow$  
            0.324 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            487 & % FN $\downarrow$  
            0.193 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            5.16 & % IDSR $\downarrow$ 
            1.0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.58m$ & % MOTP $\downarrow$
            0.435 & % MOTA $\uparrow$  
            0.390 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            1229 & % FN $\downarrow$  
            0.442 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            33.90 & % IDSR $\downarrow$ 
            18 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.24m$ & % MOTP $\downarrow$
            0.574 & % MOTA $\uparrow$  
            0.370 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            514 & % FN $\downarrow$  
            0.586 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            25.56 & % IDSR $\downarrow$ 
            14 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            $1.43m$ & % MOTP $\downarrow$
            0.476 & % MOTA $\uparrow$  
            0.366 & % IDF1 $\uparrow$  
            0.777 & % MT $\uparrow$  
            0.666 & % ML $\downarrow$  
            27.88 & % FP $\downarrow$  
            1289 & % FN $\downarrow$  
            0.490 & % Rcll $\uparrow$  
            0.987 & % Prcn $\uparrow$  
            3.245 & % FAR $\downarrow$  
            41.47 & % IDSR $\downarrow$ 
            14.22 \\ %Frag $\downarrow$
            \hline\hline
            \multicolumn{16}{c}{Kalman Filter-based Tracker}\\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.38m$ & % MOTP $\downarrow$
            0.886 & % MOTA $\uparrow$  
            0.584 & % IDF1 $\uparrow$  
            4 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            94 & % FP $\downarrow$  
            138 & % FN $\downarrow$  
            0.936 & % Rcll $\uparrow$  
            0.956 & % Prcn $\uparrow$  
            17.37 & % FAR $\downarrow$  
            9.61 & % IDSR $\downarrow$ 
            6 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.48m$ & % MOTP $\downarrow$
            0.671 & % MOTA $\uparrow$  
            0.427 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            161 & % FP $\downarrow$  
            576 & % FN $\downarrow$  
            0.747 & % Rcll $\uparrow$  
            0.913 & % Prcn $\uparrow$  
            28.19 & % FAR $\downarrow$  
            17.38 & % IDSR $\downarrow$ 
            11 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.92m$ & % MOTP $\downarrow$
            0.545 & % MOTA $\uparrow$  
            0.435 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            149 & % FP $\downarrow$  
            845 & % FN $\downarrow$  
            0.616 & % Rcll $\uparrow$  
            0.901 & % Prcn $\uparrow$  
            27.04 & % FAR $\downarrow$  
            12.97 & % IDSR $\downarrow$ 
            4 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.80m$ & % MOTP $\downarrow$
            0.334 & % MOTA $\uparrow$  
            0.501 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            402 & % FN $\downarrow$  
            0.334 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            0.0 & % IDSR $\downarrow$ 
            0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.75m$ & % MOTP $\downarrow$
            0.602 & % MOTA $\uparrow$  
            0.468 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            9 & % FP $\downarrow$  
            859 & % FN $\downarrow$  
            0.610 & % Rcll $\uparrow$  
            0.993 & % Prcn $\uparrow$  
            1.633 & % FAR $\downarrow$  
            13.10 & % IDSR $\downarrow$ 
            9 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.11m$ & % MOTP $\downarrow$
            0.734 & % MOTA $\uparrow$  
            0.659 & % IDF1 $\uparrow$  
            3 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            205 & % FP $\downarrow$  
            125 & % FN $\downarrow$  
            0.899 & % Rcll $\uparrow$  
            0.845 & % Prcn $\uparrow$  
            65.91 & % FAR $\downarrow$  
            4.44 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            $\mathbf{1.41m}$ & % MOTP $\downarrow$
            \textbf{0.629} & % MOTA $\uparrow$  
            \textbf{0.512} & % IDF1 $\uparrow$  
            1.833 & % MT $\uparrow$  
            0.333 & % ML $\downarrow$  
            103 & % FP $\downarrow$  
            490.8 & % FN $\downarrow$  
            0.690 & % Rcll $\uparrow$  
            0.934 & % Prcn $\uparrow$  
            23.36 & % FAR $\downarrow$  
            9.58 & % IDSR $\downarrow$ 
            5.16 \\ %Frag $\downarrow$
            \hline\hline
            &
            5 people & 
            $13m \times 6m$ & % Size
            4 & % \faCamera
            $1.44m$ & % MOTP $\downarrow$
            0.798 & % MOTA $\uparrow$  
            0.700 & % IDF1 $\uparrow$  
            5 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            219 & % FP $\downarrow$  
            114 & % FN $\downarrow$  
            0.932 & % Rcll $\uparrow$  
            0.877 & % Prcn $\uparrow$  
            65.17 & % FAR $\downarrow$  
            6.43 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
        \end{tabular}
    \end{adjustbox}
    \label{tab:mot}
\end{table}

==> table/mot_fpr_fnr.tex <==
\begin{table*}[t]
    \centering
    \caption{
    Multi-object localization and tracking performance at each area section at the study site when four participants walked around.
    The area sizes for each section are shown with height and width in meters.
    \faCamera\;
    % \yash{did we use all the cameras for all the captured frame. Let's say we have 7 cameras in the activity area, do we have footage from all 7 cameras in our dataset? if not, probably we need to point this out in the text.}\hyeok{Yes. We have footage of course and we use all of them as discussed in the method section.}
    shows the number of cameras that were covering the movement over 85\% of trajectories.
    Localization performance is measured by multiple object tracking precision (MOTP) and tracking performance was measured by multiple metrics to capture the detailed behavior of the proposed method.
    Each area is annotated referring to \autoref{fig:data_collection}.
    % Activity Area (A) includes both Activity Studio and Gym area, and Kitchen (B) includes the upper corridor between the right boundary of the dining area and the left boundary of the conversation room.
    % The Left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor left of the Innovation Theater.
    % Lounge (D) includes the area between the elevator and the reservation desk.
    % Staff area (F) is in the right region where staff offices are located.
    Here we demonstrate the performance of both our baseline (Hungarian) and proposed (Kalman Filter) trackers. 
    \textit{Overall} performance shows average metrics across all areas combined.
    Compared to Kalman Filter-based trackers, Hungarian-based trackers do not take into account temporal dynamics of detections over time and are significantly affected by ID switching and missing samples.
    For Kalman Filter-based tracker, the last row additionally shows the quantitative results for simulating complex movements from five people with occlusions in Activity Area.
    % \hyeok{Done:Update FP and FN to per frame average}
    }
    \vspace{-0.0in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c ||c|c||c|c|c|c|c|c|c|c|c|c|c}          
            &
            Area & 
            Size ($H\times W$) &
            \faCamera &
            MOTP $\downarrow$ &
            MOTA $\uparrow$ & 
            IDF1 $\uparrow$ & 
            MT $\uparrow$ & 
            ML $\downarrow$ & 
            FPR $\downarrow$ & 
            FNR $\downarrow$ & 
            Rcll $\uparrow$ & 
            Prcn $\uparrow$ & 
            IDSR $\downarrow$ & 
            Frag $\downarrow$ \\
            \hline\hline
            \multicolumn{15}{c}{Hungarian-based Tracker}\\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.25m$ & % MOTP $\downarrow$
            0.776 & % MOTA $\uparrow$  
            0.530 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.01 & % FP $\downarrow$  8/541
            0.84 & % FN $\downarrow$  457/541
            0.788 & % Rcll $\uparrow$  
            0.995 & % Prcn $\uparrow$  
            22.81 & % IDSR $\downarrow$ 
            16 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.39m$ & % MOTP $\downarrow$
            0.486 & % MOTA $\uparrow$  
            0.311 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.06 & % FP $\downarrow$  34/571
            1.95 & % FN $\downarrow$  1117/571
            0.510 & % Rcll $\uparrow$  
            0.971 & % Prcn $\uparrow$  
            43.05 & % IDSR $\downarrow$ 
            17 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.55m$ & % MOTP $\downarrow$
            0.496 & % MOTA $\uparrow$  
            0.360 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.02 & % FP $\downarrow$  13/551
            0.94 & % FN $\downarrow$  1074/551
            0.512 & % Rcll $\uparrow$  
            0.988 & % Prcn $\uparrow$  
            44.86 & % IDSR $\downarrow$ 
            16 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.70m$ & % MOTP $\downarrow$
            0.192 & % MOTA $\uparrow$  
            0.324 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  0/151
            3.22 & % FN $\downarrow$  487/151
            0.193 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            5.16 & % IDSR $\downarrow$ 
            1.0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.58m$ & % MOTP $\downarrow$
            0.435 & % MOTA $\uparrow$  
            0.390 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  0/551
            2.23 & % FN $\downarrow$  1229/551
            0.442 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            33.90 & % IDSR $\downarrow$ 
            18 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.24m$ & % MOTP $\downarrow$
            0.574 & % MOTA $\uparrow$  
            0.370 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  0/311
            1.65 & % FN $\downarrow$  514/311
            0.586 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            25.56 & % IDSR $\downarrow$ 
            14 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            $1.43m$ & % MOTP $\downarrow$
            0.476 & % MOTA $\uparrow$  
            0.366 & % IDF1 $\uparrow$  
            0.777 & % MT $\uparrow$  
            0.666 & % ML $\downarrow$  
            0.015 & % FP $\downarrow$  
            1.80 & % FN $\downarrow$  
            0.490 & % Rcll $\uparrow$  
            0.987 & % Prcn $\uparrow$  
            41.47 & % IDSR $\downarrow$ 
            14.22 \\ %Frag $\downarrow$
            \hline\hline
            \multicolumn{15}{c}{Kalman Filter-based Tracker}\\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.38m$ & % MOTP $\downarrow$
            0.886 & % MOTA $\uparrow$  
            0.584 & % IDF1 $\uparrow$  
            4 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.17 & % FP $\downarrow$  94/541
            0.25 & % FN $\downarrow$  138/541
            0.936 & % Rcll $\uparrow$  
            0.956 & % Prcn $\uparrow$  
            9.61 & % IDSR $\downarrow$ 
            6 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.48m$ & % MOTP $\downarrow$
            0.671 & % MOTA $\uparrow$  
            0.427 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.28 & % FP $\downarrow$  161/571
            1.01 & % FN $\downarrow$  576/571
            0.747 & % Rcll $\uparrow$  
            0.913 & % Prcn $\uparrow$  
            17.38 & % IDSR $\downarrow$ 
            11 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.92m$ & % MOTP $\downarrow$
            0.545 & % MOTA $\uparrow$  
            0.435 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.27 & % FP $\downarrow$  149/551
            1.53 & % FN $\downarrow$  845/551
            0.616 & % Rcll $\uparrow$  
            0.901 & % Prcn $\uparrow$  
            12.97 & % IDSR $\downarrow$ 
            4 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.80m$ & % MOTP $\downarrow$
            0.334 & % MOTA $\uparrow$  
            0.501 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  0/151
            2.66 & % FN $\downarrow$  402/151
            0.334 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % IDSR $\downarrow$ 
            0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.75m$ & % MOTP $\downarrow$
            0.602 & % MOTA $\uparrow$  
            0.468 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.01 & % FP $\downarrow$  9/551
            1.56 & % FN $\downarrow$  859/551
            0.610 & % Rcll $\uparrow$  
            0.993 & % Prcn $\uparrow$  
            13.10 & % IDSR $\downarrow$ 
            9 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.11m$ & % MOTP $\downarrow$
            0.734 & % MOTA $\uparrow$  
            0.659 & % IDF1 $\uparrow$  
            3 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.65 & % FP $\downarrow$  205/311
            0.40 & % FN $\downarrow$  125/311
            0.899 & % Rcll $\uparrow$  
            0.845 & % Prcn $\uparrow$  
            4.44 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            $\mathbf{1.41m}$ & % MOTP $\downarrow$
            \textbf{0.629} & % MOTA $\uparrow$  
            \textbf{0.512} & % IDF1 $\uparrow$  
            1.833 & % MT $\uparrow$  
            0.333 & % ML $\downarrow$  
            0.23 & % FP $\downarrow$  
            1.23 & % FN $\downarrow$  
            0.690 & % Rcll $\uparrow$  
            0.934 & % Prcn $\uparrow$  
            9.58 & % IDSR $\downarrow$ 
            5.16 \\ %Frag $\downarrow$
            \hline\hline
            &
            5 people & 
            $13m \times 6m$ & % Size
            4 & % \faCamera
            $1.44m$ & % MOTP $\downarrow$
            0.798 & % MOTA $\uparrow$  
            0.700 & % IDF1 $\uparrow$  
            5 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0.65 & % FP $\downarrow$  219/336
            0.34 & % FN $\downarrow$  114/336
            0.932 & % Rcll $\uparrow$  
            0.877 & % Prcn $\uparrow$  
            6.43 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
        \end{tabular}
    \end{adjustbox}
    \label{tab:mot}
\end{table*}

==> table/mot_hungarian.tex <==
\begin{table}[t]
    \centering
    \caption{Multi-object localization and tracking performance using Hungarian Tracker.
    Hungarian Tracker does not consider temporal dynamics of detections over time and significantly impacted by the ID switching and missing samples in noisy detections.}
    \vspace{-0.1in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c||c|c||c|c|c|c|c|c|c|c|c|c|c|c}
            &
            Area & 
            Size ($H\times W$) &
            \faCamera &
            MOTP $\downarrow$ &
            MOTA $\uparrow$ & 
            IDF1 $\uparrow$ & 
            MT $\uparrow$ & 
            ML $\downarrow$ & 
            FP $\downarrow$ & 
            FN $\downarrow$ & 
            Rcll $\uparrow$ & 
            Prcn $\uparrow$ & 
            FAR $\downarrow$ & 
            IDSR $\downarrow$ & 
            Frag $\downarrow$ \\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.25m$ & % MOTP $\downarrow$
            0.776 & % MOTA $\uparrow$  
            0.530 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            8 & % FP $\downarrow$  
            457 & % FN $\downarrow$  
            0.788 & % Rcll $\uparrow$  
            0.995 & % Prcn $\uparrow$  
            1.478 & % FAR $\downarrow$  
            22.81 & % IDSR $\downarrow$ 
            16 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.39m$ & % MOTP $\downarrow$
            0.486 & % MOTA $\uparrow$  
            0.311 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            34 & % FP $\downarrow$  
            1117 & % FN $\downarrow$  
            0.510 & % Rcll $\uparrow$  
            0.971 & % Prcn $\uparrow$  
            5.954 & % FAR $\downarrow$  
            43.05 & % IDSR $\downarrow$ 
            17 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.55m$ & % MOTP $\downarrow$
            0.496 & % MOTA $\uparrow$  
            0.360 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            13 & % FP $\downarrow$  
            1074 & % FN $\downarrow$  
            0.512 & % Rcll $\uparrow$  
            0.988 & % Prcn $\uparrow$  
            2.359 & % FAR $\downarrow$  
            44.86 & % IDSR $\downarrow$ 
            16 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.70m$ & % MOTP $\downarrow$
            0.192 & % MOTA $\uparrow$  
            0.324 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            487 & % FN $\downarrow$  
            0.193 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            5.16 & % IDSR $\downarrow$ 
            1.0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.58m$ & % MOTP $\downarrow$
            0.435 & % MOTA $\uparrow$  
            0.390 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            1229 & % FN $\downarrow$  
            0.442 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            33.90 & % IDSR $\downarrow$ 
            18 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.24m$ & % MOTP $\downarrow$
            0.574 & % MOTA $\uparrow$  
            0.370 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            514 & % FN $\downarrow$  
            0.586 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            25.56 & % IDSR $\downarrow$ 
            14 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            $1.43m$ & % MOTP $\downarrow$
            0.476 & % MOTA $\uparrow$  
            0.366 & % IDF1 $\uparrow$  
            0.777 & % MT $\uparrow$  
            0.666 & % ML $\downarrow$  
            27.88 & % FP $\downarrow$  
            1289 & % FN $\downarrow$  
            0.490 & % Rcll $\uparrow$  
            0.987 & % Prcn $\uparrow$  
            3.245 & % FAR $\downarrow$  
            41.47 & % IDSR $\downarrow$ 
            14.22 \\ %Frag $\downarrow$
        \end{tabular}
    \end{adjustbox}
    \label{tab:mot_hungarian}
\end{table}

==> table/mot_kalman.tex <==
\begin{table}[t]
    \centering
    \caption{Multi-object localization and tracking performance at each area section in the study site when four participants were walking in the space.
    Area size for each data capure are is shown with height and width in meter.
    \faCamera\; shows the number of cameras that was covering the movement over 85\% of trajectories.
    Localization performance is measured by multiple object tracking precision (MOTP) and tracking performance was measured by multiple metrics to capture detailed behavior of the proposed method.
    Each area is annotated referring \autoref{fig:ep6_func} and \autoref{fig:data_collection}, Activity Area (A) include both Activity Studio and Gym area, and Kitchen (B) include the upper corridor between right boundary of dining area and left boundary of conversation room.
    Left corridor (C) is the narrow corridor right next to the Innovation Accelerator, and Right Corridor (E) is the narrow corridor where the Lockers are left to the Innovation Theater.
    Lounge (D) includes the area between elevator and reservation desk.
    Staff area (F) is at the most right region where staff offices are located.
    Overall performance shows average metrics across all areas combined.
    The last row shows the quantitative results for simulating complex movements from five people with occlusions in Activity Area.
    }
    \vspace{-0.1in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c ||c|c||c|c|c|c|c|c|c|c|c|c|c|c}
            &
            Area & 
            Size ($H\times W$) &
            \faCamera &
            MOTP $\downarrow$ &
            MOTA $\uparrow$ & 
            IDF1 $\uparrow$ & 
            MT $\uparrow$ & 
            ML $\downarrow$ & 
            FP $\downarrow$ & 
            FN $\downarrow$ & 
            Rcll $\uparrow$ & 
            Prcn $\uparrow$ & 
            FAR $\downarrow$ & 
            IDSR $\downarrow$ & 
            Frag $\downarrow$ \\
            \hline\hline
            A &
            Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
            $1.38m$ & % MOTP $\downarrow$
            0.886 & % MOTA $\uparrow$  
            0.584 & % IDF1 $\uparrow$  
            4 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            94 & % FP $\downarrow$  
            138 & % FN $\downarrow$  
            0.936 & % Rcll $\uparrow$  
            0.956 & % Prcn $\uparrow$  
            17.37 & % FAR $\downarrow$  
            9.61 & % IDSR $\downarrow$ 
            6 \\ % Frag $\downarrow$
            \hline
            B &
            Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
            $1.48m$ & % MOTP $\downarrow$
            0.671 & % MOTA $\uparrow$  
            0.427 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            161 & % FP $\downarrow$  
            576 & % FN $\downarrow$  
            0.747 & % Rcll $\uparrow$  
            0.913 & % Prcn $\uparrow$  
            28.19 & % FAR $\downarrow$  
            17.38 & % IDSR $\downarrow$ 
            11 \\ % Frag $\downarrow$
            \hline
            C &
            Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
            $1.92m$ & % MOTP $\downarrow$
            0.545 & % MOTA $\uparrow$  
            0.435 & % IDF1 $\uparrow$  
            1 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            149 & % FP $\downarrow$  
            845 & % FN $\downarrow$  
            0.616 & % Rcll $\uparrow$  
            0.901 & % Prcn $\uparrow$  
            27.04 & % FAR $\downarrow$  
            12.97 & % IDSR $\downarrow$ 
            4 \\ %Frag $\downarrow$
            \hline
            D &
            Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
            $0.80m$ & % MOTP $\downarrow$
            0.334 & % MOTA $\uparrow$  
            0.501 & % IDF1 $\uparrow$  
            0 & % MT $\uparrow$  
            2 & % ML $\downarrow$  
            0 & % FP $\downarrow$  
            402 & % FN $\downarrow$  
            0.334 & % Rcll $\uparrow$  
            1.0 & % Prcn $\uparrow$  
            0.0 & % FAR $\downarrow$  
            0.0 & % IDSR $\downarrow$ 
            0 \\ %Frag $\downarrow$
            \hline
            E &
            Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
            $1.75m$ & % MOTP $\downarrow$
            0.602 & % MOTA $\uparrow$  
            0.468 & % IDF1 $\uparrow$  
            2 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            9 & % FP $\downarrow$  
            859 & % FN $\downarrow$  
            0.610 & % Rcll $\uparrow$  
            0.993 & % Prcn $\uparrow$  
            1.633 & % FAR $\downarrow$  
            13.10 & % IDSR $\downarrow$ 
            9 \\ %Frag $\downarrow$
            \hline
            F &
            Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
            $1.11m$ & % MOTP $\downarrow$
            0.734 & % MOTA $\uparrow$  
            0.659 & % IDF1 $\uparrow$  
            3 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            205 & % FP $\downarrow$  
            125 & % FN $\downarrow$  
            0.899 & % Rcll $\uparrow$  
            0.845 & % Prcn $\uparrow$  
            65.91 & % FAR $\downarrow$  
            4.44 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
            \hline\hline
            &
            Overall & 
            - & % Size
            - & % \faCamera
            \textbf{$1.41m$} & % MOTP $\downarrow$
            \textbf{0.629} & % MOTA $\uparrow$  
            \textbf{0.512} & % IDF1 $\uparrow$  
            1.833 & % MT $\uparrow$  
            0.333 & % ML $\downarrow$  
            103 & % FP $\downarrow$  
            490.8 & % FN $\downarrow$  
            0.690 & % Rcll $\uparrow$  
            0.934 & % Prcn $\uparrow$  
            23.36 & % FAR $\downarrow$  
            9.58 & % IDSR $\downarrow$ 
            5.16 \\ %Frag $\downarrow$
            \hline\hline
            &
            5 people & 
            $13m \times 6m$ & % Size
            4 & % \faCamera
            $1.44m$ & % MOTP $\downarrow$
            0.798 & % MOTA $\uparrow$  
            0.700 & % IDF1 $\uparrow$  
            5 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            219 & % FP $\downarrow$  
            114 & % FN $\downarrow$  
            0.932 & % Rcll $\uparrow$  
            0.877 & % Prcn $\uparrow$  
            65.17 & % FAR $\downarrow$  
            6.43 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
        \end{tabular}
    \end{adjustbox}
    \label{tab:mot}
\end{table}

==> table/mot_traj.tex <==
\begin{table}[t]
    \centering
    \caption{Multi-object tracking performance for five people showing complex movements in Activity Area.}
    \vspace{-0.1in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c ||c|c||c|c|c|c|c|c|c|c|c|c|c|c}
            Area & 
            Size ($H\times W$) &
            \faCamera &
            MOTP $\downarrow$ &
            MOTA $\uparrow$ & 
            IDF1 $\uparrow$ & 
            MT $\uparrow$ & 
            ML $\downarrow$ & 
            FP $\downarrow$ & 
            FN $\downarrow$ & 
            Rcll $\uparrow$ & 
            Prcn $\uparrow$ & 
            FAR $\downarrow$ & 
            IDSR $\downarrow$ & 
            Frag $\downarrow$ \\
            \hline\hline
            Activity Area & 
            $13m \times 6m$ & % Size
            4 & % \faCamera
            $1.44m$ & % MOTP $\downarrow$
            0.7982 & % MOTA $\uparrow$  
            0.7001 & % IDF1 $\uparrow$  
            5 & % MT $\uparrow$  
            0 & % ML $\downarrow$  
            219 & % FP $\downarrow$  
            114 & % FN $\downarrow$  
            0.9321 & % Rcll $\uparrow$  
            0.8773 & % Prcn $\uparrow$  
            65.17 & % FAR $\downarrow$  
            6.43 & % IDSR $\downarrow$ 
            1 \\ %Frag $\downarrow$
        \end{tabular}
    \end{adjustbox}
    \label{tab:mot_traj}
\end{table}

==> table/orientation.tex <==
\begin{table*}[t]
    \centering
    \caption{
    Body orientation estimation performance.
    We measured the Mean Absolute Error (MAE) and Accuracy-$X\degree$.
    The predictions are considered correct when the angular error is within $X\degree$ of the ground-truth orientation. 
    Following Wu~\etal~\cite{wu2020mebow}, we used $X\in\{5\degree, 15\degree, 22.5\degree, 30\degree, 45\degree, 90\degree\}$.
    The first six rows show the body orientation estimation performance at each area while four people walk in the space, and the seventh row shows the overall performance considering the entire area.
    While people walk in the study site, the model can closely estimate the body orientation with MAE of 28.97\degree and Acc.-45\degree of 78.9\% which shows that our model can distinguish eight (N, NE, E, SE, S, SW, W, NW) orientations with sufficient margin of errors.
    5 people moving with a more complex trajectory in Activity Area (8th row) resulted in an MAE of 48.33\degree.
    Our model has been significantly confused by occlusion between people, as detected bounding boxes include multiple people with different orientations.
    Yet, our model can identify equally spaced four (N, E, S, W) orientations with sufficient margin of error showing Acc.-90\degree of 81.4\%.
    The last four rows show the estimation performance when a person stands in space but rotates only their orientations.
    The first three rows show the evaluation from three different sessions, and the last row shows the aggregated results.
    Our model found it more challenging to estimate when a person is in place.
    In these cases, our model could classify equally spaced four (N, E, S, W) with tighter margin of error showing MAE of 63.4\degree and Acc.-90\degree of 69.3\%.
    Due to our method's frame-by-frame approach, it was difficult to detect fine orientation changes between $5\degree\sim 10\degree$ across frames.
    Generally, our model performed better when people were walking as the Kalman Filter updates the orientation information to incorporate moving directions as the user moves.
    }    
    \vspace{-0.0in}
    \begin{adjustbox}{width=\textwidth,center}
        \begin{tabular}{c c||c|c||c||c|c|c|c|c|c}
            &
            Area & 
            Size ($H\times W$) &
            \faCamera &
             MAE-$\theta\degree$ &
             Acc.-$5\degree$ &
             Acc.-$15\degree$ &
             Acc.-$22.5\degree$ &
             Acc.-$30\degree$ &
             Acc.-$45\degree$ &
             Acc.-$90\degree$ \\
             \hline\hline
             A &
             Activity Area & 
            $21m \times 5m$ & % Size
            7 & % \faCamera
             25.91\degree & % MAE-$\theta\degree$ &
             0.319 & %Acc.-$5\degree$
             0.622 & %Acc.-$15\degree$
             0.723 & %Acc.-$22.5\degree$
             0.800 & %Acc.-$30\degree$
             0.855 & %Acc.-$45\degree$
             0.912 \\ %Acc.-$90\degree$ 
             \hline
             B &
             Kitchen & 
            $3m\times 24m$ & % Size
            3 & % \faCamera
             31.06\degree & % MAE-$\theta\degree$ &
             0.207 & %Acc.-$5\degree$
             0.489 & %Acc.-$15\degree$
             0.590 & %Acc.-$22.5\degree$
             0.650 & %Acc.-$30\degree$
             0.748 & %Acc.-$45\degree$
             0.916 \\ %Acc.-$90\degree$ 
             \hline
             C &
             Left Corridor & 
            $33m\times 2m$ & % Size
            3 & % \faCamera
             21.68\degree & % MAE-$\theta\degree$ &
             0.223 & %Acc.-$5\degree$
             0.578 & %Acc.-$15\degree$
             0.706 & %Acc.-$22.5\degree$
             0.793 & %Acc.-$30\degree$
             0.887 & %Acc.-$45\degree$
             0.955 \\ %Acc.-$90\degree$ 
             \hline
             D &
             Lounge & 
            $3m \times 8m$ & % Size
            1 & % \faCamera
             47.37\degree & % MAE-$\theta\degree$ &
             0.038 & %Acc.-$5\degree$
             0.137 & %Acc.-$15\degree$
             0.302 & %Acc.-$22.5\degree$
             0.423 & %Acc.-$30\degree$
             0.554 & %Acc.-$45\degree$
             0.846 \\ %Acc.-$90\degree$ 
             \hline
             E &
             Right Corridor & 
            $33m\times 1.5m$ & % Size
            2 & % \faCamera
             32.41\degree & % MAE-$\theta\degree$ &
             0.214 & %Acc.-$5\degree$
             0.479 & %Acc.-$15\degree$
             0.556 & %Acc.-$22.5\degree$
             0.602 & %Acc.-$30\degree$
             0.674 & %Acc.-$45\degree$
             0.946 \\ %Acc.-$90\degree$ 
             \hline
             F &
             Staff Zone & 
            $14m\times 3m$ & % Size
            4 & % \faCamera
             33.68\degree & % MAE-$\theta\degree$ &
             0.096 & %Acc.-$5\degree$
             0.324 & %Acc.-$15\degree$
             0.464 & %Acc.-$22.5\degree$
             0.589 & %Acc.-$30\degree$
             0.778 & %Acc.-$45\degree$
             0.942 \\ %Acc.-$90\degree$ 
             \hline\hline
             &
             Overall & 
            - & % Size
            - & % \faCamera
             \textbf{28.97\degree} & % MAE-$\theta\degree$ &
             0.220 & %Acc.-$5\degree$
             0.506 & %Acc.-$15\degree$
             0.615 & %Acc.-$22.5\degree$
             0.693 & %Acc.-$30\degree$
             0.789 & %Acc.-$45\degree$
             0.930 \\ %Acc.-$90\degree$ 
             \hline\hline
             &
             5 people & 
            $13m \times 6m$ & % Size
            4 & % \faCamera
             48.33\degree & % MAE-$\theta\degree$ &
             0.149 & %Acc.-$5\degree$
             0.328 & %Acc.-$15\degree$
             0.417 & %Acc.-$22.5\degree$
             0.512 & %Acc.-$30\degree$
             0.629 & %Acc.-$45\degree$
             0.814 \\ %Acc.-$90\degree$ 
             \hline\hline
             &
             In-place (Sess. 1) & 
            $11m \times 5m$ & % Size
            3 & % \faCamera
             73.73\degree & % MAE-$\theta\degree$ &
             0.087 & %Acc.-$5\degree$
             0.181 & %Acc.-$15\degree$
             0.255 & %Acc.-$22.5\degree$
             0.261 & %Acc.-$30\degree$
             0.322 & %Acc.-$45\degree$
             0.644 \\ %Acc.-$90\degree$ 
             \hline
             &
             In-place (Sess. 2) & 
            $4m \times 7m$ & % Size
            2 & % \faCamera
             65.28\degree & % MAE-$\theta\degree$ &
             0.078 & %Acc.-$5\degree$
             0.212 & %Acc.-$15\degree$
             0.236 & %Acc.-$22.5\degree$
             0.290 & %Acc.-$30\degree$
             0.375 & %Acc.-$45\degree$
             0.672 \\ %Acc.-$90\degree$ 
             \hline
             &
             In-place (Sess. 3) & 
            $3m \times 5m$ & % Size
            4 & % \faCamera
             50.47\degree & % MAE-$\theta\degree$ &
             0.111 & %Acc.-$5\degree$
             0.265 & %Acc.-$15\degree$
             0.454 & %Acc.-$22.5\degree$
             0.580 & %Acc.-$30\degree$
             0.692 & %Acc.-$45\degree$
             0.769 \\ %Acc.-$90\degree$ 
             \hline\hline
             &
             In-place (Overall) & 
            - & % Size
            - & % \faCamera
             63.40\degree & % MAE-$\theta\degree$ &
             0.091 & %Acc.-$5\degree$
             0.218 & %Acc.-$15\degree$
             0.310 & %Acc.-$22.5\degree$
             0.371 & %Acc.-$30\degree$
             0.457 & %Acc.-$45\degree$
             0.693 \\ %Acc.-$90\degree$ 
        \end{tabular}
    \end{adjustbox}
    \label{tab:orientation}
\end{table*}

==> table/orientation_compare.tex <==
\begin{table*}[t]
    \centering
    \caption{
    Comparison of mean absolute error (MAE) between different body orientation estimation methods for the dataset collected from four participants.
    In the first two methods, only 2D information is used, either by heuristic or learning approaches.
    Two other methods additionally model 3D information for body orientation estimation by using a geometric- or learning-based approach.
    The body orientation estimation method based on only 2D pose information performs significantly worse than the algorithm based on 3D geometry information.
    Particularly, the proposed model (3D-Learning) significantly outperforms other methods by modeling 3D information as well as complex functions to estimate body orientation. 
    }
    \vspace{-0.0in}
    \begin{tabular}{c|c||c|c|c|c|c|c||c}
        \multicolumn{2}{c||}{} & \multicolumn{7}{c}{Mean Absolute Error (MAE)-$\theta\degree$} \\
        \cline{3-9}
        \multicolumn{2}{c||}{Method} & A & B & C & D & E & F\\
        \multicolumn{1}{c}{} &
        & Activity Area & Kitchen & Left Corridor & Lounge & Right Corridor & Staff Zone & Overall \\
        \hline\hline
        \multirow{2}{*}{2D} & Heuristic & 
        155.67\degree & % Activity Area
        146.91\degree & % Kitchen
        128.80\degree & % Left Corridor
        122.62\degree & % Lounge
        78.03\degree & % Right Corridor
        125.09\degree & % Staff Zone
        130.34\degree \\ % Overall
        \cline{2-9}
        & Learning & 
        92.62\degree & % Activity Area
        103.74\degree & % Kitchen
        111.00\degree & % Left Corridor
        61.42\degree & % Lounge
        129.06\degree & % Right Corridor
        123.01\degree & % Staff Zone
        108.34\degree \\ % Overall
        \hline
        \multirow{2}{*}{3D} & Geometry & 
        63.21\degree & % Activity Area
        60.44\degree & % Kitchen
        84.08\degree & % Left Corridor
        109.11\degree & % Lounge
        98.35\degree & % Right Corridor
        70.10\degree & % Staff Zone
        74.59\degree \\ % Overall
        \cline{2-9}
         & Learning & 
        25.91\degree & % Activity Area
        31.06\degree & % Kitchen
        21.68\degree & % Left Corridor
        47.37\degree & % Lounge
        32.41\degree & % Right Corridor
        33.68\degree & % Staff Zone
        \textbf{28.97}\degree \\ % Overall
    \end{tabular}
    \label{tab:ori_compare}
\end{table*}
